The Star Formation Reference Survey. IV. Stellar mass distribution of local star-forming galaxies

We constrain the mass distribution in nearby, star-forming galaxies with the Star Formation Reference Survey (SFRS), a galaxy sample constructed to be representative of all known combinations of star formation rate (SFR), dust temperature, and specific star formation rate (sSFR) that exist in the Local Universe. An innovative two-dimensional bulge/disk decomposition of the 2MASS/$K_{s}$-band images of the SFRS galaxies yields global luminosity and stellar mass functions, along with separate mass functions for their bulges and disks. These accurate mass functions cover the full range from dwarf galaxies to large spirals, and are representative of star-forming galaxies selected based on their infra-red luminosity, unbiased by AGN content and environment. We measure an integrated luminosity density $j$ = 1.72 $\pm$ 0.93 $\times$ 10$^{9}$ L$_{\odot}$ $h^{-1}$ Mpc$^{-3}$ and a total stellar mass density $\rho_{M}$ = 4.61 $\pm$ 2.40 $\times$ 10$^{8}$ M$_{\odot}$ $h^{-1}$ Mpc$^{-3}$. While the stellar mass of the \emph{average} star-forming galaxy is equally distributed between its sub-components, disks globally dominate the mass density budget by a ratio 4:1 with respect to bulges. In particular, our functions suggest that recent star formation happened primarily in massive systems, where they have yielded a disk stellar mass density larger than that of bulges by more than 1 dex. Our results constitute a reference benchmark for models addressing the assembly of stellar mass on the bulges and disks of local ($z = 0$) star-forming galaxies.

==> full_tables/TABLE_D1/TABLE_SFRS_2MASS_SDSS_full.tex <==
%------------------------------------- TABLE  -------------------------------------
\begin{landscape}
 \small 
 \begin{longtable}{llccccccc}
  \caption*{Table D1: List of SDSS (Data Release 12) $u$, $r$, and 2MASS $J$, $H$, $K$ magnitudes for the SFRS sample.}\\
  \hline
  \multicolumn{9}{c}{\textsc{SFRS --- 2MASS and SDSS Photometry}} \\
  \hline
  \addlinespace % requires packages booktabs and longtable
  \hline
  \addlinespace % requires packages booktabs and longtable
  \multicolumn{1}{c}{SFRS}       & \multicolumn{1}{c}{Target}	  & \multicolumn{3}{c}{\hrulefill~~SDSS~~\hrulefill} & \multicolumn{4}{c}{\hrulefill~~2MASS~~\hrulefill}             \\
  \multicolumn{1}{c}{ID}         & \multicolumn{1}{c}{Name}	  & ID	       & $u^{\dagger}$ & $r^{\dagger}$       & ID	  & $J^{\ddagger}$ & $H^{\ddagger}$ & $K^{\ddagger}$ \\ 
  \multicolumn{1}{c}{\tiny{(1)}} & \multicolumn{1}{c}{\tiny{(2)}} & \tiny{(3)} & \tiny{(4)}    & \tiny{(5)}          & \tiny{(6)} & \tiny{(7)}     & \tiny{(8)}     & \tiny{(9)}     \\
  \hline
  \addlinespace % requires packages booktabs and longtable
  \endfirsthead

  \multicolumn{8}{@{}l}{Table D1 - \emph{continued}}\\
  \hline
  \multicolumn{1}{c}{SFRS}       & \multicolumn{1}{c}{Target}	  & \multicolumn{3}{c}{\hrulefill~~SDSS~~\hrulefill} & \multicolumn{4}{c}{\hrulefill~~2MASS~~\hrulefill}             \\
  \multicolumn{1}{c}{ID}         & \multicolumn{1}{c}{Name}	  & ID	       & $u^{\dagger}$ & $r^{\dagger}$       & ID	  & $J^{\ddagger}$ & $H^{\ddagger}$ & $K^{\ddagger}$ \\ 
  \multicolumn{1}{c}{\tiny{(1)}} & \multicolumn{1}{c}{\tiny{(2)}} & \tiny{(3)} & \tiny{(4)}    & \tiny{(5)}          & \tiny{(6)} & \tiny{(7)}     & \tiny{(8)}     & \tiny{(9)}     \\
  \hline
  \addlinespace % requires packages booktabs and longtable
  \endhead
1   & IC486                          & SDSSJ080020.98+263648.8  & 15.856(0.006) & 13.377(0.002) & XSC---08002097+2636483  & 11.514(0.020) & 10.826(0.021) & 10.496(0.028) \\
2   & IC2217                         & SDSSJ080049.73+273001.5  & 15.269(0.005) & 13.838(0.002) & XSC---08004972+2730010  & 11.834(0.024) & 11.186(0.027) & 10.898(0.040) \\
3   & NGC2500                        & SDSSJ080153.17+504413.5  & 14.104(0.005) & 12.263(0.002) & XSC---08015322+5044135  & 10.790(0.021) & 10.160(0.030) &  9.276(0.065) \\
4   & NGC2512                        & SDSSJ080307.84+232330.5  & 15.081(0.005) & 12.865(0.002) & XSC---08030785+2323308  & 10.859(0.020) & 10.117(0.026) &  9.820(0.028) \\
5   & MCG6-18-009                    & SDSSJ080328.94+332744.5  & 15.502(0.006) & 13.642(0.002) & XSC---08032897+3327444  & 11.803(0.034) & 11.135(0.034) & 10.763(0.040) \\
6   & MK1212                         & SDSSJ080705.51+270733.7  & 16.365(0.007) & 14.588(0.002) & XSC---08070551+2707336  & 12.594(0.026) & 11.995(0.032) & 11.589(0.045) \\
7   & IRAS08072+1847                 & SDSSJ081006.99+183818.0  & 18.271(0.020) & 15.590(0.003) & XSC---08100697+1838176  & 13.270(0.038) & 12.684(0.059) & 12.189(0.056) \\
8   & NGC2532                        & SDSSJ081015.17+335723.9  & 15.549(0.009) & 12.983(0.002) & XSC---08101519+3357233  & 10.643(0.022) & 10.004(0.029) &  9.615(0.036) \\
9   & UGC4261                        & SDSSJ081056.21+364941.3  & 15.771(0.006) & 14.984(0.003) & XSC---08105615+3649435  & 12.887(0.037) & 12.291(0.056) & 12.027(0.067) \\
10  & NGC2535                        & SDSSJ081113.48+251224.8  & 15.227(0.008) & 12.980(0.002) & XSC---08111348+2512249  & 10.993(0.027) & 10.341(0.029) & 10.120(0.043) \\
11  & NGC2543                        & SDSSJ081257.92+361516.6  & 15.083(0.007) & 12.514(0.002) & XSC---08125795+3615162  & 10.532(0.023) &  9.745(0.026) &  9.431(0.030) \\
12  & NGC2537                        & SDSSJ081314.69+455922.0  & 13.880(0.004) & 12.318(0.002) & XSC---08131464+4559232  &  9.949(0.022) &  9.366(0.025) &  9.130(0.034) \\
13  & IC2233                         & SDSSJ081358.77+454441.9  & 20.296(0.052) & 22.550(0.250) & XSC---08135890+4544317  & 11.463(0.032) & 10.950(0.042) & 10.754(0.062) \\
14  & IC2239                         & SDSSJ081406.79+235158.9  & 15.931(0.007) & 13.527(0.002) & XSC---08140678+2351588  & 11.363(0.021) & 10.687(0.025) & 10.339(0.028) \\
15  & UGC4286                        & SDSSJ081416.47+182626.3  & 16.045(0.011) & 13.570(0.002) & XSC---08141648+1826258  & 11.897(0.025) & 11.175(0.033) & 10.868(0.038) \\
16  & UGC4306                        & SDSSJ081736.78+352644.3  & 16.221(0.011) & 13.585(0.002) & XSC---08173676+3526455  & 11.449(0.023) & 10.660(0.024) & 10.333(0.030) \\
17  & NGC2552                        & SDSSJ081919.17+500017.6  & 22.230(0.295) & 20.584(0.047) & XSC---08192055+5000351  & 14.524(0.088) & 13.859(0.122) & 13.607(0.148) \\
18  & UGC4383                        & SDSSJ082334.21+212051.5  & 15.614(0.006) & 13.892(0.002) & XSC---08233424+2120514  & 12.244(0.037) & 11.575(0.040) & 11.368(0.047) \\
19  & IRAS08234+1054                 & SDSSJ082607.85+104451.0  & 21.853(0.272) & 18.768(0.014) & XSC---08260790+1044514  & 13.927(0.094) & 13.053(0.086) & 12.778(0.167) \\
20  & IRAS08269+1514                 & SDSSJ082945.19+150439.3  & 17.804(0.031) & 15.671(0.005) & XSC---08294519+1504394  & 13.671(0.075) & 12.934(0.089) & 12.373(0.090) \\
21  & NGC2604                        & SDSSJ083323.13+293219.7  & 14.412(0.004) & 13.363(0.002) & XSC---08332305+2932190  & 12.041(0.037) & 11.422(0.050) & 11.044(0.060) \\
22  & NGC2608                        & SDSSJ083517.33+282824.3  & 15.016(0.007) & 12.838(0.002) & XSC---08351736+2828246  & 10.299(0.019) &  9.611(0.023) &  9.326(0.030) \\
23  & MK92                           & SDSSJ083539.96+462928.1  & 16.065(0.005) & 14.632(0.002) & XSC---08353993+4629279  & 12.493(0.071) & 11.797(0.066) & 11.468(0.053) \\
24  & NGC2623                        & SDSSJ083824.01+254516.2  & 16.134(0.008) & 13.802(0.002) & XSC---08382409+2545167  & 11.572(0.020) & 10.808(0.025) & 10.427(0.027) \\
25  & CGCG120-018                    & SDSSJ083950.75+230836.1  & 16.946(0.014) & 14.502(0.002) & XSC---08395080+2308357  & 12.582(0.032) & 11.803(0.038) & 11.488(0.051) \\
26  & NGC2644                        & SDSSJ084131.84+045851.3  & 14.925(0.005) & 13.184(0.002) & XSC---08413189+0458488  & 11.232(0.034) & 10.646(0.043) & 10.359(0.061) \\
27  & UGC4572                        & SDSSJ084537.85+365604.7  & 15.566(0.005) & 13.276(0.002) & XSC---08453783+3656047  & 11.546(0.024) & 10.896(0.023) & 10.649(0.039) \\
28  & UGC4653                        & SDSSJ085354.62+350844.0  & 16.746(0.013) & 14.370(0.002) & XSC---08535462+3508439  & 11.960(0.104) & 11.150(0.040) & 10.654(0.033) \\
29  & IRAS08512+2727                 & SDSSJ085416.77+271559.5  & 16.640(0.008) & 14.837(0.002) & XSC---08541681+2715592  & 12.952(0.043) & 12.392(0.069) & 11.924(0.067) \\
30  & OJ287                          & SDSSJ085448.87+200630.6  & 16.573(0.007) & 15.421(0.004) & XSC---08544889+2006307  & 13.503(0.039) & 12.567(0.039) & 11.768(0.032) \\
31  & IRAS08538+4256                 & SDSSJ085710.39+424522.9  & 17.212(0.014) & 14.905(0.003) & XSC---08571044+4245234  & 12.816(0.049) & 11.930(0.056) & 11.627(0.062) \\
32  & IRAS08550+3908                 & SDSSJ085813.73+385632.1  & 18.451(0.029) & 16.146(0.005) & XSC---08581389+3856314  & 13.332(0.059) & 12.536(0.070) & 11.870(0.060) \\
33  & NGC2718                        & SDSSJ085850.46+061734.7  & 14.718(0.005) & 12.672(0.002) & XSC---08585046+0617354  & 10.560(0.020) &  9.857(0.027) &  9.512(0.026) \\
34  & NGC2712                        & SDSSJ085930.47+445450.0  & 14.306(0.004) & 12.029(0.002) & XSC---08593045+4454504  & 10.010(0.021) &  9.368(0.024) &  9.103(0.030) \\
35  & NGC2719                        & SDSSJ090015.70+354339.4  & 15.140(0.004) & 14.113(0.002) & XSC---09001576+3543387  & 12.492(0.031) & 12.196(0.054) & 11.833(0.071) \\
36  & IRAS08572+3915NW               & SDSSJ090025.37+390353.7  & 18.713(0.034) & 16.848(0.005) & XSC---09002536+3903542  & 14.968(0.125) & 13.748(0.103) & 13.082(0.087) \\
37  & IRAS08579+3447                 & SDSSJ090105.72+343526.2  & 17.353(0.016) & 15.341(0.003) & XSC---09010572+3435270  & 13.262(0.043) & 12.448(0.050) & 12.021(0.060) \\
38  & NGC2731                        & SDSSJ090208.40+081805.9  & 14.920(0.005) & 13.179(0.002) & XSC---09020839+0818063  & 11.452(0.030) & 10.815(0.037) & 10.491(0.052) \\
39  & NGC2730                        & SDSSJ090215.83+165017.6  & 15.392(0.009) & 13.513(0.002) & XSC---09021583+1650175  & 12.473(0.034) & 11.887(0.060) & 11.823(0.076) \\
40  & IC2431                         & SDSSJ090434.23+143544.7  & 24.524(0.963) & 22.332(0.165) & PSC---09043464+1435432  & 13.599(NA)    &  13.47(0.115) & 12.926(0.116) \\
41  & NGC2750                        & SDSSJ090547.92+252614.9  & 15.058(0.005) & 13.437(0.002) & XSC---09054789+2526145  & 10.484(0.034) & 10.051(0.054) &  9.672(0.056) \\
42  & IC2434                         & SDSSJ090716.05+371255.3  & 15.462(0.008) & 12.797(0.002) & XSC---09071631+3712555  & 11.284(0.018) & 10.579(0.023) & 10.236(0.026) \\
43  & NGC2761                        & SDSSJ090730.82+182605.2  & 16.747(0.012) & 14.166(0.002) & XSC---09073082+1826057  & 11.907(0.028) & 11.178(0.037) & 10.739(0.037) \\
44  & NGC2773                        & SDSSJ090944.17+071025.8  & 16.393(0.046) & 13.892(0.002) & XSC---09094416+0710255  & 11.572(0.024) & 10.833(0.025) & 10.502(0.034) \\
45  & NGC2776                        & SDSSJ091214.51+445717.4  & 14.143(0.005) & 11.969(0.002) & XSC---09121453+4457176  & 10.050(0.024) &  9.442(0.023) &  9.131(0.035) \\
46  & NGC2789                        & SDSSJ091459.66+294348.8  & 14.944(0.004) & 12.636(0.002) & XSC---09145961+2943492  & 10.862(0.022) & 10.114(0.024) &  9.846(0.027) \\
47  & NGC2824                        & SDSSJ091902.22+261611.9  & 15.540(0.006) & 13.032(0.002) & XSC---09190222+2616119  & 11.076(0.019) & 10.398(0.020) & 10.126(0.027) \\
48  & IRAS09121+3908                 & SDSSJ091522.14+385635.0  & 19.715(0.052) & 16.803(0.004) & XSC---09152215+3856355  & 14.167(0.069) & 13.567(0.097) & 12.868(0.091) \\
49  & IRAS09184+4356                 & SDSSJ092138.71+434334.2  & 17.528(0.015) & 15.072(0.003) & XSC---09213873+4343339  & 12.902(0.036) & 12.048(0.037) & 11.760(0.053) \\
50  & CGCG238-041                    & SDSSJ092225.27+471440.0  & 16.327(0.006) & 15.341(0.003) & XSC---09222523+4714401  & 13.936(0.059) & 13.576(0.112) & 12.968(0.107) \\
51  & IRAS09197+2210                 & SDSSJ092237.39+215726.7  & 17.832(0.024) & 15.287(0.003) & XSC---09223730+2157258  & 13.050(0.042) & 12.271(0.058) & 11.819(0.052) \\
52  & NGC2854                        & SDSSJ092403.06+491215.5  & 15.135(0.015) & 13.024(0.006) & XSC---09240315+4912156  & 11.046(0.025) & 10.326(0.032) & 10.095(0.031) \\
53  & UGC5046                        & SDSSJ092806.64+171147.3  & 15.212(0.006) & 13.589(0.002) & XSC---09280661+1711473  & 11.737(0.026) & 10.983(0.025) & 10.616(0.029) \\
54  & UGC5055                        & SDSSJ093011.75+555108.7  & 15.848(0.006) & 13.772(0.002) & XSC---09301176+5551085  & 11.850(0.027) & 11.147(0.027) & 10.801(0.036) \\
55  & NGC2893                        & SDSSJ093016.95+293223.8  & 14.812(0.004) & 12.832(0.002) & XSC---09301694+2932239  & 11.235(0.018) & 10.514(0.018) & 10.309(0.023) \\
56  & MCG3-24-062                    & SDSSJ093022.98+192809.2  & 16.605(0.017) & 13.939(0.002) & XSC---09302300+1928090  & 12.080(0.029) & 11.284(0.033) & 10.798(0.038) \\
57  & CGCG238-066                    & SDSSJ093106.75+490447.1  & 16.407(0.009) & 14.246(0.002) & XSC---09310680+4904467  & 12.424(0.027) & 11.710(0.038) & 11.406(0.043) \\
58  & UGC5097                        & SDSSJ093410.54+001430.3  & 14.939(0.004) & 13.742(0.002) & XSC---09341062+0014312  & 12.010(0.031) & 11.433(0.035) & 11.182(0.063) \\
59  & CGCG289-012                    & SDSSJ093631.88+592354.2  & 16.362(0.009) & 14.628(0.002) & XSC---09363188+5923544  & 12.630(0.034) & 12.072(0.060) & 11.650(0.048) \\
60  & MCG8-18-013                    & SDSSJ093637.18+482827.8  & 16.368(0.008) & 14.278(0.002) & XSC---09363719+4828275  & 12.133(0.028) & 11.429(0.036) & 11.069(0.037) \\
61  & CGCG181-068                    & SDSSJ093719.22+334925.7  & 17.218(0.018) & 14.587(0.002) & XSC---09371929+3349247  & 12.293(0.036) & 11.478(0.040) & 10.994(0.041) \\
62  & NGC2936                        & SDSSJ093744.14+024538.9  & 16.717(0.013) & 13.639(0.002) & XSC---09374413+0245394  & 10.872(0.023) & 10.136(0.025) &  9.850(0.041) \\
63  & NGC2955                        & SDSSJ094116.61+355256.1  & 14.690(0.005) & 12.597(0.002) & XSC---09411660+3552556  & 10.994(0.022) & 10.295(0.031) & 10.040(0.030) \\
64  & CGCG182-010                    & SDSSJ094515.21+344244.2  & 16.714(0.010) & 14.490(0.002) & XSC---09451522+3442443  & 12.491(0.027) & 11.766(0.032) & 11.367(0.044) \\
65  & UGC5228                        & SDSSJ094603.59+014006.0  & 15.181(0.010) & 13.116(0.004) & XSC---09460365+0140059  & 11.235(0.041) & 10.584(0.045) & 10.169(0.061) \\
66  & IRAS09438+1141                 & SDSSJ094632.56+112719.5  & 16.943(0.011) & 15.135(0.003) & XSC---09463253+1127199  & 13.486(0.071) & 12.684(0.066) & 12.432(0.112) \\
67  & NGC3015                        & SDSSJ094922.91+010843.5  & 15.630(0.006) & 13.505(0.002) & XSC---09492289+0108437  & 11.619(0.023) & 10.841(0.023) & 10.566(0.033) \\
68  & MCG2-25-039                    & SDSSJ094936.99+090018.7  & 15.961(0.007) & 14.026(0.002) & XSC---09493698+0900192  & 12.369(0.039) & 11.527(0.037) & 11.297(0.057) \\
69  & NGC3020                        & SDSSJ095006.62+124849.2  & 14.436(0.004) & 13.133(0.002) & XSC---09500659+1248489  & 11.482(0.039) & 10.967(0.063) & 10.683(0.076) \\
70  & NGC3049                        & SDSSJ095449.56+091615.8  & 14.414(0.004) & 12.777(0.002) & XSC---09544965+0916179  & 10.928(0.039) & 10.296(0.045) &  9.958(0.062) \\
71  & NGC3055                        & SDSSJ095518.06+041612.0  & 13.896(0.003) & 12.341(0.002) & XSC---09551804+0416122  & 10.406(0.027) &  9.717(0.026) &  9.494(0.042) \\
72  & IC2520                         & SDSSJ095620.11+271339.2  & 15.638(0.006) & 13.675(0.002) & XSC---09562016+2713393  & 11.391(0.023) & 10.659(0.021) & 10.377(0.028) \\
73  & UGC5403                        & SDSSJ100235.54+191036.8  & 15.694(0.008) & 13.230(0.002) & XSC---10023555+1910374  & 11.369(0.017) & 10.611(0.022) & 10.336(0.025) \\
74  & UGC5459                        & SDSSJ100810.08+530501.3  & 15.379(0.011) & 12.874(0.003) & XSC---10081007+5305005  & 10.443(0.028) &  9.986(0.043) &  9.652(0.049) \\
75  & MCG5-24-022                    & SDSSJ101003.38+320412.8  & 16.206(0.008) & 13.834(0.002) & PSC---10100336+3204129  & 12.953(0.039) &  12.01(NA)    & 11.672(NA)    \\
76  & IC2551                         & SDSSJ101040.31+242450.9  & 15.621(0.005) & 13.750(0.002) & XSC---10104029+2424510  & 11.700(0.025) & 11.078(0.032) & 10.744(0.038) \\
77  & IRAS10106+2745                 & SDSSJ101329.48+273040.0  & 18.927(0.042) & 15.954(0.004) & XSC---10132945+2730402  & 13.307(0.052) & 12.538(0.059) & 11.957(0.058) \\
78  & NGC3162                        & SDSSJ101331.58+224415.1  & 13.768(0.003) & 12.110(0.002) & XSC---10133157+2244152  & 10.210(0.018) &  9.618(0.020) &  9.472(0.035) \\
79  & IRAS10120+1653                 & SDSSJ101447.90+163850.1  & 20.035(0.080) & 17.538(0.008) & XSC---10144793+1638499  & 15.364(0.109) & 14.458(0.131) & 13.459(0.127) \\
80  & NGC3190                        & SDSSJ101805.67+214956.2  & 13.948(0.003) & 11.051(0.001) & XSC---10180564+2149549  &  8.504(0.017) &  7.767(0.017) &  7.457(0.019) \\
81  & IC602                          & SDSSJ101819.70+070257.7  & 14.850(0.004) & 13.138(0.002) & XSC---10181970+0702571  & 11.388(0.028) & 10.842(0.037) & 10.554(0.050) \\
82  & NGC3191                        & SDSSJ101905.12+462714.6  & 15.959(0.008) & 13.998(0.002) & XSC---10190493+4627121  & 12.077(0.033) & 11.390(0.047) & 11.153(0.047) \\
83  & NGC3206                        & SDSSJ102147.59+565549.5  & 14.720(0.005) & 13.136(0.002) & XSC---10214758+5655494  & 11.876(0.039) & 11.379(0.055) & 11.152(0.064) \\
84  & UGC5613                        & SDSSJ102332.52+522031.3  & 16.170(0.011) & 14.018(0.002) & XSC---10233258+5220308  & 12.033(0.031) & 11.244(0.030) & 10.813(0.037) \\
85  & UGC5644                        & SDSSJ102546.26+134300.6  & 16.738(0.013) & 13.661(0.002) & XSC---10254628+1343007  & 11.550(0.026) & 10.835(0.031) & 10.626(0.038) \\
86  & NGC3245                        & SDSSJ102718.40+283026.7  & 13.585(0.003) & 10.751(0.001) & XSC---10271836+2830267  &  8.793(0.006) &  8.102(0.007) &  7.862(0.010) \\
87  & IRAS10246+2042                 & SDSSJ102725.86+202651.3  & 15.810(0.006) & 13.899(0.002) & XSC---10272584+2026510  & 11.921(0.019) & 11.279(0.024) & 11.010(0.034) \\
88  & MCG7-22-012                    & SDSSJ103011.28+432139.5  & 16.739(0.014) & 14.507(0.003) & XSC---10301140+4321397  & 12.194(0.031) & 11.345(0.031) & 10.924(0.037) \\
89  & IRAS10276+1119                 & SDSSJ103014.76+110415.8  & 16.907(0.011) & 15.218(0.003) & XSC---10301478+1104154  & 13.461(0.072) & 12.724(0.084) & 12.200(0.093) \\
90  & NGC3265                        & SDSSJ103106.76+284747.9  & 14.940(0.004) & 13.123(0.002) & XSC---10310676+2847470  & 11.374(0.021) & 10.681(0.022) & 10.439(0.029) \\
91  & UGC5713                        & SDSSJ103138.89+255902.1  & 16.214(0.009) & 13.425(0.002) & XSC---10313885+2559023  & 11.549(0.020) & 10.821(0.019) & 10.558(0.028) \\
92  & NGC3274                        & SDSSJ103217.21+274007.7  & 14.063(0.005) & 12.780(0.002) & XSC---10321728+2740075  & 11.568(0.029) & 11.025(0.038) & 10.742(0.054) \\
93  & UGC5720                        & SDSSJ103231.89+542403.4  & 14.119(0.003) & 12.874(0.002) & XSC---10323195+5424035  & 11.407(0.028) & 10.704(0.035) & 10.429(0.040) \\
94  & KUG1031+351                    & SDSSJ103402.40+345210.2  & 15.727(0.006) & 14.398(0.002) & XSC---10340239+3452104  & 12.251(0.032) & 11.709(0.044) & 11.106(0.037) \\
95  & NGC3306                        & SDSSJ103710.21+123909.2  & 15.456(0.005) & 13.306(0.002) & XSC---10371021+1239087  & 11.407(0.022) & 10.710(0.029) & 10.412(0.032) \\
96  & NGC3323                        & SDSSJ103939.03+251921.8  & 15.375(0.006) & 13.838(0.002) & XSC---10393902+2519214  & 12.246(0.051) & 11.732(0.058) & 11.299(0.064) \\
97  & IC2598                         & SDSSJ103942.36+264338.8  & 16.309(0.007) & 14.393(0.003) & XSC---10394233+2643394  & 12.259(0.027) & 11.483(0.029) & 11.050(0.031) \\
98  & NGC3338                        & SDSSJ104207.53+134449.1  & 14.466(0.005) & 12.084(0.002) & XSC---10420754+1344489  &  9.110(0.028) &  8.397(0.035) &  8.131(0.040) \\
99  & NGC3353                        & SDSSJ104522.03+555740.0  & 14.598(0.004) & 14.066(0.002) & XSC---10452239+5557373  & 11.381(0.025) & 10.712(0.033) & 10.613(0.046) \\
100 & UGC5881                        & SDSSJ104642.51+255553.5  & 16.019(0.007) & 13.618(0.002) & XSC---10464247+2555540  & 11.635(0.029) & 10.987(0.036) & 10.769(0.047) \\
101 & NGC3370                        & SDSSJ104704.05+171625.0  & 14.317(0.004) & 12.107(0.002) & XSC---10470403+1716253  & 10.352(0.020) &  9.667(0.023) &  9.426(0.030) \\
102 & NGC3381                        & SDSSJ104824.81+344241.0  & 14.102(0.004) & 12.623(0.002) & XSC---10482482+3442405  & 11.379(0.039) & 10.632(0.041) & 10.319(0.048) \\
103 & UGC5941\_NED02                 & SDSSJ105021.59+412750.5  & 15.929(0.006) & 13.743(0.002) & XSC---10502157+4127501  & 11.758(0.023) & 10.972(0.027) & 10.667(0.035) \\
104 & NGC3413                        & SDSSJ105120.73+324558.9  & 14.242(0.003) & 12.805(0.002) & XSC---10512070+3245589  & 11.387(0.018) & 10.835(0.025) & 10.729(0.040) \\
105 & NGC3408                        & SDSSJ105211.67+582617.1  & 15.841(0.008) & 13.774(0.002) & XSC---10521167+5826168  & 11.831(0.033) & 11.197(0.048) & 10.773(0.045) \\
106 & NGC3430                        & SDSSJ105211.40+325701.4  & 14.231(0.004) & 11.860(0.002) & XSC---10521141+3257015  &  9.813(0.014) &  9.143(0.016) &  8.896(0.022) \\
107 & CGCG95-055                     & SDSSJ105250.74+165907.5  & 17.033(0.019) & 14.482(0.002) & XSC---10525072+1659070  & 12.597(0.033) & 11.798(0.040) & 11.478(0.054) \\
108 & IRAS10565+2448W                & SDSSJ105918.12+243234.7  & 17.195(0.014) & 14.888(0.002) & XSC---10591815+2432343  & 12.388(0.038) & 11.678(0.047) & 11.294(0.052) \\
109 & UGC6074                        & SDSSJ105958.25+505410.7  & 19.587(0.040) & 16.578(0.004) & XSC---10595821+5054110  & 11.552(0.022) & 10.892(0.033) & 10.574(0.037) \\
110 & NGC3495                        & SDSSJ110116.22+033740.7  & 14.537(0.006) & 12.248(0.002) & XSC---11011616+0337409  &  9.887(0.013) &  9.242(0.016) &  8.931(0.022) \\
111 & UGC6103                        & SDSSJ110158.99+451340.9  & 15.030(0.004) & 13.485(0.002) & XSC---11015898+4513406  & 11.789(0.023) & 11.086(0.029) & 10.746(0.034) \\
112 & MCG7-23-019                    & SDSSJ110354.31+405100.1  & 16.932(0.009) & 15.393(0.003) & XSC---11035389+4050598  & 12.578(0.033) & 11.809(0.041) & 11.431(0.043) \\
113 & UGC6135                        & SDSSJ110436.95+450730.7  & 14.791(0.005) & 12.702(0.002) & XSC---11043695+4507309  & 10.957(0.017) & 10.270(0.021) &  9.992(0.025) \\
114 & CGCG241-078                    & SDSSJ110637.35+460219.6  & 17.309(0.015) & 14.868(0.002) & XSC---11063730+4602196  & 12.707(0.031) & 11.883(0.035) & 11.541(0.039) \\
115 & IRAS11069+2711                 & SDSSJ110938.88+265455.8  & 18.601(0.036) & 16.594(0.006) & XSC---11093889+2654563  & 15.006(0.097) & 14.191(0.101) & 13.851(0.139) \\
116 & IC676                          & SDSSJ111239.80+090321.0  & 14.602(0.005) & 12.615(0.002) & XSC---11123981+0903206  & 10.686(0.027) &  9.953(0.029) &  9.699(0.048) \\
117 & IRAS11102+3026                 & SDSSJ111257.49+301028.3  & 17.861(0.018) & 15.279(0.003) & XSC---11125751+3010283  & 13.139(0.042) & 12.451(0.054) & 12.099(0.063) \\
118 & IC2637                         & SDSSJ111349.74+093510.7  & 15.290(0.005) & 13.387(0.002) & XSC---11134972+0935106  & 11.531(0.032) & 10.806(0.034) & 10.453(0.050) \\
119 & MCG9-19-013                    & SDSSJ111449.36+501922.7  & 18.144(0.036) & 15.551(0.003) & XSC---11144937+5019228  & 13.501(0.059) & 12.771(0.079) & 12.217(0.073) \\
120 & 7ZW384                         & SDSSJ111653.96+593146.8  & 17.184(0.009) & 15.903(0.003) & XSC---11165402+5931468  & 13.610(0.066) & 12.903(0.106) & 12.332(0.074) \\
121 & 2MASXJ11193404+5335181         & SDSSJ111934.00+533518.5  & 17.970(0.019) & 15.914(0.003) & XSC---11193404+5335181  & 13.811(0.061) & 12.902(0.065) & 12.202(0.052) \\
122 & NGC3633                        & SDSSJ112026.21+033508.3  & 15.887(0.007) & 13.246(0.002) & XSC---11202621+0335077  & 10.969(0.019) & 10.207(0.018) &  9.869(0.027) \\
123 & NGC3652                        & SDSSJ112239.02+374554.4  & 14.599(0.005) & 13.075(0.002) & XSC---11223905+3745541  & 11.732(0.051) & 10.951(0.062) & 10.460(0.065) \\
124 & NGC3656                        & SDSSJ112338.64+535031.6  & 15.496(0.010) & 12.437(0.002) & XSC---11233859+5350313  & 10.302(0.019) &  9.586(0.026) &  9.275(0.027) \\
125 & NGC3659                        & SDSSJ112345.53+174907.1  & 14.211(0.004) & 12.640(0.002) & XSC---11234549+1749068  & 11.059(0.018) & 10.520(0.031) & 10.281(0.034) \\
126 & NGC3664                        & SDSSJ112424.24+031930.3  & 15.632(0.013) & 14.117(0.005) & XSC---11242425+0319299  & 13.076(0.078) & 12.527(0.098) & 12.323(0.168) \\
127 & NGC3666                        & SDSSJ112426.06+112031.9  & 14.299(0.004) & 12.116(0.002) & XSC---11242608+1120312  & 10.172(0.019) &  9.474(0.018) &  9.228(0.030) \\
128 & IC691                          & SDSSJ112644.31+590919.5  & 15.049(0.004) & 13.605(0.002) & XSC---11264427+5909197  & 11.918(0.028) & 11.270(0.041) & 10.859(0.039) \\
129 & NGC3686                        & SDSSJ112743.96+171327.0  & 13.774(0.004) & 12.024(0.002) & XSC---11274394+1713266  &  9.442(0.008) &  8.688(0.012) &  8.488(0.013) \\
130 & UGC6469                        & SDSSJ112817.70+023914.2  & 15.500(0.008) & 13.913(0.002) & XSC---11281767+0239141  & 12.081(0.035) & 11.523(0.041) & 11.276(0.069) \\
131 & NGC3690                        & SDSSJ112830.65+583348.5  & 14.395(0.003) & 13.466(0.002) & XSC---11283132+5833417  &  9.628(0.022) &  8.847(0.026) &  8.422(0.024) \\
132 & IC698                          & SDSSJ112903.83+090643.4  & 15.868(0.006) & 13.617(0.002) & XSC---11290382+0906439  & 11.343(0.026) & 10.553(0.025) & 10.168(0.036) \\
133 & IRAS11267+1558                 & SDSSJ112924.69+154141.2  & 20.317(0.059) & 19.138(0.015) & XSC---11292484+1541431  & 15.552(0.096) & 15.036(0.000) & 14.161(0.112) \\
134 & NGC3705                        & SDSSJ113007.03+091640.7  & 14.476(0.005) & 13.134(0.007) & XSC---11300745+0916358  &  8.823(0.022) &  8.162(0.023) &  7.919(0.033) \\
135 & MCG3-29-061                    & SDSSJ113103.68+201408.2  & 16.349(0.010) & 14.156(0.002) & XSC---11310372+2014086  & 12.191(0.030) & 11.563(0.042) & 11.159(0.042) \\
136 & NGC3720                        & SDSSJ113221.59+004814.3  & 18.345(0.017) & 16.006(0.004) & XSC---11322159+0048145  & 10.897(0.025) & 10.258(0.028) &  9.919(0.041) \\
137 & NGC3729                        & SDSSJ113349.32+530731.8  & 13.800(0.004) & 11.629(0.002) & XSC---11334932+5307317  &  9.359(0.013) &  8.734(0.019) &  8.729(0.027) \\
138 & MCG10-17-019                   & SDSSJ113524.80+573859.8  & 15.999(0.007) & 13.901(0.002) & XSC---11352476+5738597  & 11.878(0.025) & 11.149(0.031) & 10.874(0.036) \\
139 & NGC3758                        & SDSSJ113628.93+213546.4  & 15.740(0.007) & 13.775(0.002) & XSC---11362932+2135454  & 11.751(0.030) & 11.002(0.037) & 10.386(0.035) \\
140 & UGC6583                        & SDSSJ113654.34+195818.1  & 15.601(0.006) & 14.022(0.002) & XSC---11365438+1958179  & 12.113(0.029) & 11.473(0.030) & 11.236(0.047) \\
141 & MCG1-30-003                    & SDSSJ113706.42+025044.1  & 18.179(0.020) & 16.703(0.005) & XSC---11370674+0250451  & 12.950(0.053) & 12.295(0.059) & 11.840(0.077) \\
142 & NGC3769                        & SDSSJ113744.10+475335.2  & 14.015(0.004) & 12.072(0.002) & XSC---11374410+4753351  & 10.110(0.018) &  9.327(0.022) &  9.198(0.027) \\
143 & NGC3773                        & SDSSJ113812.90+120643.6  & 14.429(0.005) & 12.937(0.002) & XSC---11381296+1206429  & 11.504(0.034) & 11.119(0.053) & 10.696(0.063) \\
144 & NGC3781                        & SDSSJ113903.77+262142.2  & 16.217(0.008) & 13.603(0.002) & XSC---11390377+2621419  & 11.600(0.023) & 10.889(0.025) & 10.491(0.025) \\
145 & UGC6625                        & SDSSJ113947.54+195600.2  & 15.634(0.008) & 13.636(0.002) & XSC---11394756+1955599  & 11.964(0.030) & 11.364(0.047) & 10.929(0.042) \\
146 & NGC3808\_NED02                 & SDSSJ114044.47+222646.9  & 16.310(0.008) & 14.703(0.002) & XSC---11404456+2226479  & 12.407(0.042) & 11.647(0.032) & 11.365(0.043) \\
147 & NGC3811                        & SDSSJ114116.62+474126.9  & 14.998(0.005) & 12.581(0.002) & XSC---11411665+4741266  & 10.630(0.018) & 10.002(0.022) &  9.698(0.030) \\
148 & NGC3822                        & SDSSJ114211.10+101640.0  & 15.077(0.006) & 12.724(0.002) & XSC---11421107+1016398  & 10.728(0.020) &  9.980(0.020) &  9.580(0.027) \\
149 & UGC6665                        & SDSSJ114212.25+002004.0  & 14.850(0.003) & 13.954(0.002) & XSC---11421225+0020036  & 12.295(0.031) & 11.659(0.038) & 11.339(0.054) \\
150 & MCG3-30-051                    & SDSSJ114224.49+200709.4  & 15.852(0.010) & 13.730(0.002) & XSC---11422448+2007100  & 12.000(0.025) & 11.275(0.029) & 10.997(0.039) \\
151 & NGC3839                        & SDSSJ114354.33+104704.9  & 15.024(0.005) & 13.443(0.002) & XSC---11435429+1047051  & 11.764(0.036) & 11.105(0.038) & 10.678(0.050) \\
152 & UGC6732                        & SDSSJ114533.12+585841.1  & 14.884(0.004) & 12.831(0.002) & XSC---11453317+5858408  & 11.079(0.014) & 10.421(0.015) & 10.159(0.022) \\
153 & IC730                          & SDSSJ114535.24+031354.6  & 16.355(0.008) & 13.674(0.002) & XSC---11453527+0313550  & 11.607(0.023) & 10.838(0.024) & 10.410(0.031) \\
154 & IC732\_NED01                   & SDSSJ114559.42+202649.5  & 17.471(0.019) & 14.996(0.003) & XSC---11455945+2026498  & 12.874(0.044) & 11.999(0.043) & 11.575(0.050) \\
155 & NGC3912                        & SDSSJ115004.45+262845.0  & 14.624(0.004) & 12.812(0.002) & XSC---11500444+2628443  & 10.919(0.014) & 10.183(0.019) &  9.951(0.025) \\
156 & NGC3928                        & SDSSJ115147.62+484059.3  & 13.995(0.003) & 12.226(0.002) & XSC---11514768+4840593  & 10.592(0.016) &  9.936(0.024) &  9.674(0.025) \\
157 & NGC3934                        & SDSSJ115212.57+165106.7  & 16.157(0.012) & 13.623(0.002) & XSC---11521256+1651049  & 11.608(0.025) & 10.828(0.022) & 10.461(0.025) \\
158 & UGC6865                        & SDSSJ115339.96+432739.3  & 16.879(0.019) & 13.736(0.002) & XSC---11533995+4327396  & 11.233(0.024) & 10.642(0.035) & 10.304(0.041) \\
159 & UGC6901                        & SDSSJ115538.34+430245.1  & 15.480(0.008) & 13.335(0.002) & XSC---11553833+4302453  & 11.556(0.019) & 10.896(0.022) & 10.563(0.031) \\
160 & CGCG013-010                    & SDSSJ115705.93+010731.8  & 17.383(0.015) & 14.592(0.002) & XSC---11570595+0107315  & 12.050(0.032) & 11.372(0.040) & 10.938(0.041) \\
161 & NGC3991                        & SDSSJ115731.57+322022.9  & 15.296(0.005) & 14.554(0.003) & XSC---11573046+3220030  & 11.665(0.029) & 11.047(0.036) & 10.876(0.050) \\
162 & NGC4004                        & SDSSJ115805.22+275244.0  & 14.671(0.004) & 13.316(0.002) & XSC---11580522+2752441  & 11.667(0.022) & 11.013(0.027) & 10.743(0.040) \\
163 & NGC4014                        & SDSSJ115835.83+161038.1  & 15.088(0.006) & 12.424(0.002) & XSC---11583580+1610384  & 10.521(0.014) &  9.820(0.015) &  9.513(0.018) \\
164 & NGC4010                        & SDSSJ115838.14+471539.5  & 20.070(0.053) & 20.695(0.063) & XSC---11583799+4715407  & 10.671(0.011) &  9.877(0.011) &  9.591(0.017) \\
165 & NGC4018                        & SDSSJ115840.76+251858.8  & 15.862(0.013) & 13.854(0.003) & XSC---11584070+2518591  & 11.799(0.023) & 10.961(0.023) & 10.553(0.028) \\
166 & NGC4020                        & SDSSJ115856.67+302442.7  & 14.175(0.012) & 12.449(0.002) & XSC---11585693+3024490  & 11.589(0.014) & 10.982(0.019) & 10.761(0.028) \\
167 & IRAS11571+3003                 & SDSSJ115942.60+294712.4  & 18.167(0.041) & 15.779(0.003) & XSC---11594259+2947129  & 13.651(0.061) & 12.914(0.073) & 12.659(0.105) \\
168 & UGC7017                        & SDSSJ120222.52+295142.3  & 15.388(0.005) & 13.466(0.002) & XSC---12022253+2951420  & 11.539(0.019) & 10.763(0.018) & 10.434(0.025) \\
169 & UGC7016                        & SDSSJ120223.97+145037.1  & 15.920(0.008) & 13.285(0.002) & XSC---12022396+1450374  & 11.175(0.024) & 10.404(0.024) & 10.086(0.024) \\
170 & MCG3-31-030                    & SDSSJ120335.96+160319.9  & 15.426(0.008) & 13.915(0.005) & XSC---12033602+1603197  & 12.036(0.025) & 11.460(0.039) & 11.185(0.045) \\
171 & NGC4062                        & SDSSJ120403.82+315344.8  & 13.412(0.005) & 11.251(0.002) & XSC---12040383+3153449  &  9.134(0.008) &  8.470(0.011) &  8.213(0.012) \\
172 & NGC4064                        & SDSSJ120411.16+182636.8  & 14.469(0.006) & 11.972(0.002) & XSC---12041119+1826364  &  9.452(0.022) &  8.783(0.026) &  8.559(0.034) \\
173 & CGCG098-059                    & SDSSJ120709.55+165944.1  & 16.019(0.008) & 13.848(0.002) & XSC---12070958+1659439  & 11.810(0.028) & 11.070(0.029) & 10.682(0.030) \\
174 & NGC4116                        & SDSSJ120736.78+024132.4  & 21.082(0.137) & 19.114(0.018) & XSC---12073681+0241319  & 11.933(0.046) & 11.115(0.042) & 11.237(0.090) \\
175 & NGC4136                        & SDSSJ120917.70+295539.4  & 14.760(0.006) & 12.692(0.002) & XSC---12091770+2955393  & 10.315(0.042) &  9.609(0.050) &  9.307(0.060) \\
176 & NGC4150                        & SDSSJ121033.68+302406.0  & 13.857(0.003) & 11.464(0.002) & XSC---12103365+3024053  &  9.923(0.011) &  9.249(0.015) &  8.988(0.017) \\
177 & IRAS12086+1441                 & SDSSJ121114.37+142435.2  & 18.106(0.019) & 16.275(0.004) & XSC---12111428+1424348  & 14.343(0.074) & 13.369(0.079) & 12.875(0.081) \\
178 & NGC4162                        & SDSSJ121152.49+240725.0  & 14.698(0.005) & 12.396(0.002) & XSC---12115246+2407252  & 10.285(0.015) &  9.615(0.020) &  9.366(0.022) \\
179 & NGC4178                        & SDSSJ121246.32+105154.9  & 14.073(0.005) & 12.153(0.002) & XSC---12124644+1051575  &  9.886(0.050) &  9.371(0.069) &  9.575(0.034) \\
180 & IRAS12112+0305                 & SDSSJ121346.10+024841.4  & 18.452(0.031) & 16.589(0.005) & XSC---12134598+0248399  & 14.036(0.105) & 13.273(0.108) & 12.782(0.150) \\
181 & NGC4189                        & SDSSJ121347.26+132529.2  & 14.935(0.008) & 12.724(0.002) & XSC---12134727+1325294  &  9.948(0.028) &  9.330(0.040) &  8.914(0.043) \\
182 & NGC4194                        & SDSSJ121409.61+543135.9  & 14.445(0.003) & 13.234(0.002) & XSC---12140957+5431360  & 10.630(0.016) &  9.934(0.017) &  9.626(0.022) \\
183 & NGC4204                        & SDSSJ121514.43+203930.9  & 14.647(0.007) & 13.097(0.003) & XSC---12151435+2039326  & 12.255(0.048) & 12.358(0.045) & 11.843(0.094) \\
184 & NGC4207                        & SDSSJ121530.50+093505.5  & 14.762(0.005) & 12.477(0.002) & XSC---12153043+0935057  & 10.485(0.020) &  9.759(0.022) &  9.442(0.032) \\
185 & UGC7286                        & SDSSJ121559.24+272631.9  & 17.059(0.015) & 14.347(0.002) & XSC---12155920+2726317  & 12.097(0.030) & 11.297(0.034) & 11.048(0.037) \\
186 & NGC4234                        & SDSSJ121709.14+034059.2  & 14.528(0.006) & 12.928(0.002) & XSC---12170789+0340563  & 12.053(0.027) & 11.513(0.045) & 11.184(0.049) \\
187 & NGC4237                        & SDSSJ121711.41+151926.3  & 13.796(0.004) & 11.576(0.002) & XSC---12171141+1519262  &  9.568(0.011) &  8.849(0.014) &  8.608(0.018) \\
188 & NGC4244                        & SDSSJ121729.43+374826.4  & 12.882(0.003) & 11.145(0.002) & XSC---12172965+3748255  &  8.564(0.027) &  7.978(0.033) &  7.724(0.046) \\
189 & NGC4253                        & SDSSJ121826.51+294846.4  & 14.898(0.004) & 12.934(0.002) & XSC---12182648+2948461  & 11.101(0.021) & 10.379(0.027) &  9.839(0.022) \\
190 & MCG3-32-005                    & SDSSJ122047.23+170057.6  & 16.173(0.009) & 14.144(0.003) & XSC---12204725+1700571  & 12.165(0.027) & 11.405(0.030) & 11.129(0.041) \\
191 & NGC4290                        & SDSSJ122047.51+580533.0  & 14.630(0.005) & 12.367(0.002) & XSC---12204750+5805325  & 10.263(0.019) &  9.592(0.022) &  9.297(0.030) \\
192 & NGC4294                        & SDSSJ122117.83+113037.3  & 13.257(0.003) & 11.965(0.003) & XSC---12211778+1130399  & 10.580(0.044) & 10.189(0.061) &  9.699(0.073) \\
193 & NGC4314                        & SDSSJ122232.01+295343.7  & 13.488(0.003) & 10.906(0.001) & XSC---12223197+2953430  &  8.517(0.012) &  7.825(0.017) &  7.559(0.015) \\
194 & NGC4385                        & SDSSJ122542.80+003421.4  & 14.578(0.004) & 12.666(0.002) & XSC---12254281+0034213  & 10.645(0.026) & 10.016(0.028) &  9.776(0.046) \\
195 & NGC4395                        & SDSSJ122548.86+333248.7  & 15.356(0.012) & 13.732(0.003) & XSC---12254892+3332482  & 10.660(0.031) & 10.246(0.045) &  9.976(0.058) \\
196 & NGC4396                        & NA                       &     NA(NA)    &     NA(NA)    & XSC---12255880+1540172  & 11.060(0.048) & 10.455(0.066) & 10.336(0.081) \\
197 & NGC4412                        & SDSSJ122636.07+035752.9  & 14.436(0.005) & 12.463(0.002) & XSC---12263610+0357526  & 10.755(0.038) & 10.171(0.039) &  9.652(0.052) \\
198 & NGC4418                        & SDSSJ122654.61-005239.3  & 15.083(0.005) & 12.637(0.002) & XSC---12265462-0052395  & 11.043(0.021) & 10.354(0.025) & 10.117(0.045) \\
199 & NGC4420                        & SDSSJ122658.50+022939.4  & 13.724(0.003) & 12.011(0.003) & XSC---12265847+0229396  & 10.514(0.023) &  9.885(0.023) &  9.659(0.039) \\
200 & NGC4424                        & SDSSJ122711.75+092512.7  & 19.493(0.051) & 19.035(0.022) & XSC---12271158+0925138  &  9.867(0.024) &  9.268(0.028) &  9.091(0.043) \\
201 & NGC4435                        & SDSSJ122740.47+130444.4  & 14.579(0.005) & 10.351(0.001) & XSC---12274050+1304444  &  8.421(0.013) &  7.159(0.010) &  7.297(0.016) \\
202 & NGC4438                        & NA                       &     NA(NA)    &     NA(NA)    & XSC---12274565+1300309  &  8.247(0.018) &  7.556(0.020) &  7.265(0.023) \\
203 & NGC4448                        & SDSSJ122815.45+283713.1  & 13.883(0.003) & 11.151(0.002) & XSC---12281542+2837130  &  8.731(0.017) &  8.056(0.019) &  7.813(0.019) \\
204 & 3C273                          & SDSSJ122906.70+020308.6  & 13.993(0.005) & 12.880(0.002) & XSC---12290674+0203083  & 11.692(0.023) & 10.953(0.023) &  9.937(0.020) \\
205 & NGC4470                        & SDSSJ122937.77+074926.7  & 13.884(0.004) & 12.460(0.002) & XSC---12293780+0749266  & 10.877(0.027) & 10.300(0.037) & 10.123(0.052) \\
206 & IRAS12274+0018                 & SDSSJ122958.84+000138.0  & 18.140(0.019) & 15.676(0.003) & XSC---12295883+0001379  & 13.553(0.083) & 12.801(0.088) & 12.200(0.103) \\
207 & NGC4491                        & SDSSJ123057.11+112900.6  & 14.728(0.005) & 12.599(0.002) & XSC---12305713+1129007  & 10.695(0.031) & 10.060(0.039) &  9.878(0.054) \\
208 & NGC4500                        & SDSSJ123122.20+575752.1  & 14.611(0.004) & 12.776(0.002) & XSC---12312214+5757528  & 10.674(0.015) & 10.062(0.020) &  9.745(0.022) \\
209 & NGC4495                        & SDSSJ123122.88+290811.3  & 15.136(0.007) & 12.901(0.002) & XSC---12312290+2908109  & 11.283(0.022) & 10.508(0.028) & 10.143(0.028) \\
210 & IC3476                         & SDSSJ123241.88+140301.5  & 14.569(0.005) & 13.146(0.006) & XSC---12324174+1403058  & 11.752(0.051) & 11.401(0.082) & 10.910(0.075) \\
211 & NGC4509                        & SDSSJ123306.72+320534.4  & 15.520(0.007) & 14.763(0.008) & XSC---12330650+3205273  & 13.506(0.088) & 12.693(0.079) & 12.707(0.144) \\
212 & NGC4519                        & SDSSJ123330.25+083917.0  & 14.270(0.005) & 12.379(0.002) & XSC---12333027+0839160  & 10.517(0.037) &  9.946(0.049) &  9.555(0.059) \\
213 & NGC4548                        & NA                       &     NA(NA)    &     NA(NA)    & XSC---12352642+1429467  &  8.010(0.022) &  7.373(0.028) &  7.115(0.031) \\
214 & IRAS12337+5044                 & SDSSJ123606.82+502813.4  & 16.911(0.010) & 15.388(0.003) & XSC---12360677+5028181  & 13.351(0.051) & 12.621(0.064) & 12.177(0.072) \\
215 & IC3581                         & SDSSJ123638.06+242543.6  & 15.906(0.007) & 13.727(0.002) & XSC---12363799+2425429  & 11.822(0.023) & 11.116(0.031) & 10.728(0.027) \\
216 & NGC4592                        & SDSSJ123918.73-003155.0  & 13.422(0.003) & 11.944(0.002) & XSC---12391877-0031546  & 11.004(0.014) & 10.401(0.018) & 10.218(0.031) \\
217 & NGC4607                        & SDSSJ124112.18+115312.7  & 22.810(0.596) & 19.557(0.026) & XSC---12411240+1153118  & 10.751(0.015) &  9.953(0.016) &  9.584(0.022) \\
218 & NGC4625                        & SDSSJ124152.71+411626.2  & 14.146(0.004) & 12.453(0.002) & XSC---12415270+4116253  & 10.651(0.032) &  9.931(0.038) &  9.745(0.052) \\
219 & NGC4630                        & SDSSJ124231.12+035737.0  & 13.801(0.005) & 12.539(0.002) & XSC---12423114+0357372  & 10.752(0.036) & 10.209(0.049) &  9.886(0.065) \\
220 & IC3690                         & SDSSJ124249.19+102126.8  & 16.825(0.017) & 14.465(0.002) & XSC---12424923+1021268  & 12.483(0.048) & 11.749(0.050) & 11.255(0.065) \\
221 & UGC7905\_NED01                 & SDSSJ124347.94+545345.4  & 15.282(0.005) & 14.130(0.002) & XSC---12434789+5453461  & 12.677(0.030) & 11.888(0.034) & 11.691(0.052) \\
222 & MCG5-30-069                    & SDSSJ124441.25+262510.5  & 16.464(0.010) & 13.970(0.002) & XSC---12444123+2625109  & 11.996(0.028) & 11.415(0.038) & 11.002(0.038) \\
223 & IC3721                         & SDSSJ124453.11+184518.8  & 15.734(0.007) & 13.402(0.002) & XSC---12445314+1845182  & 11.378(0.022) & 10.626(0.026) & 10.312(0.028) \\
224 & NGC4670                        & SDSSJ124517.25+270732.1  & 13.322(0.002) & 12.397(0.002) & XSC---12451714+2707317  & 11.306(0.022) & 10.743(0.034) & 10.407(0.043) \\
225 & NGC4675                        & SDSSJ124531.88+544415.3  & 16.504(0.014) & 13.740(0.002) & XSC---12453191+5444151  & 11.705(0.025) & 10.936(0.025) & 10.638(0.035) \\
226 & MCG7-26-051                    & SDSSJ124656.84+421559.1  & 18.209(0.035) & 15.290(0.003) & XSC---12465672+4215595  & 12.462(0.040) & 11.544(0.039) & 10.974(0.037) \\
227 & NGC4689                        & SDSSJ124745.56+134546.1  & 14.991(0.008) & 12.690(0.002) & XSC---12474552+1345456  &  8.762(0.027) &  8.058(0.038) &  7.961(0.047) \\
228 & NGC4688                        & SDSSJ124746.52+042009.6  & 15.790(0.011) & 13.934(0.003) & XSC---12474646+0420098  & 12.328(0.085) & 11.324(0.062) & 11.161(0.103) \\
229 & NGC4704                        & SDSSJ124846.42+415516.5  & 16.035(0.013) & 13.446(0.002) & XSC---12484638+4155166  & 11.819(0.040) & 11.123(0.057) & 10.689(0.053) \\
230 & NGC4701                        & SDSSJ124911.58+032319.3  & 14.290(0.004) & 12.577(0.002) & XSC---12491156+0323194  & 10.714(0.027) & 10.065(0.028) &  9.766(0.043) \\
231 & IRAS12468+3436                 & SDSSJ124917.17+341942.9  & 20.404(0.086) & 17.770(0.007) & XSC---12491718+3419432  & 15.491(0.123) & 14.927(0.178) & 14.018(0.125) \\
232 & IRAS12470+1404                 & SDSSJ124934.79+134809.8  & 17.060(0.011) & 15.865(0.003) & XSC---12493477+1348095  & 14.269(0.078) & 13.535(0.110) & 13.298(0.120) \\
233 & MCG8-23-097                    & SDSSJ125039.83+475600.3  & 18.059(0.027) & 14.636(0.002) & XSC---12503981+4756010  & 12.184(0.033) & 11.426(0.038) & 10.951(0.045) \\
234 & NGC4747                        & SDSSJ125145.05+254628.2  & 23.620(0.864) & 21.250(0.067) & XSC---12514596+2546383  & 10.938(0.034) & 10.181(0.045) & 10.285(0.028) \\
235 & UGC8017                        & SDSSJ125253.58+282216.5  & 15.967(0.008) & 13.574(0.002) & XSC---12525355+2822160  & 11.407(0.020) & 10.587(0.024) & 10.252(0.028) \\
236 & NGC4765                        & SDSSJ125314.55+042747.7  & 14.288(0.014) & 12.979(0.002) & XSC---12531456+0427479  & 11.637(0.031) & 10.978(0.037) & 10.824(0.060) \\
237 & VCC2096                        & SDSSJ125325.00+114234.3  & 16.949(0.015) & 15.415(0.003) & XSC---12532472+1142397  & 13.591(0.062) & 12.860(0.074) & 12.576(0.097) \\
238 & UGC8041                        & SDSSJ125512.65+000659.9  & 15.714(0.012) & 13.470(0.002) & XSC---12551268+0007000  & 12.436(0.043) & 11.720(0.053) & 11.984(0.125) \\
239 & UGC8058                        & SDSSJ125614.22+565225.2  & 15.079(0.004) & 13.501(0.005) & XSC---12561432+5652244  & 11.024(0.020) &  9.889(0.019) &  8.813(0.017) \\
240 & NGC4837\_NED01                 & SDSSJ125648.31+481749.0  & 16.688(0.014) & 13.929(0.002) & XSC---12564828+4817485  & 11.585(0.033) & 10.875(0.117) & 10.521(0.030) \\
241 & UM530                          & SDSSJ125808.34+015144.4  & 16.976(0.010) & 16.154(0.004) & XSC---12580832+0151442  & 14.680(0.153) & 13.813(0.146) & 13.175(0.157) \\
242 & NGC4861                        & SDSSJ125900.27+345044.8  & 15.542(0.006) & 15.252(0.003) & XSC---12590028+3450440  & 13.390(0.047) & 13.215(0.086) & 12.541(0.077) \\
243 & NGC4868                        & SDSSJ125908.88+371837.4  & 14.457(0.006) & 12.041(0.002) & XSC---12590891+3718370  & 10.453(0.015) &  9.763(0.017) &  9.513(0.021) \\
244 & NGC4922\_NED02                 & SDSSJ130125.26+291849.5  & 16.259(0.014) & 13.936(0.002) & PSC---13012525+2918496  & 14.009(0.071) & 13.231(0.075) & 12.504(0.056) \\
245 & UGC8179                        & SDSSJ130514.15+315958.9  & 16.246(0.013) & 13.558(0.002) & XSC---13051411+3159594  & 11.911(0.033) & 11.211(0.032) & 10.755(0.037) \\
246 & NGC5001                        & SDSSJ130933.09+532939.3  & 15.956(0.007) & 13.693(0.002) & XSC---13093325+5329391  & 11.513(0.030) & 10.784(0.032) & 10.431(0.043) \\
247 & IC856                          & SDSSJ131041.25+203210.2  & 16.422(0.012) & 14.773(0.003) & XSC---13104161+2032123  & 12.154(0.028) & 11.379(0.026) & 11.032(0.029) \\
248 & UGC8269                        & SDSSJ131115.14+464202.3  & 16.924(0.032) & 14.492(0.003) & XSC---13111517+4642024  & 12.514(0.038) & 11.635(0.044) & 11.462(0.052) \\
249 & NGC5014                        & SDSSJ131131.23+361655.3  & 15.286(0.010) & 12.731(0.002) & XSC---13113119+3616556  & 10.972(0.015) & 10.297(0.018) & 10.110(0.024) \\
250 & NGC5012                        & SDSSJ131137.03+225455.7  & 14.416(0.005) & 12.033(0.002) & XSC---13113705+2254556  &  9.749(0.014) &  9.020(0.018) &  8.762(0.020) \\
251 & IRAS13116+4508                 & SDSSJ131347.86+445258.6  & 18.245(0.026) & 15.877(0.003) & XSC---13134784+4452589  & 13.958(0.076) & 13.215(0.104) & 12.582(0.080) \\
252 & IC860                          & SDSSJ131503.51+243707.7  & 15.684(0.011) & 13.386(0.002) & XSC---13150351+2437074  & 11.563(0.018) & 10.810(0.020) & 10.592(0.028) \\
253 & IRAS13144+4508                 & SDSSJ131639.74+445235.0  & 16.724(0.009) & 15.535(0.003) & XSC---13163979+4452351  & 13.839(0.076) & 12.867(0.085) & 11.657(0.037) \\
254 & NGC5060                        & SDSSJ131716.21+060214.8  & 15.339(0.009) & 12.873(0.002) & XSC---13171622+0602149  & 11.455(0.028) & 10.637(0.029) & 10.315(0.042) \\
255 & UGC8357\_NED01                 & SDSSJ131758.79-001841.9  & 16.032(0.007) & 14.165(0.002) & XSC---13175881-0018422  & 12.022(0.030) & 11.287(0.034) & 11.012(0.054) \\
256 & UGC8361                        & SDSSJ131818.58+062007.3  & 16.263(0.009) & 13.896(0.002) & XSC---13181859+0620069  & 11.904(0.035) & 11.116(0.037) & 10.713(0.047) \\
257 & IC883                          & SDSSJ132035.40+340821.7  & 15.796(0.017) & 13.851(0.003) & XSC---13203537+3408218  & 11.993(0.023) & 11.227(0.025) & 10.929(0.033) \\
258 & NGC5100\_NED02                 & SDSSJ132059.58+085841.8  & 15.763(0.009) & 13.492(0.002) & XSC---13205961+0858421  & 11.551(0.027) & 10.782(0.028) & 10.414(0.040) \\
259 & NGC5104                        & SDSSJ132123.07+002032.7  & 15.816(0.010) & 13.160(0.002) & XSC---13212311+0020333  & 10.870(0.030) & 10.148(0.036) &  9.744(0.028) \\
260 & NGC5107                        & SDSSJ132124.26+383218.5  & 21.866(0.203) & 20.630(0.045) & XSC---13212526+3832109  & 12.187(0.034) & 11.738(0.053) & 11.486(0.068) \\
261 & NGC5112                        & SDSSJ132156.41+384405.0  & 14.015(0.005) & 12.259(0.003) & XSC---13215650+3844042  & 10.871(0.031) & 10.287(0.039) & 10.016(0.054) \\
262 & NGC5123                        & SDSSJ132310.52+430510.5  & 14.969(0.006) & 12.709(0.002) & XSC---13231050+4305108  & 11.091(0.028) & 10.385(0.028) & 10.051(0.038) \\
263 & IRAS13218+0552                 & SDSSJ132419.88+053704.6  & 18.719(0.025) & 17.553(0.006) & XSC---13241989+0537048  & 15.178(0.234) & 13.915(0.152) & 12.055(0.054) \\
264 & IRAS13232+1731                 & SDSSJ132543.85+171552.7  & 16.591(0.011) & 15.011(0.003) & XSC---13254389+1715529  & 13.005(0.037) & 12.404(0.056) & 11.872(0.055) \\
265 & NGC5147                        & SDSSJ132619.70+020602.6  & 20.061(0.064) & 17.970(0.008) & XSC---13261970+0206027  & 10.567(0.037) &  9.907(0.041) &  9.725(0.062) \\
266 & NGC5204                        & SDSSJ132936.33+582510.4  & 12.764(0.003) & 11.424(0.002) & XSC---13293650+5825074  & 10.237(0.034) &  9.642(0.050) &  9.507(0.059) \\
267 & UGC8502\_NED02                 & SDSSJ133039.36+311658.3  & 17.373(0.015) & 15.792(0.003) & PSC---13303941+3117029  & 15.392(0.104) & 14.756(0.123) & 13.436(NA)    \\
268 & UGC8561                        & SDSSJ133457.27+340238.7  & 15.307(0.006) & 13.205(0.002) & XSC---13345720+3402384  & 11.492(0.027) & 10.940(0.037) & 10.637(0.040) \\
269 & NGC5230                        & SDSSJ133531.87+134034.1  & 14.877(0.006) & 12.743(0.002) & XSC---13353188+1340344  & 10.590(0.028) &  9.800(0.034) &  9.827(0.052) \\
270 & IRAS13349+2438                 & SDSSJ133718.72+242303.3  & 15.834(0.007) & 14.427(0.004) & XSC---13371873+2423029  & 12.671(0.030) & 11.664(0.033) & 10.449(0.020) \\
271 & NGC5256                        & SDSSJ133816.86+481638.5  & 20.687(0.069) & 19.815(0.024) & XSC---13381728+4816319  & 11.271(0.046) & 10.523(0.061) &  9.799(0.046) \\
272 & UGC8626                        & SDSSJ133823.47+065315.5  & 16.192(0.011) & 13.794(0.002) & XSC---13382344+0653149  & 11.996(0.040) & 11.245(0.044) & 10.891(0.058) \\
273 & NGC5263                        & SDSSJ133955.65+282402.8  & 15.680(0.009) & 13.506(0.002) & XSC---13395563+2824020  & 11.228(0.022) & 10.518(0.030) & 10.168(0.030) \\
274 & MCG1-35-028                    & SDSSJ134027.18+044625.6  & 15.958(0.008) & 13.654(0.002) & XSC---13402720+0446253  & 11.899(0.039) & 11.123(0.035) & 10.791(0.049) \\
275 & IC910                          & SDSSJ134107.85+231655.4  & 16.037(0.008) & 13.986(0.002) & XSC---13410784+2316550  & 12.168(0.034) & 11.502(0.037) & 11.159(0.057) \\
276 & MK268                          & SDSSJ134111.14+302241.3  & 16.208(0.008) & 13.882(0.002) & XSC---13411117+3022411  & 11.778(0.026) & 11.157(0.027) & 10.879(0.034) \\
277 & NGC5278                        & SDSSJ134139.62+554014.3  & 15.911(0.008) & 13.422(0.002) & XSC---13413961+5540146  & 11.250(0.023) & 10.636(0.027) & 10.271(0.032) \\
278 & NGC5273                        & SDSSJ134208.38+353915.5  & 14.051(0.004) & 11.622(0.002) & XSC---13420838+3539152  &  9.501(0.013) &  8.837(0.016) &  8.665(0.024) \\
279 & UGC8685                        & SDSSJ134308.83+302015.8  & 15.833(0.009) & 13.521(0.002) & XSC---13430886+3020153  & 11.917(0.024) & 11.237(0.031) & 10.872(0.039) \\
280 & UGC8686                        & SDSSJ134340.13+035347.2  & 15.859(0.009) & 13.774(0.002) & XSC---13434013+0353468  & 11.795(0.031) & 10.993(0.034) & 10.758(0.048) \\
281 & UGC8696                        & SDSSJ134442.16+555313.5  & 16.584(0.009) & 14.304(0.002) & XSC---13444207+5553131  & 12.181(0.026) & 11.417(0.031) & 10.891(0.029) \\
282 & NGC5297                        & SDSSJ134624.49+435212.1  & 21.462(0.178) & 18.350(0.010) & XSC---13462369+4352193  &  9.839(0.021) &  9.176(0.023) &  8.891(0.029) \\
283 & MK796                          & SDSSJ134649.45+142401.7  & 15.762(0.005) & 14.200(0.002) & XSC---13464948+1424020  & 12.316(0.027) & 11.514(0.032) & 11.092(0.036) \\
284 & IRAS13446+1121                 & SDSSJ134704.35+110622.5  & 16.792(0.012) & 14.402(0.002) & XSC---13470435+1106224  & 12.445(0.050) & 11.561(0.047) & 11.102(0.061) \\
285 & NGC5303                        & SDSSJ134744.98+381816.6  & 15.066(0.005) & 13.411(0.002) & XSC---13474496+3818163  & 11.098(0.016) & 10.525(0.019) & 10.227(0.026) \\
286 & NGC5313                        & SDSSJ134944.34+395905.1  & 14.423(0.004) & 11.681(0.002) & XSC---13494435+3959045  &  9.802(0.010) &  9.118(0.012) &  8.820(0.016) \\
287 & MCG3-35-034\_NED01             & SDSSJ135309.66+143920.8  & 16.382(0.012) & 14.063(0.002) & XSC---13530964+1439213  & 12.021(0.030) & 11.255(0.029) & 10.892(0.038) \\
288 & NGC5347                        & SDSSJ135317.78+332927.0  & 14.852(0.006) & 12.431(0.002) & XSC---13531785+3329267  & 10.620(0.028) &  9.977(0.038) &  9.645(0.040) \\
289 & NGC5350                        & NA                       &     NA(NA)    &     NA(NA)    & XSC---13532158+4021502  &  9.237(0.012) &  8.870(0.018) &  8.622(0.026) \\
290 & NGC5368                        & SDSSJ135429.15+541950.3  & 15.563(0.006) & 13.068(0.002) & XSC---13542914+5419507  & 11.144(0.021) & 10.461(0.023) & 10.195(0.029) \\
291 & UGC8827                        & SDSSJ135431.17+150238.8  & 15.302(0.004) & 13.239(0.002) & XSC---13543115+1502388  & 11.328(0.019) & 10.697(0.021) & 10.322(0.027) \\
292 & UGC8850                        & SDSSJ135602.89+182218.2  & 15.361(0.006) & 14.006(0.002) & PSC---13560261+1822181  & 14.203(0.101) & 13.512(0.108) & 11.093(NA)    \\
293 & UGC8856\_NED01                 & SDSSJ135607.89+300452.8  & 17.290(0.017) & 15.115(0.003) & XSC---13560826+3004553  & 12.884(0.046) & 12.065(0.059) & 11.662(0.056) \\
294 & NGC5374                        & SDSSJ135729.63+060549.3  & 14.783(0.005) & 12.863(0.002) & XSC---13572962+0605487  & 10.537(0.030) &  9.930(0.035) &  9.704(0.052) \\
295 & UGC8902                        & SDSSJ135902.80+153356.6  & 15.778(0.008) & 12.983(0.002) & XSC---13590275+1533561  & 10.924(0.017) & 10.228(0.020) &  9.949(0.030) \\
296 & NGC5403                        & SDSSJ135950.70+381055.6  & 21.769(0.200) & 18.494(0.011) & PSC---13595085+3810567  & 13.499(0.064) & 11.885(NA)    & 11.338(NA)    \\
297 & MCG7-29-036                    & SDSSJ140057.83+425120.3  & 18.050(0.028) & 15.275(0.003) & XSC---14005782+4251207  & 12.965(0.041) & 12.256(0.048) & 11.831(0.058) \\
298 & NGC5414                        & SDSSJ140203.52+095545.5  & 14.839(0.004) & 13.488(0.002) & XSC---14020351+0955458  & 11.972(0.027) & 11.373(0.035) & 11.200(0.059) \\
299 & MCG5-33-046                    & SDSSJ140447.98+304437.3  & 17.283(0.021) & 14.244(0.002) & XSC---14044805+3044377  & 11.936(0.030) & 11.178(0.033) & 10.989(0.045) \\
300 & NGC5474                        & NA                       &     NA(NA)    &     NA(NA)    & XSC---14050160+5339439  & 10.232(0.024) &  9.563(0.029) &  9.484(0.045) \\
301 & NGC5480                        & SDSSJ140621.57+504330.2  & 13.938(0.004) & 12.250(0.002) & XSC---14062152+5043299  & 10.369(0.025) &  9.738(0.029) &  9.459(0.043) \\
302 & MCG6-31-070                    & SDSSJ140649.09+334618.3  & 17.646(0.022) & 14.850(0.002) & XSC---14064909+3346181  & 12.540(0.034) & 11.558(0.038) & 11.275(0.040) \\
303 & CGCG74-129                     & SDSSJ141041.34+133328.7  & 16.757(0.015) & 14.062(0.002) & XSC---14104135+1333285  & 12.422(0.030) & 11.632(0.033) & 11.356(0.047) \\
304 & NGC5520                        & SDSSJ141222.81+502054.3  & 14.386(0.004) & 12.496(0.002) & XSC---14122277+5020543  & 10.884(0.018) & 10.254(0.019) &  9.970(0.032) \\
305 & NGC5515                        & SDSSJ141238.14+391836.5  & 15.681(0.007) & 13.117(0.002) & XSC---14123812+3918369  & 11.056(0.019) & 10.284(0.022) &  9.928(0.024) \\
306 & NGC5526\_NED02                 & SDSSJ141353.77+574616.8  & 15.369(0.008) & 13.392(0.002) & XSC---14135372+5746167  & 11.410(0.022) & 10.675(0.028) & 10.322(0.034) \\
307 & NGC5522                        & SDSSJ141450.37+150848.7  & 15.302(0.006) & 12.932(0.002) & XSC---14145036+1508480  & 10.985(0.023) & 10.262(0.029) &  9.906(0.030) \\
308 & NGC5541                        & NA                       &     NA(NA)    &     NA(NA)    & XSC---14163182+3935207  & 11.131(0.024) & 10.393(0.020) & 10.021(0.023) \\
309 & IC4395                         & SDSSJ141721.07+265126.7  & 16.183(0.009) & 14.002(0.002) & XSC---14172108+2651264  & 11.552(0.019) & 10.838(0.021) & 10.451(0.024) \\
310 & UGC9165                        & SDSSJ141847.78+245625.9  & 16.084(0.009) & 13.865(0.002) & XSC---14184786+2456255  & 11.544(0.023) & 10.721(0.021) & 10.290(0.029) \\
311 & MK1490                         & SDSSJ141943.23+491411.9  & 16.960(0.010) & 14.543(0.002) & XSC---14194323+4914121  & 12.553(0.034) & 11.722(0.037) & 11.302(0.044) \\
312 & NGC5585                        & SDSSJ141948.19+564345.6  & 14.201(0.005) & 12.455(0.002) & XSC---14194820+5643445  & 10.226(0.026) &  9.576(0.035) &  9.500(0.047) \\
313 & IC4408                         & SDSSJ142113.09+295936.6  & 16.003(0.008) & 13.734(0.002) & XSC---14211313+2959367  & 11.643(0.025) & 10.906(0.027) & 10.588(0.033) \\
314 & NGC5584                        & SDSSJ142223.77-002315.5  & 14.274(0.005) & 12.362(0.002) & XSC---14222381-0023148  & 10.835(0.021) & 10.046(0.023) &  9.949(0.067) \\
315 & NGC5633                        & SDSSJ142728.39+460847.6  & 14.171(0.003) & 12.315(0.002) & XSC---14272838+4608475  & 10.518(0.016) &  9.867(0.020) &  9.593(0.024) \\
316 & NGC5660                        & SDSSJ142949.81+493721.5  & 14.259(0.005) & 12.249(0.002) & XSC---14294980+4937214  & 10.261(0.028) &  9.544(0.032) &  9.390(0.043) \\
317 & NGC5656                        & SDSSJ143025.50+351915.7  & 14.785(0.005) & 12.377(0.002) & XSC---14302551+3519159  & 10.328(0.014) &  9.637(0.016) &  9.350(0.018) \\
318 & NGC5657                        & SDSSJ143043.59+291050.7  & 15.491(0.007) & 13.210(0.002) & XSC---14304364+2910503  & 11.344(0.020) & 10.646(0.023) & 10.376(0.029) \\
319 & CGCG133-083                    & SDSSJ143154.09+215618.3  & 16.757(0.015) & 14.726(0.003) & XSC---14315406+2156182  & 13.145(0.053) & 12.343(0.063) & 11.890(0.067) \\
320 & MCG7-30-028                    & SDSSJ143348.35+400538.9  & 15.995(0.007) & 13.996(0.002) & XSC---14334840+4005392  & 12.016(0.039) & 11.282(0.047) & 10.791(0.055) \\
321 & MCG6-32-070                    & SDSSJ143518.38+350707.4  & 15.412(0.005) & 13.674(0.002) & XSC---14351842+3507077  & 11.688(0.024) & 11.058(0.036) & 10.692(0.033) \\
322 & UGC9412                        & SDSSJ143622.08+584739.4  & 14.810(0.004) & 13.688(0.002) & XSC---14362213+5847389  & 11.784(0.023) & 10.971(0.026) & 10.346(0.022) \\
323 & NGC5698                        & SDSSJ143714.69+382715.2  & 15.274(0.008) & 13.028(0.002) & XSC---14371464+3827150  & 11.242(0.028) & 10.580(0.033) & 10.287(0.049) \\
324 & NGC5691                        & SDSSJ143753.33-002355.9  & 13.737(0.003) & 12.472(0.002) & XSC---14375333-0023559  & 10.839(0.025) & 10.137(0.029) &  9.972(0.046) \\
325 & MCG9-24-035                    & SDSSJ144545.10+513450.9  & 15.785(0.007) & 13.459(0.002) & XSC---14454510+5134509  & 11.664(0.034) & 10.861(0.034) & 10.507(0.035) \\
326 & MCG9-24-038                    & SDSSJ144637.06+561358.6  & 17.406(0.025) & 14.456(0.002) & XSC---14463700+5613590  & 12.583(0.031) & 11.820(0.036) & 11.345(0.037) \\
327 & UGC9560                        & SDSSJ145056.56+353419.5  & 15.129(0.004) & 14.612(0.002) & XSC---14505649+3534182  & 13.597(0.055) & 13.067(0.081) & 12.797(0.118) \\
328 & IC1076                         & SDSSJ145459.61+180214.4  & 15.333(0.008) & 13.633(0.002) & XSC---14545961+1802141  & 11.895(0.024) & 11.186(0.027) & 10.982(0.043) \\
329 & IRAS14538+1730                 & SDSSJ145608.53+171834.4  & 19.736(0.075) & 16.639(0.005) & XSC---14560852+1718342  & 14.166(0.099) & 13.009(0.085) & 12.414(0.070) \\
330 & NGC5795                        & SDSSJ145619.87+492401.5  & 16.472(0.015) & 14.245(0.003) & PSC---14561934+4923555  & 13.113(NA)    & 12.564(0.081) & 11.804(NA)    \\
331 & UGC9618\_NED02                 & SDSSJ145700.77+243702.2  & 18.471(0.057) & 14.668(0.003) & XSC---14570066+2437026  & 11.629(0.027) & 10.759(0.026) & 10.239(0.028) \\
332 & UGC9639                        & SDSSJ145835.99+445301.0  & 15.679(0.007) & 13.369(0.002) & XSC---14583603+4453010  & 11.563(0.026) & 10.803(0.026) & 10.495(0.030) \\
333 & MCG6-33-022                    & SDSSJ150806.01+342324.5  & 23.646(11.554) & 26.110(10.851) & PSC---15080569+3423233  & 14.172(0.082) & 12.674(NA)    & 12.149(NA)    \\
334 & NGC5879                        & SDSSJ150946.75+570000.6  & 13.910(0.004) & 11.606(0.002) & XSC---15094675+5700007  &  9.677(0.011) &  8.981(0.013) &  8.792(0.018) \\
335 & MCG9-25-036                    & SDSSJ151252.32+512355.0  & 16.319(0.010) & 14.564(0.002) & XSC---15125237+5123553  & 12.763(0.048) & 12.199(0.060) & 11.894(0.064) \\
336 & NGC5899                        & SDSSJ151503.23+420259.4  & 15.061(0.006) & 12.062(0.002) & XSC---15150325+4202594  &  9.620(0.028) &  8.990(0.029) &  8.585(0.022) \\
337 & NGC5905                        & SDSSJ151523.35+553102.2  & 14.693(0.006) & 12.236(0.002) & XSC---15152332+5531015  & 10.467(0.017) &  9.846(0.020) &  9.514(0.027) \\
338 & MK848                          & SDSSJ151806.13+424445.0  & 16.278(0.008) & 14.757(0.002) & XSC---15180612+4244445  & 12.654(0.039) & 11.933(0.049) & 11.545(0.056) \\
339 & IC4553                         & SDSSJ153457.20+233013.2  & 15.639(0.009) & 13.091(0.002) & XSC---15345727+2330104  & 11.035(0.026) & 10.306(0.028) &  9.852(0.036) \\
340 & UGC9922\_NED02                 & SDSSJ153553.89+384031.8  & 16.675(0.015) & 14.642(0.002) & XSC---15355381+3840302  & 12.385(0.039) & 11.761(0.037) & 11.402(0.098) \\
341 & IC4567                         & SDSSJ153713.26+431753.9  & 15.155(0.006) & 12.994(0.002) & XSC---15371331+4317544  & 11.021(0.019) & 10.339(0.021) & 10.015(0.030) \\
342 & MCG4-37-016                    & SDSSJ153927.50+245651.4  & 16.045(0.007) & 14.157(0.002) & XSC---15392748+2456515  & 12.254(0.038) & 11.596(0.050) & 11.215(0.052) \\
343 & NGC5975                        & SDSSJ153957.94+212814.2  & 15.990(0.009) & 13.226(0.002) & XSC---15395796+2128150  & 11.034(0.017) & 10.308(0.020) &  9.949(0.032) \\
344 & NGC5980                        & SDSSJ154130.44+154715.6  & 14.995(0.007) & 12.584(0.002) & XSC---15413039+1547156  & 10.518(0.019) &  9.743(0.019) &  9.441(0.024) \\
345 & NGC5992                        & SDSSJ154421.51+410510.9  & 15.405(0.006) & 14.017(0.002) & XSC---15442146+4105110  & 12.210(0.042) & 11.799(0.062) & 11.303(0.056) \\
346 & NGC5996                        & SDSSJ154658.88+175303.0  & 14.586(0.004) & 13.314(0.002) & XSC---15465887+1753031  & 11.503(0.034) & 10.813(0.045) & 10.415(0.044) \\
347 & IRAS15519+3537                 & SDSSJ155348.99+352804.5  & 18.273(0.026) & 15.929(0.003) & XSC---15534897+3528042  & 13.868(0.073) & 13.131(0.100) & 12.377(0.071) \\
348 & UGC10099                       & SDSSJ155636.39+415250.5  & 15.131(0.004) & 14.035(0.002) & XSC---15563641+4152501  & 12.565(0.030) & 11.893(0.037) & 11.621(0.056) \\
349 & MCG5-38-006                    & SDSSJ155843.69+264905.3  & 15.798(0.006) & 13.561(0.002) & XSC---15584368+2649050  & 11.347(0.028) & 10.776(0.030) & 10.701(0.051) \\
350 & UGC10120                       & SDSSJ155909.62+350147.5  & 15.658(0.008) & 14.047(0.002) & XSC---15590967+3501473  & 12.142(0.037) & 11.524(0.054) & 10.978(0.042) \\
351 & NGC6027A                       & SDSSJ155911.15+204517.0  & 16.288(0.014) & 13.274(0.002) & XSC---15591112+2045163  & 11.499(0.023) & 10.802(0.030) & 10.525(0.040) \\
352 & NGC6040B                       & SDSSJ160426.51+174431.1  & 17.008(0.015) & 14.104(0.002) & XSC---16042652+1744311  & 11.699(0.040) & 11.070(0.058) & 10.639(0.059) \\
353 & UGC10200                       & SDSSJ160545.89+412041.0  & 14.469(0.003) & 13.430(0.002) & XSC---16054591+4120410  & 12.245(0.031) & 11.701(0.042) & 11.543(0.061) \\
354 & IRAS16052+5334                 & SDSSJ160632.99+532632.2  & 19.126(0.040) & 16.521(0.004) & XSC---16063296+5326319  & 14.089(0.089) & 13.006(0.075) & 12.639(0.089) \\
355 & IRAS16053+1836                 & SDSSJ160738.52+182848.3  & 17.470(0.017) & 14.675(0.002) & XSC---16073851+1828485  & 12.392(0.036) & 11.683(0.052) & 11.239(0.048) \\
356 & NGC6090\_NED01                 & SDSSJ161140.30+522722.9  & 15.938(0.006) & 15.078(0.003) & PSC---16114033+5227228  & 14.423(0.075) & 13.833(0.085) & 13.314(0.061) \\
357 & UGC10273\_NED01                & SDSSJ161244.67+281710.0  & 16.629(0.012) & 15.163(0.003) & XSC---16124472+2817095  & 13.217(0.047) & 13.348(0.000) & 12.109(0.073) \\
358 & IRAS16150+2233                 & SDSSJ161708.94+222628.0  & 19.298(0.061) & 16.482(0.005) & XSC---16170895+2226279  & 13.994(0.069) & 13.230(0.082) & 12.821(0.093) \\
359 & UGC10322                       & SDSSJ161807.83+221332.2  & 15.864(0.017) & 13.755(0.003) & XSC---16180792+2213329  & 11.635(0.028) & 10.908(0.028) & 10.535(0.031) \\
360 & NGC6120                        & SDSSJ161948.11+374627.7  & 15.684(0.006) & 13.507(0.002) & XSC---16194809+3746282  & 11.476(0.021) & 10.785(0.021) & 10.472(0.029) \\
361 & MCG3-42-004                    & SDSSJ162415.17+201100.7  & 16.649(0.012) & 14.189(0.002) & XSC---16241515+2011009  & 12.260(0.034) & 11.647(0.046) & 11.144(0.048) \\
362 & UGC10407                       & SDSSJ162827.88+411303.6  & 16.072(0.007) & 14.927(0.003) & XSC---16282802+4113128  & 12.994(0.074) & 12.487(0.115) & 11.811(0.103) \\
363 & IRAS16320+3922                 & SDSSJ163349.61+391547.4  & 15.987(0.007) & 13.797(0.002) & XSC---16334964+3915478  & 11.984(0.032) & 11.220(0.038) & 10.954(0.044) \\
364 & NGC6186                        & SDSSJ163425.48+213227.0  & 15.802(0.006) & 13.593(0.002) & XSC---16342548+2132270  & 10.630(0.017) &  9.868(0.019) &  9.604(0.024) \\
365 & MCG9-27-053                    & SDSSJ163515.42+524649.7  & 18.162(0.033) & 14.936(0.003) & XSC---16351542+5246497  & 12.540(0.031) & 11.829(0.042) & 11.467(0.042) \\
366 & UGC10514                       & SDSSJ164223.73+250509.1  & 16.815(0.011) & 14.894(0.003) & XSC---16422373+2505093  & 12.674(0.041) & 11.951(0.056) & 11.614(0.056) \\
367 & IRAS16435+2154                 & SDSSJ164540.67+214919.0  & 17.710(0.019) & 15.328(0.003) & XSC---16454059+2149183  & 13.148(0.042) & 12.480(0.055) & 12.117(0.074) \\
368 & IC4623                         & SDSSJ165105.33+223138.6  & 16.596(0.011) & 14.383(0.002) & XSC---16510537+2231394  & 12.259(0.030) & 11.470(0.034) & 11.100(0.036) \\
369 & IRAS16516+3030                 & SDSSJ165337.16+302609.7  & 17.920(0.016) & 15.462(0.003) & XSC---16533720+3026104  & 13.158(0.033) & 12.368(0.035) & 11.802(0.034) \\
  \addlinespace % requires packages booktabs and longtable
  \hline
  \addlinespace % requires packages booktabs and longtable

  \label{table:SFRS_2MASS_SDSS}
 \end{longtable}
 
 \vspace{-1cm} 
 
 \begin{center}
  \begin{minipage}{0.85\linewidth}
   \noindent
   $^{(1)}$ SFRS target ID;
   $^{(2)}$ Galaxy name;
   $^{(3)}$ SDSS-DR12 ID;
   $^{(4)}$ SDSS $u$ magnitude (SDSS $ugriz$ filter set);
   $^{(5)}$ SDSS $r$ magnitude (SDSS $ugriz$ filter set);
   $^{(6)}$ 2MASS Extended Source Catalogue (XSC) or Point Source Catalogue (PSC) ID;
   $^{(7)}$ 2MASS $J$-band magnitude;
   $^{(8)}$ 2MASS $H$-band magnitude;
   $^{(9)}$ 2MASS $K$-band magnitude.
   \\
   $\dagger$: SDSS modelMag;
   $\ddagger$: 2MASS-XSC values refer to the ``extrapolated magnitudes''.
   ($J.ext$, $H.ext$, and $K.ext$; see Section 3.1).

  \end{minipage}
 \end{center}
\end{landscape}


==> full_tables/TABLE_D2/TABLE_selected_models.tex <==
 
%------------------------------------- TABLE  -------------------------------------
% generated by selected_models_v5.1.pl
\begin{landscape}
 {
  \definecolor{LightGray}{rgb}{0.92,0.92,0.92}
  \definecolor{White}{rgb}{1.0,1.0,1.0}
  \footnotesize
  \renewcommand{\tabcolsep}{0.3em}
  \renewcommand{\arraystretch}{0.95}
  \begin{longtable}[!h]{ll @{\hskip 0.35cm} ccccccccccccccccc}
   \caption*{{\normalsize Table D2: \GALFIT{} model results for the SFRS sample.
   }}\\
   \hline
   \addlinespace % requires packages booktabs and longtable
   \multicolumn{19}{c}{{\normalsize \textsc{SFRS Targets --- Galfit Model Results}}}\\
   \hline
   \addlinespace % requires packages booktabs and longtable
   \hline
   \addlinespace % requires packages booktabs and longtable
   \multicolumn{1}{c}{Target}      & \multicolumn{1}{c}{Selected Model} & Model       & Comp.       & S\'{e}rsic  & $R$       & Comp. $m_{K}$ & K-corr      & Comp. $L_{K}$  & ($u-r$)    & Comp. $M/L$                   & $M/L$                         & Comp. M          & Total M$^{\dagger}$ & Decomp.      & $B/T$      & $D$	       & Nuc.         & Weight       \\
   \multicolumn{1}{c}{Name}        & \multicolumn{1}{c}{}               & Comp.       & Nature      & $n$        & [\arcsec]  & [mag]           &             & [erg s$^{-1}$] & [mag]        & [$L_{\odot}$/M$_{\odot}$] & [$L_{\odot}$/M$_{\odot}$] & [M$_{\odot}$] & [M$_{\odot}$]       & Method       &              & [Mpc]             & Class.       &              \\
   \multicolumn{1}{c}{\tiny{(1)}} & \multicolumn{1}{c}{\tiny{(2)}}    & \tiny{(3)} & \tiny{(4)} & \tiny{(5)}  & \tiny{(6)} & \tiny{(7)}     & \tiny{(8)} & \tiny{(9)}      & \tiny{(10)} & \tiny{(11)}                    & \tiny{(12)}                    & \tiny{(13)}     & \tiny{(14)}	          & \tiny{(15)} & \tiny{(16)} & \tiny{(17)} & \tiny{(18)} & \tiny{(19)} \\
   \hline
   \addlinespace % requires packages booktabs and longtable
   \endfirsthead

   \multicolumn{16}{@{}l}{{\normalsize Table D2 --- \emph{continued}}}\\
   \hline
   \addlinespace % requires packages booktabs and longtable
   \multicolumn{1}{c}{Target}      & \multicolumn{1}{c}{Selected Model} & Model       & Comp.       & S\'{e}rsic  & $R$       & Comp. $m_{K}$ & K-corr      & Comp. $L_{K}$  & ($u-r$)    & Comp. $M/L$                   & $M/L$                         & Comp. M          & Total M$^{\dagger}$ & Decomp.      & $B/T$      & $D$	       & Nuc.         & Weight       \\
   \multicolumn{1}{c}{Name}        & \multicolumn{1}{c}{}               & Comp.       & Nature      & $n$        & [\arcsec]  & [mag]           &             & [erg s$^{-1}$] & [mag]        & [$L_{\odot}$/M$_{\odot}$] & [$L_{\odot}$/M$_{\odot}$] & [M$_{\odot}$] & [M$_{\odot}$]       & Method       &              & [Mpc]             & Class.       &              \\
   \multicolumn{1}{c}{\tiny{(1)}} & \multicolumn{1}{c}{\tiny{(2)}}    & \tiny{(3)} & \tiny{(4)} & \tiny{(5)}  & \tiny{(6)} & \tiny{(7)}     & \tiny{(8)} & \tiny{(9)}      & \tiny{(10)} & \tiny{(11)}                    & \tiny{(12)}                    & \tiny{(13)}     & \tiny{(14)}	          & \tiny{(15)} & \tiny{(16)} & \tiny{(17)} & \tiny{(18)} & \tiny{(19)} \\
   \hline
   \addlinespace % requires packages booktabs and long
   \endhead
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC2217                 & Sersic + exDisk          & Sersic         & bulge & 4.0 & 8.1   & 11.56$\pm$0.12 & 0.969 & 1.48e+43 & 2.48  & 0.897 & 0.720 & 2.67e+10 & 4.51e+10 & \textsc{Galfit}   & 0.473$\pm$0.125 & 7.61e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
IC2217                 & Sersic + exDisk          & exDisk         & disk  & --- & 5.9   & 11.44$\pm$0.07 & 0.969 & 1.65e+43 & 1.58  & 0.743 & 0.720 & 2.47e+10 & 4.51e+10 & \textsc{Galfit}   & 0.473$\pm$0.125 & 7.61e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2500                & Sersic + psfAgn          & Sersic         & disk  & 1.8 & 89.1  & 8.51 $\pm$0.04 & 0.980 & 9.63e+42 & 1.50  & 0.730 & 0.784 & 1.41e+10 & 1.52e+10 & \textsc{Galfit}   & 0.001$\pm$0.001 & 1.50e+07 & LINER & 4.2 \\ 
\rowcolor{White}
NGC2500                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 16.07$\pm$0.13 & 0.980 & 9.12e+39 & 4.64  & 1.410 & 0.784 & 2.59e+07 & 1.52e+10 & \textsc{Galfit}   & 0.001$\pm$0.001 & 1.50e+07 & LINER & 4.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2512                & Sersic + psfAgn          & Sersic         & disk  & 1.5 & 14.0  & 9.92 $\pm$0.04 & 0.962 & 5.51e+43 & 2.11  & 0.830 & 0.849 & 9.20e+10 & 1.03e+11 & \textsc{Galfit}   & 0.089$\pm$0.009 & 6.93e+07 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{LightGray}
NGC2512                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.45$\pm$0.04 & 0.962 & 5.36e+42 & 1.51  & 0.732 & 0.849 & 7.89e+09 & 1.03e+11 & \textsc{Galfit}   & 0.089$\pm$0.009 & 6.93e+07 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG6-18-009            & Sersic                   & Sersic         & mixed & 5.6 & 8.8   & 10.49$\pm$0.04 & 0.924 & 1.76e+44 & NA    & NA    & 0.788 & ---   & 2.79e+11 & $C\mapsto$~B/T    & 0.204$\pm$0.054 & 1.64e+08 & H\,{\sevensize II} & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MK1212                 & Sersic                   & Sersic         & mixed & 4.1 & 2.1   & 11.57$\pm$0.04 & 0.928 & 7.27e+43 & NA    & NA    & 0.774 & ---   & 1.13e+11 & $C\mapsto$~B/T    & 0.184$\pm$0.049 & 1.73e+08 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS08072+1847         & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 1.7   & 12.58$\pm$0.06 & 0.957 & 4.94e+42 & 2.59  & 0.918 & 0.935 & 9.12e+09 & 1.31e+10 & \textsc{Galfit}   & 0.290$\pm$0.077 & 7.08e+07 & SN    & 8.1 \\ 
\rowcolor{White}
IRAS08072+1847         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.55$\pm$0.10 & 0.957 & 2.02e+42 & 1.68  & 0.758 & 0.935 & 3.08e+09 & 1.31e+10 & \textsc{Galfit}   & 0.290$\pm$0.077 & 7.08e+07 & SN    & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2532                & Sersic + psfAgn          & Sersic         & disk  & 1.2 & 18.8  & 9.85 $\pm$0.04 & 0.959 & 7.35e+43 & 2.04  & 0.818 & 0.913 & 1.21e+11 & 1.47e+11 & \textsc{Galfit}   & 0.077$\pm$0.009 & 7.76e+07 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{LightGray}
NGC2532                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.55$\pm$0.04 & 0.959 & 6.11e+42 & 2.06  & 0.821 & 0.913 & 1.01e+10 & 1.47e+11 & \textsc{Galfit}   & 0.077$\pm$0.009 & 7.76e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2535                & Sersic + psfAgn          & Sersic         & disk  & 1.2 & 23.8  & 10.06$\pm$0.04 & 0.979 & 3.90e+43 & 1.70  & 0.762 & 0.854 & 5.98e+10 & 7.14e+10 & \textsc{Galfit}   & 0.065$\pm$0.006 & 6.16e+07 & H\,{\sevensize II} & 5.5 \\ 
\rowcolor{White}
NGC2535                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.96$\pm$0.04 & 0.979 & 2.70e+42 & 2.36  & 0.875 & 0.854 & 4.75e+09 & 7.14e+10 & \textsc{Galfit}   & 0.065$\pm$0.006 & 6.16e+07 & H\,{\sevensize II} & 5.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2543                & Sersic + psfAgn          & Sersic         & disk  & 3.5 & 43.1  & 9.04 $\pm$0.04 & 0.982 & 1.82e+43 & 2.42  & 0.886 & 0.914 & 3.24e+10 & 3.51e+10 & \textsc{Galfit}   & 0.043$\pm$0.010 & 2.63e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{LightGray}
NGC2543                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.41$\pm$0.04 & 0.982 & 8.18e+41 & 2.08  & 0.825 & 0.914 & 1.36e+09 & 3.51e+10 & \textsc{Galfit}   & 0.043$\pm$0.010 & 2.63e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2537                & Sersic                   & Sersic         & disk  & 0.3 & 22.5  & 9.24 $\pm$0.04 & 0.996 & 5.00e+42 & 2.01  & 0.813 & 0.740 & 8.18e+09 & 7.44e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.50e+07 & H\,{\sevensize II} & 3.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC2233                 & Sersic                   & Sersic         & disk  & 1.0 & 50.1  & 10.73$\pm$0.04 & 0.998 & 1.06e+42 & 2.01  & 0.813 & 0.333 & 1.73e+09 & 7.09e+08 & \textsc{Galfit}   & 0    $\pm$0     & 1.37e+07 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC2239                 & Sersic + psfAgn          & Sersic         & disk  & 3.5 & 7.3   & 10.41$\pm$0.04 & 0.955 & 5.68e+43 & 2.37  & 0.876 & 0.883 & 1.00e+11 & 1.15e+11 & \textsc{Galfit}   & 0.123$\pm$0.041 & 8.85e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{White}
IC2239                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.54$\pm$0.06 & 0.955 & 7.98e+42 & 2.44  & 0.889 & 0.883 & 1.43e+10 & 1.15e+11 & \textsc{Galfit}   & 0.123$\pm$0.041 & 8.85e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC4286                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.1   & 12.97$\pm$0.09 & 0.961 & 3.73e+42 & 4.09  & 1.257 & 0.896 & 9.43e+09 & 4.44e+10 & \textsc{Galfit}   & 0.151$\pm$0.136 & 7.35e+07 & H\,{\sevensize II} & 3.0 \\ 
\rowcolor{LightGray}
UGC4286                & Sersic + exDisk          & exDisk         & disk  & --- & 7.4   & 11.10$\pm$0.04 & 0.961 & 2.09e+43 & 1.89  & 0.792 & 0.896 & 3.33e+10 & 4.44e+10 & \textsc{Galfit}   & 0.151$\pm$0.136 & 7.35e+07 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC4306                & Sersic                   & Sersic         & disk  & 1.1 & 5.5   & 10.53$\pm$0.04 & 0.975 & 8.59e+42 & 2.01  & 0.813 & 0.927 & 1.41e+10 & 1.60e+10 & \textsc{Galfit}   & 0    $\pm$0     & 3.60e+07 & H\,{\sevensize II} & 8.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC4383                & Sersic + psfAgn          & Sersic         & disk  & 1.4 & 11.1  & 11.45$\pm$0.04 & 0.974 & 1.78e+43 & 1.82  & 0.781 & 0.765 & 2.80e+10 & 3.04e+10 & \textsc{Galfit}   & 0.094$\pm$0.027 & 7.93e+07 & H\,{\sevensize II} & 3.0 \\ 
\rowcolor{LightGray}
UGC4383                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.91$\pm$0.05 & 0.974 & 1.85e+42 & 0.82  & 0.633 & 0.765 & 2.36e+09 & 3.04e+10 & \textsc{Galfit}   & 0.094$\pm$0.027 & 7.93e+07 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS08234+1054         & Sersic + psfAgn          & Sersic         & disk  & 0.1 & 4.1   & 13.13$\pm$0.04 & 0.864 & 3.98e+43 & 2.38  & 0.878 & 1.018 & 7.03e+10 & 1.06e+11 & \textsc{Galfit}   & 0.230$\pm$0.061 & 2.73e+08 & H\,{\sevensize II} & 6.6 \\ 
\rowcolor{White}
IRAS08234+1054         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.44$\pm$0.09 & 0.864 & 1.19e+43 & 2.64  & 0.927 & 1.018 & 2.22e+10 & 1.06e+11 & \textsc{Galfit}   & 0.230$\pm$0.061 & 2.73e+08 & H\,{\sevensize II} & 6.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS08269+1514         & Sersic                   & Sersic         & mixed & 6.2 & 8.3   & 11.93$\pm$0.08 & 0.888 & 3.01e+43 & NA    & NA    & 0.834 & ---   & 5.05e+10 & $C\mapsto$~B/T    & 0.133$\pm$0.035 & 1.34e+08 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2604                & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 36.1  & 10.15$\pm$0.04 & 0.981 & 1.25e+43 & 2.65  & 0.929 & 0.664 & 2.34e+10 & 1.67e+10 & \textsc{Galfit}   & 1.000$\pm$0.265 & 3.63e+07 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2608                & Sersic + psfAgn          & Sersic         & disk  & 2.5 & 65.5  & 8.64 $\pm$0.04 & 0.982 & 5.02e+43 & 1.97  & 0.806 & 0.842 & 8.14e+10 & 8.74e+10 & \textsc{Galfit}   & 0.030$\pm$0.003 & 3.63e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{LightGray}
NGC2608                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.43$\pm$0.04 & 0.982 & 1.53e+42 & 2.52  & 0.904 & 0.842 & 2.78e+09 & 8.74e+10 & \textsc{Galfit}   & 0.030$\pm$0.003 & 3.63e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2623                & Sersic + psfAgn          & Sersic         & disk  & 1.3 & 4.9   & 11.20$\pm$0.04 & 0.944 & 2.31e+43 & 2.19  & 0.844 & 0.869 & 3.92e+10 & 6.28e+10 & \textsc{Galfit}   & 0.358$\pm$0.037 & 8.16e+07 & SN    & 15.5\\ 
\rowcolor{White}
NGC2623                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.83$\pm$0.04 & 0.944 & 1.29e+43 & 2.19  & 0.844 & 0.869 & 2.19e+10 & 6.28e+10 & \textsc{Galfit}   & 0.358$\pm$0.037 & 8.16e+07 & SN    & 15.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
CGCG120-018            & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 4.1   & 12.20$\pm$0.05 & 0.937 & 1.59e+43 & 2.30  & 0.864 & 0.890 & 2.76e+10 & 5.00e+10 & \textsc{Galfit}   & 0.430$\pm$0.079 & 1.08e+08 & H\,{\sevensize II} & 8.1 \\ 
\rowcolor{LightGray}
CGCG120-018            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.51$\pm$0.05 & 0.937 & 1.20e+43 & 3.13  & 1.028 & 0.890 & 2.48e+10 & 5.00e+10 & \textsc{Galfit}   & 0.430$\pm$0.079 & 1.08e+08 & H\,{\sevensize II} & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2644                & Sersic                   & Sersic         & mixed & 1.6 & 15.8  & 10.36$\pm$0.04 & 0.991 & 4.93e+42 & NA    & NA    & 0.768 & ---   & 7.61e+09 & $C\mapsto$~B/T    & 0.160$\pm$0.042 & 2.50e+07 & H\,{\sevensize II} & 4.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC4572                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.8   & 11.43$\pm$0.08 & 0.978 & 1.06e+43 & 2.76  & 0.951 & 0.862 & 2.03e+10 & 3.64e+10 & \textsc{Galfit}   & 0.507$\pm$0.133 & 6.05e+07 & TO    & 4.3 \\ 
\rowcolor{LightGray}
UGC4572                & Sersic + exDisk          & exDisk         & disk  & --- & 4.8   & 11.46$\pm$0.06 & 0.978 & 1.03e+43 & 1.29  & 0.699 & 0.862 & 1.45e+10 & 3.64e+10 & \textsc{Galfit}   & 0.507$\pm$0.133 & 6.05e+07 & TO    & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS08512+2727         & Sersic + psfAgn          & Sersic         & disk  & 0.8 & 4.8   & 12.08$\pm$0.04 & 0.903 & 1.04e+44 & 1.63  & 0.750 & 0.778 & 1.57e+11 & 1.92e+11 & \textsc{Galfit}   & 0.149$\pm$0.039 & 2.65e+08 & H\,{\sevensize II} & 1.0 \\ 
\rowcolor{White}
IRAS08512+2727         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.97$\pm$0.06 & 0.903 & 1.82e+43 & 3.15  & 1.032 & 0.778 & 3.78e+10 & 1.92e+11 & \textsc{Galfit}   & 0.149$\pm$0.039 & 2.65e+08 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS08538+4256         & Sersic                   & Sersic         & mixed & 3.0 & 3.4   & 11.61$\pm$0.04 & 0.915 & 3.38e+43 & NA    & NA    & 0.865 & ---   & 5.88e+10 & $C\mapsto$~B/T    & 0.141$\pm$0.037 & 1.21e+08 & H\,{\sevensize II} & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS08550+3908         & Sersic + psfAgn          & Sersic         & disk  & 3.6 & 7.8   & 11.70$\pm$0.06 & 0.719 & 2.25e+44 & 3.07  & 1.015 & 0.864 & 4.60e+11 & 4.14e+11 & \textsc{Galfit}   & 0.056$\pm$0.015 & 3.68e+08 & SN    & 1.5 \\ 
\rowcolor{White}
IRAS08550+3908         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.77$\pm$0.10 & 0.719 & 1.33e+43 & 3.45  & 1.099 & 0.864 & 2.94e+10 & 4.14e+11 & \textsc{Galfit}   & 0.056$\pm$0.015 & 3.68e+08 & SN    & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2718                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.2   & 11.60$\pm$0.04 & 0.967 & 8.09e+42 & 1.33  & 0.705 & 0.819 & 1.15e+10 & 1.01e+11 & \textsc{Galfit}   & 0.132$\pm$0.019 & 5.74e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{LightGray}
NGC2718                & Sersic + exDisk          & exDisk         & disk  & --- & 15.7  & 9.55 $\pm$0.04 & 0.967 & 5.34e+43 & 2.04  & 0.818 & 0.819 & 8.79e+10 & 1.01e+11 & \textsc{Galfit}   & 0.132$\pm$0.019 & 5.74e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2712                & Sersic + psfAgn          & Sersic         & disk  & 2.6 & 38.4  & 8.94 $\pm$0.04 & 0.988 & 2.77e+43 & 2.03  & 0.816 & 0.859 & 4.55e+10 & 5.02e+10 & \textsc{Galfit}   & 0.049$\pm$0.002 & 3.09e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{White}
NGC2712                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.17$\pm$0.04 & 0.988 & 1.42e+42 & 2.74  & 0.947 & 0.859 & 2.71e+09 & 5.02e+10 & \textsc{Galfit}   & 0.049$\pm$0.002 & 3.09e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2719                & Sersic                   & Sersic         & disk  & 1.3 & 14.0  & 11.76$\pm$0.04 & 0.996 & 5.70e+42 & 2.01  & 0.813 & 0.661 & 9.32e+09 & 7.58e+09 & \textsc{Galfit}   & 0    $\pm$0     & 5.11e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS08579+3447         & Sersic + psfAgn          & Sersic         & disk  & 0.5 & 4.8   & 12.37$\pm$0.04 & 0.835 & 7.80e+43 & 1.84  & 0.784 & 0.813 & 1.23e+11 & 1.64e+11 & \textsc{Galfit}   & 0.219$\pm$0.058 & 2.74e+08 & H\,{\sevensize II} & 6.6 \\ 
\rowcolor{White}
IRAS08579+3447         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.75$\pm$0.06 & 0.835 & 2.19e+43 & 2.98  & 0.996 & 0.813 & 4.39e+10 & 1.64e+11 & \textsc{Galfit}   & 0.219$\pm$0.058 & 2.74e+08 & H\,{\sevensize II} & 6.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2731                & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 10.8  & 10.54$\pm$0.03 & 0.983 & 8.12e+42 & 1.47  & 0.726 & 0.768 & 1.19e+10 & 1.28e+10 & \textsc{Galfit}   & 0.021$\pm$0.012 & 3.50e+07 & H\,{\sevensize II} & 6.9 \\ 
\rowcolor{LightGray}
NGC2731                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.70$\pm$0.08 & 0.983 & 1.76e+41 & 2.55  & 0.910 & 0.768 & 3.22e+08 & 1.28e+10 & \textsc{Galfit}   & 0.021$\pm$0.012 & 3.50e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2750                & Sersic                   & Sersic         & mixed & 6.9 & 14.5  & 10.13$\pm$0.04 & 0.990 & 1.33e+43 & NA    & NA    & 0.749 & ---   & 2.01e+10 & $C\mapsto$~B/T    & 0.211$\pm$0.056 & 3.70e+07 & H\,{\sevensize II} & 8.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC2434                 & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.9   & 12.43$\pm$0.06 & 0.945 & 1.22e+43 & 3.15  & 1.032 & 0.932 & 2.53e+10 & 1.72e+11 & \textsc{Galfit}   & 0.134$\pm$0.057 & 1.04e+08 & TO    & 7.4 \\ 
\rowcolor{LightGray}
IC2434                 & Sersic + exDisk          & exDisk         & disk  & --- & 7.2   & 10.40$\pm$0.04 & 0.945 & 7.91e+43 & 2.38  & 0.878 & 0.932 & 1.40e+11 & 1.72e+11 & \textsc{Galfit}   & 0.134$\pm$0.057 & 1.04e+08 & TO    & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2761                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.6   & 12.74$\pm$0.09 & 0.917 & 1.27e+43 & 2.96  & 0.992 & 0.916 & 2.53e+10 & 1.47e+11 & \textsc{Galfit}   & 0.160$\pm$0.160 & 1.25e+08 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{White}
NGC2761                & Sersic + exDisk          & exDisk         & disk  & --- & 5.0   & 10.94$\pm$0.04 & 0.917 & 6.68e+43 & 2.07  & 0.823 & 0.916 & 1.11e+11 & 1.47e+11 & \textsc{Galfit}   & 0.160$\pm$0.160 & 1.25e+08 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2773                & Sersic                   & Sersic         & mixed & 1.8 & 5.3   & 10.47$\pm$0.03 & 0.953 & 4.43e+43 & NA    & NA    & 0.901 & ---   & 8.03e+10 & $C\mapsto$~B/T    & 0.149$\pm$0.039 & 8.04e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2776                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 7.2   & 11.09$\pm$0.07 & 0.985 & 5.18e+42 & 2.91  & 0.981 & 0.841 & 1.02e+10 & 5.09e+10 & \textsc{Galfit}   & 0.172$\pm$0.078 & 3.60e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{White}
NGC2776                & Sersic + exDisk          & exDisk         & disk  & --- & 14.6  & 9.38 $\pm$0.04 & 0.985 & 2.50e+43 & 1.63  & 0.750 & 0.841 & 3.77e+10 & 5.09e+10 & \textsc{Galfit}   & 0.172$\pm$0.078 & 3.60e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2789                & Sersic + psfAgn          & Sersic         & disk  & 5.0 & 8.8   & 9.70 $\pm$0.04 & 0.953 & 1.22e+44 & 4.25  & 1.299 & 0.865 & 3.19e+11 & 2.18e+11 & \textsc{Galfit}   & 0.025$\pm$0.015 & 9.36e+07 & H\,{\sevensize II} & 3.8 \\ 
\rowcolor{LightGray}
NGC2789                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.68$\pm$0.12 & 0.953 & 3.12e+42 & 6.07  & 1.903 & 0.865 & 1.19e+10 & 2.18e+11 & \textsc{Galfit}   & 0.025$\pm$0.015 & 9.36e+07 & H\,{\sevensize II} & 3.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2824                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.3   & 10.92$\pm$0.05 & 0.983 & 6.39e+42 & 2.43  & 0.887 & 0.902 & 1.14e+10 & 2.38e+10 & \textsc{Galfit}   & 0.489$\pm$0.096 & 3.70e+07 & LINER & 2.3 \\ 
\rowcolor{White}
NGC2824                & Sersic + exDisk          & exDisk         & disk  & --- & 5.0   & 10.87$\pm$0.05 & 0.983 & 6.69e+42 & 2.45  & 0.891 & 0.902 & 1.20e+10 & 2.38e+10 & \textsc{Galfit}   & 0.489$\pm$0.096 & 3.70e+07 & LINER & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS09121+3908         & Sersic + psfAgn          & Sersic         & disk  & 2.1 & 1.8   & 13.20$\pm$0.06 & 0.959 & 1.01e+42 & 2.84  & 0.967 & 0.982 & 1.97e+09 & 2.58e+09 & \textsc{Galfit}   & 0.227$\pm$0.060 & 4.25e+07 & H\,{\sevensize II} & 3.5 \\ 
\rowcolor{LightGray}
IRAS09121+3908         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.53$\pm$0.18 & 0.959 & 2.96e+41 & 3.39  & 1.085 & 0.982 & 6.46e+08 & 2.58e+09 & \textsc{Galfit}   & 0.227$\pm$0.060 & 4.25e+07 & H\,{\sevensize II} & 3.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS09184+4356         & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 3.4   & 11.24$\pm$0.04 & 0.900 & 9.21e+43 & 2.65  & 0.929 & 0.892 & 1.72e+11 & 1.65e+11 & \textsc{Galfit}   & 1.000$\pm$0.265 & 1.70e+08 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
CGCG238-041            & Sersic                   & Sersic         & mixed & 3.7 & 8.0   & 12.16$\pm$0.09 & 0.947 & 2.48e+43 & NA    & NA    & 0.656 & ---   & 3.27e+10 & $C\mapsto$~B/T    & 0.100$\pm$0.027 & 1.32e+08 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS09197+2210         & Sersic                   & Sersic         & disk  & 0.9 & 6.2   & 11.88$\pm$0.04 & 0.895 & 3.61e+43 & 2.01  & 0.813 & 0.909 & 5.91e+10 & 6.60e+10 & \textsc{Galfit}   & 0    $\pm$0     & 1.43e+08 & TO    & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2854                & Sersic + psfAgn          & Sersic         & mixed & 1.9 & 17.4  & 9.79 $\pm$0.04 & 0.988 & 8.30e+42 & NA    & NA    & 0.830 & ---   & 1.39e+10 & $C\mapsto$~B/T    & 0.123$\pm$0.033 & 2.50e+07 & TO    & 5.7 \\ 
\rowcolor{LightGray}
NGC2854                & Sersic + psfAgn          & psfAgn         & AGN   & --- & ---   & 13.55$\pm$0.06 & 0.988 & 2.60e+41 & NA    & NA    & 0.830 & ---   & 1.39e+10 & $C\mapsto$~B/T    & 0.123$\pm$0.033 & 2.50e+07 & TO    & 5.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC5046                & Sersic + psfAgn          & Sersic         & disk  & 1.9 & 9.1   & 10.61$\pm$0.04 & 0.957 & 2.55e+43 & 1.75  & 0.770 & 0.749 & 3.95e+10 & 3.95e+10 & \textsc{Galfit}   & 0.030$\pm$0.017 & 6.49e+07 & H\,{\sevensize II} & 6.9 \\ 
\rowcolor{White}
UGC5046                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.37$\pm$0.12 & 0.957 & 7.98e+41 & -0.29 & 0.502 & 0.749 & 8.06e+08 & 3.95e+10 & \textsc{Galfit}   & 0.030$\pm$0.017 & 6.49e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5055                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.5   & 11.45$\pm$0.04 & 0.942 & 3.36e+43 & 2.17  & 0.840 & 0.824 & 5.68e+10 & 1.03e+11 & \textsc{Galfit}   & 0.539$\pm$0.074 & 1.11e+08 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{LightGray}
UGC5055                & Sersic + exDisk          & exDisk         & disk  & --- & 9.5   & 11.62$\pm$0.04 & 0.942 & 2.87e+43 & 1.80  & 0.778 & 0.824 & 4.49e+10 & 1.03e+11 & \textsc{Galfit}   & 0.539$\pm$0.074 & 1.11e+08 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC2893                & Sersic + psfAgn          & Sersic         & disk  & 1.6 & 7.4   & 10.49$\pm$0.04 & 0.990 & 4.02e+42 & 1.97  & 0.806 & 0.808 & 6.52e+09 & 7.78e+09 & \textsc{Galfit}   & 0.164$\pm$0.020 & 2.40e+07 & H\,{\sevensize II} & 5.7 \\ 
\rowcolor{White}
NGC2893                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.26$\pm$0.04 & 0.990 & 7.88e+41 & 1.08  & 0.669 & 0.808 & 1.06e+09 & 7.78e+09 & \textsc{Galfit}   & 0.164$\pm$0.020 & 2.40e+07 & H\,{\sevensize II} & 5.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG3-24-062            & Sersic + exDisk          & Sersic         & bulge & 4.0 & 8.0   & 11.35$\pm$0.04 & 0.941 & 1.32e+43 & 3.16  & 1.034 & 0.932 & 2.75e+10 & 4.58e+10 & \textsc{Galfit}   & 0.541$\pm$0.067 & 6.62e+07 & H\,{\sevensize II} & 5.5 \\ 
\rowcolor{LightGray}
MCG3-24-062            & Sersic + exDisk          & exDisk         & disk  & --- & 5.8   & 11.53$\pm$0.04 & 0.941 & 1.12e+43 & 2.16  & 0.839 & 0.932 & 1.89e+10 & 4.58e+10 & \textsc{Galfit}   & 0.541$\pm$0.067 & 6.62e+07 & H\,{\sevensize II} & 5.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
CGCG238-066            & Sersic + psfAgn          & Sersic         & disk  & 3.7 & 7.4   & 11.29$\pm$0.06 & 0.933 & 6.81e+43 & 2.09  & 0.826 & 0.839 & 1.13e+11 & 1.31e+11 & \textsc{Galfit}   & 0.118$\pm$0.056 & 1.47e+08 & SN    & 6.0 \\ 
\rowcolor{White}
CGCG238-066            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.47$\pm$0.09 & 0.933 & 9.15e+42 & 4.50  & 1.369 & 0.839 & 2.52e+10 & 1.31e+11 & \textsc{Galfit}   & 0.118$\pm$0.056 & 1.47e+08 & SN    & 6.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5097                & Sersic                   & Sersic         & disk  & 1.1 & 7.3   & 11.22$\pm$0.03 & 0.980 & 1.86e+43 & 2.01  & 0.813 & 0.685 & 3.04e+10 & 2.56e+10 & \textsc{Galfit}   & 0    $\pm$0     & 7.25e+07 & H\,{\sevensize II} & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
CGCG289-012            & Sersic                   & Sersic         & disk  & 1.3 & 4.5   & 11.60$\pm$0.04 & 0.934 & 7.04e+43 & 2.01  & 0.813 & 0.767 & 1.15e+11 & 1.09e+11 & \textsc{Galfit}   & 0    $\pm$0     & 1.72e+08 & H\,{\sevensize II} & 4.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG8-18-013            & Sersic + psfAgn          & Sersic         & disk  & 1.2 & 5.3   & 11.47$\pm$0.04 & 0.940 & 3.31e+43 & 2.65  & 0.929 & 0.826 & 6.19e+10 & 7.87e+10 & \textsc{Galfit}   & 0.303$\pm$0.062 & 1.11e+08 & H\,{\sevensize II} & 14.2\\ 
\rowcolor{LightGray}
MCG8-18-013            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.37$\pm$0.04 & 0.940 & 1.44e+43 & 2.65  & 0.929 & 0.826 & 2.69e+10 & 7.87e+10 & \textsc{Galfit}   & 0.303$\pm$0.062 & 1.11e+08 & H\,{\sevensize II} & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
CGCG181-068            & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.2   & 12.24$\pm$0.06 & 0.912 & 1.30e+43 & 2.97  & 0.994 & 0.926 & 2.60e+10 & 7.79e+10 & \textsc{Galfit}   & 0.312$\pm$0.118 & 1.01e+08 & TO    & 5.5 \\ 
\rowcolor{White}
CGCG181-068            & Sersic + exDisk          & exDisk         & disk  & --- & 6.4   & 11.38$\pm$0.04 & 0.912 & 2.87e+43 & 2.61  & 0.922 & 0.926 & 5.32e+10 & 7.79e+10 & \textsc{Galfit}   & 0.312$\pm$0.118 & 1.01e+08 & TO    & 5.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC2955                & Sersic + psfAgn          & Sersic         & disk  & 2.2 & 13.4  & 10.08$\pm$0.04 & 0.958 & 1.06e+44 & 2.09  & 0.826 & 0.827 & 1.76e+11 & 1.84e+11 & \textsc{Galfit}   & 0.041$\pm$0.007 & 1.04e+08 & H\,{\sevensize II} & 4.8 \\ 
\rowcolor{LightGray}
NGC2955                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.49$\pm$0.06 & 0.958 & 4.57e+42 & 4.75  & 1.443 & 0.827 & 1.33e+10 & 1.84e+11 & \textsc{Galfit}   & 0.041$\pm$0.007 & 1.04e+08 & H\,{\sevensize II} & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
CGCG182-010            & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.0   & 12.10$\pm$0.06 & 0.902 & 4.43e+43 & 2.80  & 0.959 & 0.850 & 8.55e+10 & 1.42e+11 & \textsc{Galfit}   & 0.532$\pm$0.030 & 1.75e+08 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{White}
CGCG182-010            & Sersic + exDisk          & exDisk         & disk  & --- & 2.2   & 12.24$\pm$0.05 & 0.902 & 3.89e+43 & 1.86  & 0.788 & 0.850 & 6.17e+10 & 1.42e+11 & \textsc{Galfit}   & 0.532$\pm$0.030 & 1.75e+08 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5228                & Sersic                   & Sersic         & disk  & 1.4 & 36.8  & 10.00$\pm$0.04 & 0.982 & 8.65e+42 & 2.01  & 0.813 & 0.822 & 1.41e+10 & 1.43e+10 & \textsc{Galfit}   & 0    $\pm$0     & 2.82e+07 & H\,{\sevensize II} & 4.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS09438+1141         & Sersic                   & Sersic         & mixed & 3.0 & 4.7   & 12.14$\pm$0.07 & 0.909 & 5.78e+43 & NA    & NA    & 0.779 & ---   & 9.06e+10 & $C\mapsto$~B/T    & 0.119$\pm$0.032 & 2.03e+08 & H\,{\sevensize II} & 4.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3015                & Sersic + psfAgn + exDisk & Sersic         & bulge & 4.0 & 0.7   & 12.65$\pm$0.26 & 0.942 & 1.08e+43 & 2.85  & 0.969 & 0.832 & 2.11e+10 & 1.12e+11 & \textsc{Galfit}   & 0.162$\pm$0.161 & 1.09e+08 & TO    & 7.4 \\ 
\rowcolor{LightGray}
NGC3015                & Sersic + psfAgn + exDisk & psfAgn         & AGN   & --- & ---   & 13.66$\pm$0.14 & 0.942 & 4.24e+42 & NA    & NA    & 0.832 & ---   & 1.12e+11 & \textsc{Galfit}   & 0.162$\pm$0.161 & 1.09e+08 & TO    & 7.4 \\ 
\rowcolor{LightGray}
NGC3015                & Sersic + psfAgn + exDisk & exDisk         & disk  & --- & 2.7   & 10.86$\pm$0.05 & 0.942 & 5.60e+43 & 1.95  & 0.803 & 0.832 & 9.05e+10 & 1.12e+11 & \textsc{Galfit}   & 0.162$\pm$0.161 & 1.09e+08 & TO    & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG2-25-039            & Sersic                   & Sersic         & mixed & 1.7 & 5.2   & 11.32$\pm$0.03 & 0.954 & 1.89e+43 & NA    & NA    & 0.800 & ---   & 3.04e+10 & $C\mapsto$~B/T    & 0.181$\pm$0.048 & 7.76e+07 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3020                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 37.4  & 10.41$\pm$0.05 & 0.995 & 2.53e+42 & 1.15  & 0.679 & 0.701 & 3.46e+09 & 3.57e+09 & \textsc{Galfit}   & 0.004$\pm$0.014 & 1.83e+07 & H\,{\sevensize II} & 3.0 \\ 
\rowcolor{LightGray}
NGC3020                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 16.29$\pm$0.23 & 0.995 & 1.13e+40 & 0.70  & 0.618 & 0.701 & 1.41e+07 & 3.57e+09 & \textsc{Galfit}   & 0.004$\pm$0.014 & 1.83e+07 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3049                & Sersic + psfAgn          & Sersic         & disk  & 3.0 & 35.4  & 10.14$\pm$0.04 & 0.991 & 3.23e+42 & 2.01  & 0.813 & 0.752 & 5.28e+09 & 4.98e+09 & \textsc{Galfit}   & 0.017$\pm$0.008 & 1.83e+07 & H\,{\sevensize II} & 5.7 \\ 
\rowcolor{White}
NGC3049                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.54$\pm$0.09 & 0.991 & 5.62e+40 & 2.65  & 0.929 & 0.752 & 1.05e+08 & 4.98e+09 & \textsc{Galfit}   & 0.017$\pm$0.008 & 1.83e+07 & H\,{\sevensize II} & 5.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3055                & Sersic + psfAgn          & Sersic         & disk  & 2.3 & 42.9  & 9.05 $\pm$0.04 & 0.990 & 1.64e+43 & 1.52  & 0.733 & 0.739 & 2.42e+10 & 2.49e+10 & \textsc{Galfit}   & 0.017$\pm$0.004 & 2.50e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{LightGray}
NGC3055                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.46$\pm$0.04 & 0.990 & 2.83e+41 & 1.35  & 0.708 & 0.739 & 4.03e+08 & 2.49e+10 & \textsc{Galfit}   & 0.017$\pm$0.004 & 2.50e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC2520                 & Sersic                   & Sersic         & disk  & 1.4 & 5.8   & 10.40$\pm$0.04 & 0.985 & 5.26e+42 & 2.01  & 0.813 & 0.805 & 8.60e+09 & 8.52e+09 & \textsc{Galfit}   & 0    $\pm$0     & 2.64e+07 & H\,{\sevensize II} & 8.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5403                & Sersic                   & Sersic         & mixed & 5.9 & 10.9  & 9.96 $\pm$0.04 & 0.981 & 1.23e+43 & NA    & NA    & 0.894 & ---   & 2.21e+10 & $C\mapsto$~B/T    & 0.187$\pm$0.050 & 3.30e+07 & H\,{\sevensize II} & 5.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC5459                & Sersic                   & Sersic         & disk  & 1.0 & 45.9  & 9.76 $\pm$0.04 & 0.993 & 9.14e+42 & 2.01  & 0.813 & 0.901 & 1.50e+10 & 1.66e+10 & \textsc{Galfit}   & 0    $\pm$0     & 2.58e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG5-24-022            & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.7   & 11.50$\pm$0.05 & 0.921 & 2.17e+43 & 2.93  & 0.985 & 0.877 & 4.30e+10 & 6.85e+10 & \textsc{Galfit}   & 0.559$\pm$0.080 & 9.21e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{LightGray}
MCG5-24-022            & Sersic + exDisk          & exDisk         & disk  & --- & 3.3   & 11.76$\pm$0.04 & 0.921 & 1.71e+43 & 2.03  & 0.816 & 0.877 & 2.81e+10 & 6.85e+10 & \textsc{Galfit}   & 0.559$\pm$0.080 & 9.21e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC2551                 & Sersic                   & Sersic         & mixed & 9.2 & 7.7   & 10.33$\pm$0.05 & 0.960 & 7.07e+43 & NA    & NA    & 0.789 & ---   & 1.12e+11 & $C\mapsto$~B/T    & 0.250$\pm$0.066 & 9.49e+07 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS10106+2745         & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 4.5   & 12.09$\pm$0.04 & 0.827 & 6.21e+43 & 2.39  & 0.880 & 0.994 & 1.10e+11 & 1.31e+11 & \textsc{Galfit}   & 0.051$\pm$0.014 & 2.16e+08 & H\,{\sevensize II} & 2.7 \\ 
\rowcolor{LightGray}
IRAS10106+2745         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.26$\pm$0.15 & 0.827 & 3.35e+42 & 3.88  & 1.202 & 0.994 & 8.10e+09 & 1.31e+11 & \textsc{Galfit}   & 0.051$\pm$0.014 & 2.16e+08 & H\,{\sevensize II} & 2.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3162                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 2.7   & 11.87$\pm$0.05 & 0.995 & 1.37e+42 & 1.34  & 0.706 & 0.755 & 1.95e+09 & 2.16e+10 & \textsc{Galfit}   & 0.096$\pm$0.030 & 2.64e+07 & H\,{\sevensize II} & 14.5\\ 
\rowcolor{White}
NGC3162                & Sersic + exDisk          & exDisk         & disk  & --- & 17.0  & 9.44 $\pm$0.04 & 0.995 & 1.29e+43 & 1.61  & 0.747 & 0.755 & 1.94e+10 & 2.16e+10 & \textsc{Galfit}   & 0.096$\pm$0.030 & 2.64e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS10120+1653         & Sersic                   & Sersic         & mixed & 4.2 & 1.9   & 13.49$\pm$0.07 & 0.452 & 5.39e+43 & NA    & NA    & 0.900 & ---   & 9.76e+10 & $C\mapsto$~B/T    & 0.128$\pm$0.034 & 5.17e+08 & LINER & 3.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3190                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 2.6   & 9.05 $\pm$0.04 & 0.984 & 1.82e+43 & 2.65  & 0.929 & 0.979 & 3.40e+10 & 1.32e+11 & \textsc{Galfit}   & 0.273$\pm$0.020 & 2.64e+07 & LINER & 22.2\\ 
\rowcolor{White}
NGC3190                & Sersic + exDisk          & exDisk         & disk  & --- & 17.5  & 7.99 $\pm$0.04 & 0.984 & 4.84e+43 & 2.01  & 0.813 & 0.979 & 7.92e+10 & 1.32e+11 & \textsc{Galfit}   & 0.273$\pm$0.020 & 2.64e+07 & LINER & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC602                  & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 9.9   & 10.53$\pm$0.03 & 0.983 & 2.22e+43 & 2.01  & 0.813 & 0.763 & 3.63e+10 & 3.50e+10 & \textsc{Galfit}   & 0.024$\pm$0.015 & 5.76e+07 & H\,{\sevensize II} & 8.3 \\ 
\rowcolor{LightGray}
IC602                  & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.57$\pm$0.07 & 0.983 & 5.37e+41 & 2.65  & 0.929 & 0.763 & 1.00e+09 & 3.50e+10 & \textsc{Galfit}   & 0.024$\pm$0.015 & 5.76e+07 & H\,{\sevensize II} & 8.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3191                & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 9.5   & 11.13$\pm$0.04 & 0.953 & 6.70e+43 & 1.57  & 0.741 & 0.804 & 9.99e+10 & 1.17e+11 & \textsc{Galfit}   & 0.072$\pm$0.014 & 1.34e+08 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
NGC3191                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.90$\pm$0.05 & 0.953 & 5.22e+42 & 3.48  & 1.106 & 0.804 & 1.16e+10 & 1.17e+11 & \textsc{Galfit}   & 0.072$\pm$0.014 & 1.34e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3206                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 29.4  & 10.49$\pm$0.05 & 0.996 & 4.68e+42 & 1.38  & 0.712 & 0.743 & 6.70e+09 & 6.99e+09 & \textsc{Galfit}   & 0.004$\pm$0.010 & 2.58e+07 & H\,{\sevensize II} & 2.8 \\ 
\rowcolor{LightGray}
NGC3206                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 16.40$\pm$0.24 & 0.996 & 2.02e+40 & 0.50  & 0.592 & 0.743 & 2.41e+07 & 6.99e+09 & \textsc{Galfit}   & 0.004$\pm$0.010 & 2.58e+07 & H\,{\sevensize II} & 2.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC5613                & Sersic                   & Sersic         & mixed & 1.9 & 6.0   & 10.82$\pm$0.04 & 0.899 & 9.15e+43 & NA    & NA    & 0.837 & ---   & 1.54e+11 & $C\mapsto$~B/T    & 0.190$\pm$0.050 & 1.40e+08 & H\,{\sevensize II} & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5644                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.5   & 12.62$\pm$0.05 & 0.953 & 1.79e+43 & 3.31  & 1.067 & 1.016 & 3.84e+10 & 1.96e+11 & \textsc{Galfit}   & 0.188$\pm$0.247 & 1.38e+08 & LINER & 1.7 \\ 
\rowcolor{LightGray}
UGC5644                & Sersic + exDisk          & exDisk         & disk  & --- & 7.2   & 11.03$\pm$0.04 & 0.953 & 7.74e+43 & 2.51  & 0.902 & 1.016 & 1.40e+11 & 1.96e+11 & \textsc{Galfit}   & 0.188$\pm$0.247 & 1.38e+08 & LINER & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3245                & Sersic + psfAgn          & Sersic         & disk  & 5.6 & 35.0  & 7.58 $\pm$0.04 & 0.991 & 4.45e+43 & 2.68  & 0.935 & 0.966 & 8.37e+10 & 8.90e+10 & \textsc{Galfit}   & 0.031$\pm$0.000 & 2.09e+07 & H\,{\sevensize II} & 2.0 \\ 
\rowcolor{White}
NGC3245                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.31$\pm$0.04 & 0.991 & 1.43e+42 & 3.15  & 1.032 & 0.966 & 2.97e+09 & 8.90e+10 & \textsc{Galfit}   & 0.031$\pm$0.000 & 2.09e+07 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS10246+2042         & Sersic + psfAgn          & Sersic         & disk  & 1.8 & 4.9   & 10.94$\pm$0.04 & 0.969 & 3.20e+43 & 2.18  & 0.842 & 0.796 & 5.42e+10 & 5.27e+10 & \textsc{Galfit}   & 0.030$\pm$0.008 & 8.42e+07 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{LightGray}
IRAS10246+2042         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.70$\pm$0.19 & 0.969 & 1.00e+42 & 2.93  & 0.985 & 0.796 & 1.98e+09 & 5.27e+10 & \textsc{Galfit}   & 0.030$\pm$0.008 & 8.42e+07 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG7-22-012            & Sersic + psfAgn          & Sersic         & disk  & 0.5 & 9.9   & 11.02$\pm$0.04 & 0.942 & 1.78e+43 & 2.24  & 0.853 & 0.851 & 3.06e+10 & 3.19e+10 & \textsc{Galfit}   & 0.043$\pm$0.016 & 6.60e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{White}
MCG7-22-012            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.38$\pm$0.06 & 0.942 & 8.05e+41 & 2.24  & 0.853 & 0.851 & 1.38e+09 & 3.19e+10 & \textsc{Galfit}   & 0.043$\pm$0.016 & 6.60e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS10276+1119         & Sersic                   & Sersic         & mixed & 6.0 & 2.3   & 12.21$\pm$0.07 & 0.829 & 8.83e+43 & NA    & NA    & 0.760 & ---   & 1.35e+11 & $C\mapsto$~B/T    & 0.192$\pm$0.051 & 2.71e+08 & H\,{\sevensize II} & 2.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3265                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 7.2   & 10.54$\pm$0.04 & 0.990 & 3.17e+42 & 1.75  & 0.770 & 0.780 & 4.91e+09 & 5.46e+09 & \textsc{Galfit}   & 0.086$\pm$0.023 & 2.18e+07 & H\,{\sevensize II} & 5.7 \\ 
\rowcolor{White}
NGC3265                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.11$\pm$0.06 & 0.990 & 2.97e+41 & 1.62  & 0.749 & 0.780 & 4.48e+08 & 5.46e+09 & \textsc{Galfit}   & 0.086$\pm$0.023 & 2.18e+07 & H\,{\sevensize II} & 5.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5713                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.9   & 11.80$\pm$0.04 & 0.956 & 1.82e+43 & 3.68  & 1.153 & 0.957 & 4.22e+10 & 1.18e+11 & \textsc{Galfit}   & 0.296$\pm$0.033 & 9.50e+07 & SN    & 2.3 \\ 
\rowcolor{LightGray}
UGC5713                & Sersic + exDisk          & exDisk         & disk  & --- & 9.9   & 10.86$\pm$0.04 & 0.956 & 4.33e+43 & 2.37  & 0.876 & 0.957 & 7.63e+10 & 1.18e+11 & \textsc{Galfit}   & 0.296$\pm$0.033 & 9.50e+07 & SN    & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3274                & Sersic                   & Sersic         & disk  & 1.3 & 21.9  & 10.64$\pm$0.04 & 0.997 & 6.13e+41 & 2.01  & 0.813 & 0.698 & 1.00e+09 & 8.60e+08 & \textsc{Galfit}   & 0    $\pm$0     & 1.00e+07 & H\,{\sevensize II} & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5720                & Sersic + psfAgn          & Sersic         & disk  & 5.9 & 16.2  & 10.09$\pm$0.05 & 0.990 & 4.04e+42 & 0.00  & 0.533 & 0.692 & 4.33e+09 & 5.62e+09 & \textsc{Galfit}   & 0.004$\pm$0.002 & 2.00e+07 & H\,{\sevensize II} & 4.3 \\ 
\rowcolor{LightGray}
UGC5720                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 16.16$\pm$0.49 & 0.990 & 1.51e+40 & 0.00  & 0.533 & 0.692 & 1.62e+07 & 5.62e+09 & \textsc{Galfit}   & 0.004$\pm$0.002 & 2.00e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
KUG1031+351            & Sersic                   & Sersic         & mixed & 3.6 & 9.1   & 10.70$\pm$0.04 & 0.860 & 4.45e+44 & NA    & NA    & 0.705 & ---   & 6.30e+11 & $C\mapsto$~B/T    & 0.126$\pm$0.033 & 2.98e+08 & H\,{\sevensize II} & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3306                & Sersic + psfAgn          & Sersic         & disk  & 1.2 & 8.0   & 10.46$\pm$0.04 & 0.976 & 1.54e+43 & 1.95  & 0.803 & 0.837 & 2.49e+10 & 2.64e+10 & \textsc{Galfit}   & 0.021$\pm$0.014 & 4.66e+07 & H\,{\sevensize II} & 8.3 \\ 
\rowcolor{LightGray}
NGC3306                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.65$\pm$0.16 & 0.976 & 3.24e+41 & 1.95  & 0.803 & 0.837 & 5.23e+08 & 2.64e+10 & \textsc{Galfit}   & 0.021$\pm$0.014 & 4.66e+07 & H\,{\sevensize II} & 8.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3323                & Sersic                   & Sersic         & disk  & 1.4 & 11.0  & 11.24$\pm$0.04 & 0.967 & 2.16e+43 & 2.01  & 0.813 & 0.736 & 3.53e+10 & 3.20e+10 & \textsc{Galfit}   & 0    $\pm$0     & 7.95e+07 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC2598                 & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.9   & 13.18$\pm$0.20 & 0.932 & 4.38e+42 & 3.61  & 1.136 & 0.797 & 1.00e+10 & 4.95e+10 & \textsc{Galfit}   & 0.142$\pm$0.079 & 8.91e+07 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{LightGray}
IC2598                 & Sersic + exDisk          & exDisk         & disk  & --- & 2.6   & 11.23$\pm$0.05 & 0.932 & 2.64e+43 & 2.55  & 0.910 & 0.797 & 4.83e+10 & 4.95e+10 & \textsc{Galfit}   & 0.142$\pm$0.079 & 8.91e+07 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3338                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 5.4   & 11.01$\pm$0.05 & 0.989 & 1.98e+42 & 3.26  & 1.056 & 0.879 & 4.21e+09 & 3.73e+10 & \textsc{Galfit}   & 0.094$\pm$0.027 & 2.14e+07 & LINER & 13.2\\ 
\rowcolor{White}
NGC3338                & Sersic + exDisk          & exDisk         & disk  & --- & 27.2  & 8.55 $\pm$0.04 & 0.989 & 1.91e+43 & 2.00  & 0.811 & 0.879 & 3.12e+10 & 3.73e+10 & \textsc{Galfit}   & 0.094$\pm$0.027 & 2.14e+07 & LINER & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3353                & Sersic                   & Sersic         & mixed & 1.9 & 9.4   & 10.60$\pm$0.04 & 0.996 & 1.63e+42 & NA    & NA    & 0.596 & ---   & 1.95e+09 & $C\mapsto$~B/T    & 0.142$\pm$0.038 & 1.60e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC5881                & Sersic                   & Sersic         & mixed & 7.7 & 8.3   & 10.26$\pm$0.06 & 0.972 & 7.33e+43 & NA    & NA    & 0.882 & ---   & 1.30e+11 & $C\mapsto$~B/T    & 0.189$\pm$0.050 & 9.30e+07 & H\,{\sevensize II} & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3370                & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 21.7  & 9.37 $\pm$0.03 & 0.991 & 8.57e+42 & 1.98  & 0.808 & 0.847 & 1.39e+10 & 1.49e+10 & \textsc{Galfit}   & 0.015$\pm$0.006 & 2.09e+07 & H\,{\sevensize II} & 14.5\\ 
\rowcolor{LightGray}
NGC3370                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.92$\pm$0.06 & 0.991 & 1.30e+41 & 3.47  & 1.103 & 0.847 & 2.89e+08 & 1.49e+10 & \textsc{Galfit}   & 0.015$\pm$0.006 & 2.09e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3381                & Sersic + psfAgn          & Sersic         & disk  & 1.3 & 23.4  & 10.32$\pm$0.04 & 0.984 & 5.36e+42 & 1.40  & 0.715 & 0.727 & 7.71e+09 & 7.92e+09 & \textsc{Galfit}   & 0.012$\pm$0.007 & 2.57e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{White}
NGC3381                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.07$\pm$0.06 & 0.984 & 6.75e+40 & -0.30 & 0.501 & 0.727 & 6.80e+07 & 7.92e+09 & \textsc{Galfit}   & 0.012$\pm$0.007 & 2.57e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC5941\_NED02         & Sersic + psfAgn          & Sersic         & disk  & 8.7 & 10.4  & 10.31$\pm$0.05 & 0.938 & 8.94e+43 & 2.50  & 0.901 & 0.843 & 1.62e+11 & 1.53e+11 & \textsc{Galfit}   & 0.007$\pm$0.007 & 1.07e+08 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
UGC5941\_NED02         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.65$\pm$0.39 & 0.938 & 6.54e+41 & 6.26  & 1.980 & 0.843 & 2.61e+09 & 1.53e+11 & \textsc{Galfit}   & 0.007$\pm$0.007 & 1.07e+08 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3413                & Sersic                   & Sersic         & disk  & 1.4 & 10.7  & 10.82$\pm$0.04 & 0.999 & 1.36e+42 & 2.01  & 0.813 & 0.721 & 2.22e+09 & 1.98e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.62e+07 & H\,{\sevensize II} & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3408                & Sersic + psfAgn          & Sersic         & disk  & 1.4 & 13.4  & 10.60$\pm$0.04 & 0.929 & 1.13e+44 & 1.86  & 0.788 & 0.822 & 1.79e+11 & 1.96e+11 & \textsc{Galfit}   & 0.042$\pm$0.013 & 1.38e+08 & H\,{\sevensize II} & 1.5 \\ 
\rowcolor{LightGray}
NGC3408                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.00$\pm$0.06 & 0.929 & 4.93e+42 & 2.04  & 0.818 & 0.822 & 8.11e+09 & 1.96e+11 & \textsc{Galfit}   & 0.042$\pm$0.013 & 1.38e+08 & H\,{\sevensize II} & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3430                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.5   & 12.22$\pm$0.05 & 0.988 & 1.14e+42 & 3.07  & 1.015 & 0.877 & 2.33e+09 & 4.45e+10 & \textsc{Galfit}   & 0.045$\pm$0.017 & 2.84e+07 & H\,{\sevensize II} & 22.2\\ 
\rowcolor{White}
NGC3430                & Sersic + exDisk          & exDisk         & disk  & --- & 19.3  & 8.91 $\pm$0.04 & 0.988 & 2.41e+43 & 1.89  & 0.792 & 0.877 & 3.84e+10 & 4.45e+10 & \textsc{Galfit}   & 0.045$\pm$0.017 & 2.84e+07 & H\,{\sevensize II} & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
CGCG95-055             & Sersic + psfAgn          & Sersic         & disk  & 3.2 & 7.7   & 11.58$\pm$0.06 & 0.982 & 1.68e+42 & 2.57  & 0.914 & 0.910 & 3.09e+09 & 3.53e+09 & \textsc{Galfit}   & 0.127$\pm$0.065 & 2.57e+07 & SN    & 1.5 \\ 
\rowcolor{LightGray}
CGCG95-055             & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.67$\pm$0.09 & 0.982 & 2.45e+41 & 3.93  & 1.215 & 0.910 & 5.99e+08 & 3.53e+09 & \textsc{Galfit}   & 0.127$\pm$0.065 & 2.57e+07 & SN    & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS10565+2448W        & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 0.7   & 11.46$\pm$0.04 & 0.905 & 8.96e+43 & 2.65  & 0.929 & 0.865 & 1.67e+11 & 1.56e+11 & \textsc{Galfit}   & 1.000$\pm$0.265 & 1.85e+08 & SN    & 15.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC6074                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.6   & 12.19$\pm$0.05 & 0.981 & 2.09e+42 & 3.53  & 1.117 & 1.002 & 4.70e+09 & 1.85e+10 & \textsc{Galfit}   & 0.227$\pm$0.073 & 3.80e+07 & H\,{\sevensize II} & 6.9 \\ 
\rowcolor{LightGray}
UGC6074                & Sersic + exDisk          & exDisk         & disk  & --- & 7.1   & 10.86$\pm$0.04 & 0.981 & 7.11e+42 & 2.15  & 0.837 & 1.002 & 1.20e+10 & 1.85e+10 & \textsc{Galfit}   & 0.227$\pm$0.073 & 3.80e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3495                & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 85.2  & 8.46 $\pm$0.03 & 0.992 & 1.39e+43 & 2.01  & 0.813 & 0.862 & 2.27e+10 & 2.41e+10 & \textsc{Galfit}   & 0.004$\pm$0.002 & 1.75e+07 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{White}
NGC3495                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.46$\pm$0.06 & 0.992 & 5.53e+40 & 2.65  & 0.929 & 0.862 & 1.03e+08 & 2.41e+10 & \textsc{Galfit}   & 0.004$\pm$0.002 & 1.75e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC6103                & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 10.6  & 10.95$\pm$0.04 & 0.951 & 3.69e+43 & 1.44  & 0.721 & 0.737 & 5.35e+10 & 6.53e+10 & \textsc{Galfit}   & 0.158$\pm$0.017 & 9.17e+07 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{LightGray}
UGC6103                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.77$\pm$0.04 & 0.951 & 6.91e+42 & 1.35  & 0.708 & 0.737 & 9.84e+09 & 6.53e+10 & \textsc{Galfit}   & 0.158$\pm$0.017 & 9.17e+07 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC6135                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 9.0   & 9.93 $\pm$0.04 & 0.961 & 9.38e+43 & 2.01  & 0.813 & 0.826 & 1.53e+11 & 1.60e+11 & \textsc{Galfit}   & 0.026$\pm$0.007 & 9.09e+07 & LINER & 4.8 \\ 
\rowcolor{White}
UGC6135                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.88$\pm$0.06 & 0.961 & 2.47e+42 & 4.47  & 1.361 & 0.826 & 6.76e+09 & 1.60e+11 & \textsc{Galfit}   & 0.026$\pm$0.007 & 9.09e+07 & LINER & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
CGCG241-078            & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 3.7   & 11.80$\pm$0.06 & 0.925 & 2.40e+43 & 2.75  & 0.949 & 0.889 & 4.58e+10 & 5.36e+10 & \textsc{Galfit}   & 0.195$\pm$0.072 & 1.11e+08 & H\,{\sevensize II} & 8.1 \\ 
\rowcolor{LightGray}
CGCG241-078            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.34$\pm$0.13 & 0.925 & 5.81e+42 & 2.62  & 0.923 & 0.889 & 1.08e+10 & 5.36e+10 & \textsc{Galfit}   & 0.195$\pm$0.072 & 1.11e+08 & H\,{\sevensize II} & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC676                  & Sersic + psfAgn          & Sersic         & disk  & 3.0 & 21.8  & 9.70 $\pm$0.04 & 0.986 & 1.04e+43 & 1.96  & 0.804 & 0.809 & 1.68e+10 & 1.73e+10 & \textsc{Galfit}   & 0.016$\pm$0.006 & 2.69e+07 & H\,{\sevensize II} & 5.7 \\ 
\rowcolor{White}
IC676                  & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.17$\pm$0.09 & 0.986 & 1.70e+41 & -0.48 & 0.482 & 0.809 & 1.65e+08 & 1.73e+10 & \textsc{Galfit}   & 0.016$\pm$0.006 & 2.69e+07 & H\,{\sevensize II} & 5.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS11102+3026         & Sersic                   & Sersic         & mixed & 2.0 & 2.7   & 12.22$\pm$0.04 & 0.936 & 2.25e+43 & NA    & NA    & 0.916 & ---   & 4.15e+10 & $C\mapsto$~B/T    & 0.130$\pm$0.034 & 1.30e+08 & LINER & 7.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC2637                 & Sersic                   & Sersic         & mixed & 5.4 & 11.9  & 10.15$\pm$0.04 & 0.930 & 1.47e+44 & NA    & NA    & 0.795 & ---   & 2.36e+11 & $C\mapsto$~B/T    & 0.188$\pm$0.050 & 1.28e+08 & SN    & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG9-19-013            & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.9   & 13.07$\pm$0.10 & 0.852 & 2.27e+43 & 3.20  & 1.043 & 0.918 & 4.76e+10 & 1.01e+11 & \textsc{Galfit}   & 0.417$\pm$0.165 & 2.02e+08 & TO    & 2.7 \\ 
\rowcolor{LightGray}
MCG9-19-013            & Sersic + exDisk          & exDisk         & disk  & --- & 2.8   & 12.71$\pm$0.05 & 0.852 & 3.17e+43 & 1.93  & 0.799 & 0.918 & 5.10e+10 & 1.01e+11 & \textsc{Galfit}   & 0.417$\pm$0.165 & 2.02e+08 & TO    & 2.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
2MASXJ11193404+5335181 & Sersic$^{n=1}$           & Sersic$^{n=1}$ & disk  & 1.0 & 1.1   & 12.26$\pm$0.04 & 0.625 & 1.73e+44 & 2.01  & 0.813 & 0.821 & 2.83e+11 & 2.85e+11 & \textsc{Galfit}   & 0    $\pm$0     & 4.47e+08 & NA    & 6.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3633                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.9   & 11.74$\pm$0.04 & 0.980 & 1.97e+42 & 3.57  & 1.127 & 0.928 & 4.47e+09 & 2.06e+10 & \textsc{Galfit}   & 0.178$\pm$0.067 & 3.00e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{LightGray}
NGC3633                & Sersic + exDisk          & exDisk         & disk  & --- & 7.3   & 10.08$\pm$0.03 & 0.980 & 9.08e+42 & 2.47  & 0.895 & 0.928 & 1.64e+10 & 2.06e+10 & \textsc{Galfit}   & 0.178$\pm$0.067 & 3.00e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3652                & Sersic + psfAgn          & Sersic         & disk  & 1.2 & 22.5  & 10.21$\pm$0.04 & 0.985 & 2.16e+42 & 1.13  & 0.676 & 0.734 & 2.94e+09 & 3.22e+09 & \textsc{Galfit}   & 0.007$\pm$0.011 & 1.55e+07 & H\,{\sevensize II} & 4.7 \\ 
\rowcolor{White}
NGC3652                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.60$\pm$0.13 & 0.985 & 1.51e+40 & 2.84  & 0.967 & 0.734 & 2.94e+07 & 3.22e+09 & \textsc{Galfit}   & 0.007$\pm$0.011 & 1.55e+07 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3656                & Sersic + psfAgn          & Sersic         & disk  & 3.1 & 17.0  & 9.09 $\pm$0.04 & 0.979 & 3.43e+43 & 2.94  & 0.988 & 1.012 & 6.82e+10 & 7.19e+10 & \textsc{Galfit}   & 0.025$\pm$0.011 & 3.70e+07 & LINER & 12.1\\ 
\rowcolor{LightGray}
NGC3656                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.05$\pm$0.06 & 0.979 & 8.95e+41 & 2.94  & 0.988 & 1.012 & 1.78e+09 & 7.19e+10 & \textsc{Galfit}   & 0.025$\pm$0.011 & 3.70e+07 & LINER & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3659                & Sersic + psfAgn          & Sersic         & disk  & 0.8 & 15.6  & 10.45$\pm$0.04 & 0.995 & 3.21e+42 & 1.51  & 0.732 & 0.741 & 4.73e+09 & 4.83e+09 & \textsc{Galfit}   & 0.009$\pm$0.006 & 2.10e+07 & H\,{\sevensize II} & 4.6 \\ 
\rowcolor{White}
NGC3659                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.55$\pm$0.11 & 0.995 & 2.93e+40 & 1.72  & 0.765 & 0.741 & 4.51e+07 & 4.83e+09 & \textsc{Galfit}   & 0.009$\pm$0.006 & 2.10e+07 & H\,{\sevensize II} & 4.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3664                & Sersic                   & Sersic         & disk  & 0.5 & 11.5  & 12.43$\pm$0.05 & 0.995 & 8.50e+41 & 2.01  & 0.813 & 0.733 & 1.39e+09 & 1.25e+09 & \textsc{Galfit}   & 0    $\pm$0     & 2.69e+07 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3666                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 7.2   & 11.53$\pm$0.09 & 0.992 & 7.14e+41 & 4.54  & 1.381 & 0.843 & 1.98e+09 & 9.97e+09 & \textsc{Galfit}   & 0.121$\pm$0.048 & 1.63e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{White}
NGC3666                & Sersic + exDisk          & exDisk         & disk  & --- & 16.4  & 9.38 $\pm$0.03 & 0.992 & 5.17e+42 & 1.96  & 0.804 & 0.843 & 8.36e+09 & 9.97e+09 & \textsc{Galfit}   & 0.121$\pm$0.048 & 1.63e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC691                  & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 2.8   & 11.02$\pm$0.04 & 0.990 & 1.10e+42 & 2.65  & 0.929 & 0.722 & 2.06e+09 & 1.59e+09 & \textsc{Galfit}   & 1.000$\pm$0.265 & 1.60e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3686                & Sersic + psfAgn          & Sersic         & disk  & 1.4 & 51.2  & 8.10 $\pm$0.04 & 0.990 & 2.78e+43 & 1.82  & 0.781 & 0.770 & 4.37e+10 & 4.35e+10 & \textsc{Galfit}   & 0.012$\pm$0.001 & 2.10e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{White}
NGC3686                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.85$\pm$0.04 & 0.990 & 3.50e+41 & 0.82  & 0.633 & 0.770 & 4.46e+08 & 4.35e+10 & \textsc{Galfit}   & 0.012$\pm$0.001 & 2.10e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC6469                & Sersic                   & Sersic         & disk  & 1.5 & 7.2   & 11.37$\pm$0.04 & 0.977 & 3.23e+43 & 2.01  & 0.813 & 0.744 & 5.28e+10 & 4.83e+10 & \textsc{Galfit}   & 0    $\pm$0     & 1.03e+08 & H\,{\sevensize II} & 7.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC698                  & Sersic + psfAgn          & Sersic         & disk  & 1.3 & 7.8   & 10.26$\pm$0.03 & 0.931 & 7.61e+43 & 2.30  & 0.864 & 0.855 & 1.32e+11 & 1.40e+11 & \textsc{Galfit}   & 0.060$\pm$0.015 & 9.68e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{White}
IC698                  & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.25$\pm$0.05 & 0.931 & 4.85e+42 & 3.53  & 1.117 & 0.855 & 1.09e+10 & 1.40e+11 & \textsc{Galfit}   & 0.060$\pm$0.015 & 9.68e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS11267+1558         & Sersic                   & Sersic         & disk  & 0.2 & 0.7   & 14.21$\pm$0.06 & 0.743 & 9.25e+43 & 2.01  & 0.813 & 0.683 & 1.51e+11 & 1.27e+11 & \textsc{Galfit}   & 0    $\pm$0     & 7.37e+08 & H\,{\sevensize II} & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3705                & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 28.2  & 7.96 $\pm$0.03 & 0.993 & 1.91e+43 & 2.46  & 0.893 & 0.707 & 3.43e+10 & 2.82e+10 & \textsc{Galfit}   & 0.037$\pm$0.004 & 1.63e+07 & LINER & 13.2\\ 
\rowcolor{White}
NGC3705                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.50$\pm$0.03 & 0.993 & 7.34e+41 & 4.49  & 1.366 & 0.707 & 2.02e+09 & 2.82e+10 & \textsc{Galfit}   & 0.037$\pm$0.004 & 1.63e+07 & LINER & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG3-29-061            & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 8.7   & 11.27$\pm$0.04 & 0.963 & 1.51e+43 & 2.13  & 0.833 & 0.844 & 2.53e+10 & 2.81e+10 & \textsc{Galfit}   & 0.085$\pm$0.024 & 6.75e+07 & H\,{\sevensize II} & 6.9 \\ 
\rowcolor{LightGray}
MCG3-29-061            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.85$\pm$0.06 & 0.963 & 1.40e+42 & 2.13  & 0.833 & 0.844 & 2.35e+09 & 2.81e+10 & \textsc{Galfit}   & 0.085$\pm$0.024 & 6.75e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3720                & Sersic                   & Sersic         & mixed & 3.4 & 18.8  & 9.26 $\pm$0.04 & 0.960 & 1.69e+44 & NA    & NA    & 0.871 & ---   & 2.97e+11 & $C\mapsto$~B/T    & 0.089$\pm$0.024 & 8.98e+07 & H\,{\sevensize II} & 4.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3729                & Sersic + psfAgn          & Sersic         & disk  & 1.5 & 43.3  & 8.31 $\pm$0.04 & 0.999 & 1.53e+43 & 2.04  & 0.818 & 0.841 & 2.52e+10 & 2.64e+10 & \textsc{Galfit}   & 0.018$\pm$0.004 & 1.71e+07 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{LightGray}
NGC3729                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.66$\pm$0.04 & 0.999 & 2.79e+41 & 2.49  & 0.899 & 0.841 & 5.05e+08 & 2.64e+10 & \textsc{Galfit}   & 0.018$\pm$0.004 & 1.71e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG10-17-019           & Sersic + psfAgn          & Sersic         & disk  & 2.2 & 6.6   & 10.89$\pm$0.04 & 0.942 & 7.48e+43 & 2.07  & 0.823 & 0.828 & 1.24e+11 & 1.29e+11 & \textsc{Galfit}   & 0.033$\pm$0.016 & 1.28e+08 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{White}
MCG10-17-019           & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.55$\pm$0.14 & 0.942 & 2.57e+42 & 2.07  & 0.823 & 0.828 & 4.26e+09 & 1.29e+11 & \textsc{Galfit}   & 0.033$\pm$0.016 & 1.28e+08 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3758                & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 10.1  & 10.64$\pm$0.04 & 0.878 & 9.34e+43 & 1.81  & 0.779 & 0.805 & 1.46e+11 & 2.17e+11 & \textsc{Galfit}   & 0.302$\pm$0.067 & 1.32e+08 & SN    & 4.8 \\ 
\rowcolor{LightGray}
NGC3758                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.55$\pm$0.04 & 0.878 & 4.04e+43 & 0.90  & 0.644 & 0.805 & 5.23e+10 & 2.17e+11 & \textsc{Galfit}   & 0.302$\pm$0.067 & 1.32e+08 & SN    & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC6583                & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 6.0   & 11.29$\pm$0.04 & 0.970 & 2.85e+43 & 1.44  & 0.721 & 0.742 & 4.13e+10 & 4.66e+10 & \textsc{Galfit}   & 0.086$\pm$0.032 & 9.32e+07 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
UGC6583                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.85$\pm$0.05 & 0.970 & 2.69e+42 & 1.34  & 0.706 & 0.742 & 3.82e+09 & 4.66e+10 & \textsc{Galfit}   & 0.086$\pm$0.032 & 9.32e+07 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG1-30-003            & Sersic + psfAgn          & Sersic         & disk  & 0.4 & 6.2   & 12.18$\pm$0.03 & 0.924 & 2.28e+43 & 1.84  & 0.784 & 0.727 & 3.60e+10 & 4.02e+10 & \textsc{Galfit}   & 0.169$\pm$0.065 & 1.29e+08 & H\,{\sevensize II} & 7.0 \\ 
\rowcolor{LightGray}
MCG1-30-003            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.91$\pm$0.04 & 0.924 & 4.64e+42 & 2.66  & 0.931 & 0.727 & 8.69e+09 & 4.02e+10 & \textsc{Galfit}   & 0.169$\pm$0.065 & 1.29e+08 & H\,{\sevensize II} & 7.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3769                & Sersic + psfAgn          & Sersic         & disk  & 1.2 & 26.4  & 9.21 $\pm$0.04 & 0.993 & 6.66e+42 & 1.74  & 0.768 & 0.801 & 1.03e+10 & 1.08e+10 & \textsc{Galfit}   & 0.010$\pm$0.004 & 1.71e+07 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{White}
NGC3769                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.20$\pm$0.05 & 0.993 & 6.72e+40 & 1.92  & 0.797 & 0.801 & 1.08e+08 & 1.08e+10 & \textsc{Galfit}   & 0.010$\pm$0.004 & 1.71e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3773                & Sersic + psfAgn          & Sersic         & disk  & 3.9 & 22.4  & 10.27$\pm$0.05 & 0.995 & 2.28e+42 & 2.01  & 0.813 & 0.729 & 3.73e+09 & 3.41e+09 & \textsc{Galfit}   & 0.022$\pm$0.011 & 1.63e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{LightGray}
NGC3773                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.39$\pm$0.08 & 0.995 & 5.14e+40 & 2.65  & 0.929 & 0.729 & 9.61e+07 & 3.41e+09 & \textsc{Galfit}   & 0.022$\pm$0.011 & 1.63e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3781                & Sersic                   & Sersic         & mixed & 8.3 & 8.4   & 10.10$\pm$0.04 & 0.937 & 1.01e+44 & NA    & NA    & 0.922 & ---   & 1.88e+11 & $C\mapsto$~B/T    & 0.166$\pm$0.044 & 1.04e+08 & SN    & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC6625                & Sersic + psfAgn + exDisk & Sersic         & bulge & 4.0 & 8.2   & 11.45$\pm$0.09 & 0.927 & 6.76e+43 & 3.27  & 1.058 & 0.811 & 1.44e+11 & 1.92e+11 & \textsc{Galfit}   & 0.573$\pm$0.090 & 1.58e+08 & TO    & 5.0 \\ 
\rowcolor{LightGray}
UGC6625                & Sersic + psfAgn + exDisk & psfAgn         & AGN   & --- & ---   & 14.43$\pm$0.11 & 0.927 & 4.34e+42 & NA    & NA    & 0.811 & ---   & 1.92e+11 & \textsc{Galfit}   & 0.573$\pm$0.090 & 1.58e+08 & TO    & 5.0 \\ 
\rowcolor{LightGray}
UGC6625                & Sersic + psfAgn + exDisk & exDisk         & disk  & --- & 5.9   & 11.77$\pm$0.07 & 0.927 & 5.03e+43 & 1.32  & 0.703 & 0.811 & 7.11e+10 & 1.92e+11 & \textsc{Galfit}   & 0.573$\pm$0.090 & 1.58e+08 & TO    & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3808\_NED02         & Sersic + psfAgn          & Sersic         & disk  & 2.2 & 4.5   & 11.58$\pm$0.04 & 0.944 & 2.81e+43 & 1.77  & 0.773 & 0.747 & 4.37e+10 & 4.75e+10 & \textsc{Galfit}   & 0.109$\pm$0.029 & 1.07e+08 & H\,{\sevensize II} & 4.0 \\ 
\rowcolor{White}
NGC3808\_NED02         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.86$\pm$0.06 & 0.944 & 3.44e+42 & 1.58  & 0.743 & 0.747 & 5.14e+09 & 4.75e+10 & \textsc{Galfit}   & 0.109$\pm$0.029 & 1.07e+08 & H\,{\sevensize II} & 4.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3811                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.1   & 11.34$\pm$0.04 & 0.977 & 9.26e+42 & 2.43  & 0.887 & 0.885 & 1.65e+10 & 6.94e+10 & \textsc{Galfit}   & 0.237$\pm$0.033 & 5.42e+07 & H\,{\sevensize II} & 14.5\\ 
\rowcolor{LightGray}
NGC3811                & Sersic + exDisk          & exDisk         & disk  & --- & 12.6  & 10.07$\pm$0.04 & 0.977 & 2.98e+43 & 1.99  & 0.809 & 0.885 & 4.85e+10 & 6.94e+10 & \textsc{Galfit}   & 0.237$\pm$0.033 & 5.42e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3822                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 9.5   & 9.60 $\pm$0.03 & 0.936 & 1.34e+44 & 2.28  & 0.860 & 0.873 & 2.32e+11 & 2.49e+11 & \textsc{Galfit}   & 0.050$\pm$0.013 & 9.46e+07 & SN    & 8.7 \\ 
\rowcolor{White}
NGC3822                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.79$\pm$0.05 & 0.936 & 7.11e+42 & 1.92  & 0.797 & 0.873 & 1.14e+10 & 2.49e+11 & \textsc{Galfit}   & 0.050$\pm$0.013 & 9.46e+07 & SN    & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC6665                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 2.5   & 11.89$\pm$0.07 & 0.964 & 1.35e+43 & 2.65  & 0.929 & 0.643 & 2.52e+10 & 2.99e+10 & \textsc{Galfit}   & 0.584$\pm$0.122 & 8.50e+07 & H\,{\sevensize II} & 8.1 \\ 
\rowcolor{LightGray}
UGC6665                & Sersic + exDisk          & exDisk         & disk  & --- & 2.4   & 12.26$\pm$0.06 & 0.964 & 9.62e+42 & 2.01  & 0.813 & 0.643 & 1.57e+10 & 2.99e+10 & \textsc{Galfit}   & 0.584$\pm$0.122 & 8.50e+07 & H\,{\sevensize II} & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG3-30-051            & Sersic                   & Sersic         & disk  & 1.2 & 5.2   & 11.15$\pm$0.04 & 0.956 & 3.00e+43 & 2.01  & 0.813 & 0.832 & 4.91e+10 & 5.03e+10 & \textsc{Galfit}   & 0    $\pm$0     & 9.04e+07 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3839                & Sersic + psfAgn          & Sersic         & disk  & 1.3 & 8.3   & 10.71$\pm$0.03 & 0.946 & 4.54e+43 & 1.69  & 0.760 & 0.743 & 6.94e+10 & 7.04e+10 & \textsc{Galfit}   & 0.039$\pm$0.021 & 9.13e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
NGC3839                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.19$\pm$0.09 & 0.946 & 1.84e+42 & 1.76  & 0.771 & 0.743 & 2.85e+09 & 7.04e+10 & \textsc{Galfit}   & 0.039$\pm$0.021 & 9.13e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC6732                & Sersic + psfAgn          & Sersic         & disk  & 1.8 & 4.9   & 10.31$\pm$0.04 & 0.978 & 2.34e+43 & 2.14  & 0.835 & 0.820 & 3.93e+10 & 4.27e+10 & \textsc{Galfit}   & 0.094$\pm$0.018 & 5.36e+07 & LINER & 2.3 \\ 
\rowcolor{White}
UGC6732                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.77$\pm$0.06 & 0.978 & 2.43e+42 & 2.55  & 0.910 & 0.820 & 4.45e+09 & 4.27e+10 & \textsc{Galfit}   & 0.094$\pm$0.018 & 5.36e+07 & LINER & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC730                  & Sersic + psfAgn          & Sersic         & disk  & 2.7 & 5.8   & 10.41$\pm$0.04 & 0.931 & 6.13e+43 & 2.98  & 0.996 & 0.935 & 1.23e+11 & 1.28e+11 & \textsc{Galfit}   & 0.097$\pm$0.034 & 9.31e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
IC730                  & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.83$\pm$0.09 & 0.931 & 6.60e+42 & 3.07  & 1.015 & 0.935 & 1.35e+10 & 1.28e+11 & \textsc{Galfit}   & 0.097$\pm$0.034 & 9.31e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC732\_NED01           & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.3   & 12.36$\pm$0.09 & 0.905 & 1.38e+43 & 2.47  & 0.895 & 0.896 & 2.49e+10 & 5.15e+10 & \textsc{Galfit}   & 0.484$\pm$0.144 & 1.10e+08 & H\,{\sevensize II} & 8.4 \\ 
\rowcolor{White}
IC732\_NED01           & Sersic + exDisk          & exDisk         & disk  & --- & 3.7   & 12.29$\pm$0.07 & 0.905 & 1.47e+43 & 2.36  & 0.875 & 0.896 & 2.59e+10 & 5.15e+10 & \textsc{Galfit}   & 0.484$\pm$0.144 & 1.10e+08 & H\,{\sevensize II} & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3912                & Sersic + psfAgn          & Sersic         & disk  & 1.3 & 17.5  & 9.99 $\pm$0.04 & 0.989 & 5.60e+42 & 1.57  & 0.741 & 0.780 & 8.35e+09 & 8.94e+09 & \textsc{Galfit}   & 0.022$\pm$0.006 & 2.25e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{LightGray}
NGC3912                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.12$\pm$0.04 & 0.989 & 1.25e+41 & 1.25  & 0.693 & 0.780 & 1.74e+08 & 8.94e+09 & \textsc{Galfit}   & 0.022$\pm$0.006 & 2.25e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC3928                & Sersic                   & Sersic         & mixed & 3.7 & 8.0   & 9.70 $\pm$0.04 & 0.993 & 4.14e+42 & NA    & NA    & 0.773 & ---   & 6.44e+09 & $C\mapsto$~B/T    & 0.179$\pm$0.047 & 1.69e+07 & H\,{\sevensize II} & 4.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC3934                & Sersic                   & Sersic         & mixed & 4.9 & 11.0  & 10.20$\pm$0.04 & 0.956 & 3.34e+43 & NA    & NA    & 0.907 & ---   & 6.10e+10 & $C\mapsto$~B/T    & 0.119$\pm$0.032 & 6.16e+07 & LINER & 5.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC6865                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 2.7   & 11.59$\pm$0.05 & 0.965 & 2.06e+43 & 4.56  & 1.387 & 1.030 & 5.75e+10 & 1.70e+11 & \textsc{Galfit}   & 0.253$\pm$0.026 & 9.12e+07 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{White}
UGC6865                & Sersic + exDisk          & exDisk         & disk  & --- & 11.6  & 10.41$\pm$0.04 & 0.965 & 6.09e+43 & 2.40  & 0.882 & 1.030 & 1.08e+11 & 1.70e+11 & \textsc{Galfit}   & 0.253$\pm$0.026 & 9.12e+07 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC6901                & Sersic                   & Sersic         & mixed & 2.4 & 7.5   & 10.49$\pm$0.04 & 0.951 & 7.77e+43 & NA    & NA    & 0.836 & ---   & 1.31e+11 & $C\mapsto$~B/T    & 0.167$\pm$0.044 & 1.08e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
CGCG013-010            & Sersic                   & Sersic         & mixed & 2.3 & 4.4   & 10.90$\pm$0.03 & 0.906 & 1.30e+44 & NA    & NA    & 0.957 & ---   & 2.50e+11 & $C\mapsto$~B/T    & 0.151$\pm$0.040 & 1.72e+08 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4014                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 11.1  & 9.55 $\pm$0.04 & 0.968 & 6.36e+43 & 2.26  & 0.856 & 0.932 & 1.10e+11 & 1.21e+11 & \textsc{Galfit}   & 0.018$\pm$0.003 & 6.26e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{LightGray}
NGC4014                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.92$\pm$0.08 & 0.968 & 1.14e+42 & 5.44  & 1.667 & 0.932 & 3.82e+09 & 1.21e+11 & \textsc{Galfit}   & 0.018$\pm$0.003 & 6.26e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4010                & Sersic                   & Sersic         & disk  & 1.3 & 53.9  & 9.35 $\pm$0.04 & 0.989 & 5.83e+42 & 2.01  & 0.813 & 0.468 & 9.54e+09 & 5.49e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.71e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4018                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 5.3   & 12.60$\pm$0.09 & 0.939 & 5.00e+42 & 2.20  & 0.846 & 0.812 & 8.51e+09 & 5.50e+10 & \textsc{Galfit}   & 0.149$\pm$0.040 & 7.26e+07 & H\,{\sevensize II} & 5.5 \\ 
\rowcolor{LightGray}
NGC4018                & Sersic + exDisk          & exDisk         & disk  & --- & 8.6   & 10.71$\pm$0.04 & 0.939 & 2.85e+43 & 1.81  & 0.779 & 0.812 & 4.47e+10 & 5.50e+10 & \textsc{Galfit}   & 0.149$\pm$0.040 & 7.26e+07 & H\,{\sevensize II} & 5.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4020                & Sersic + psfAgn          & Sersic         & disk  & 0.6 & 26.4  & 10.50$\pm$0.04 & 0.996 & 1.42e+42 & 1.54  & 0.736 & 0.766 & 2.10e+09 & 2.21e+09 & \textsc{Galfit}   & 0.005$\pm$0.018 & 1.43e+07 & LINER & 1.0 \\ 
\rowcolor{White}
NGC4020                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 16.16$\pm$0.16 & 0.996 & 7.75e+39 & 3.66  & 1.148 & 0.766 & 1.79e+07 & 2.21e+09 & \textsc{Galfit}   & 0.005$\pm$0.018 & 1.43e+07 & LINER & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS11571+3003         & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 4.8   & 13.16$\pm$0.06 & 0.921 & 2.65e+43 & 2.35  & 0.873 & 0.880 & 4.65e+10 & 7.11e+10 & \textsc{Galfit}   & 0.338$\pm$0.090 & 2.19e+08 & H\,{\sevensize II} & 4.5 \\ 
\rowcolor{LightGray}
IRAS11571+3003         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.89$\pm$0.07 & 0.921 & 1.35e+43 & 3.43  & 1.094 & 0.880 & 2.97e+10 & 7.11e+10 & \textsc{Galfit}   & 0.338$\pm$0.090 & 2.19e+08 & H\,{\sevensize II} & 4.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC7017                & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 8.4   & 10.57$\pm$0.04 & 0.964 & 1.92e+43 & 1.98  & 0.808 & 0.798 & 3.12e+10 & 3.33e+10 & \textsc{Galfit}   & 0.068$\pm$0.011 & 5.52e+07 & H\,{\sevensize II} & 8.3 \\ 
\rowcolor{White}
UGC7017                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.42$\pm$0.05 & 0.964 & 1.39e+42 & 2.10  & 0.828 & 0.798 & 2.32e+09 & 3.33e+10 & \textsc{Galfit}   & 0.068$\pm$0.011 & 5.52e+07 & H\,{\sevensize II} & 8.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC7016                & Sersic + psfAgn          & Sersic         & disk  & 2.4 & 15.7  & 9.97 $\pm$0.04 & 0.936 & 1.30e+44 & 2.56  & 0.912 & 0.926 & 2.39e+11 & 2.58e+11 & \textsc{Galfit}   & 0.061$\pm$0.008 & 1.10e+08 & SN    & 3.8 \\ 
\rowcolor{LightGray}
UGC7016                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.93$\pm$0.04 & 0.936 & 8.49e+42 & 2.77  & 0.953 & 0.926 & 1.63e+10 & 2.58e+11 & \textsc{Galfit}   & 0.061$\pm$0.008 & 1.10e+08 & SN    & 3.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG3-31-030            & Sersic                   & Sersic         & disk  & 0.6 & 9.1   & 11.38$\pm$0.04 & 0.996 & 5.31e+41 & 2.01  & 0.813 & 0.732 & 8.69e+08 & 7.82e+08 & \textsc{Galfit}   & 0    $\pm$0     & 1.31e+07 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4062                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 4.8   & 11.95$\pm$0.06 & 0.993 & 4.85e+41 & 3.47  & 1.103 & 0.839 & 1.08e+09 & 3.00e+10 & \textsc{Galfit}   & 0.027$\pm$0.007 & 1.63e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
NGC4062                & Sersic + exDisk          & exDisk         & disk  & --- & 34.8  & 8.07 $\pm$0.04 & 0.993 & 1.73e+43 & 2.11  & 0.830 & 0.839 & 2.89e+10 & 3.00e+10 & \textsc{Galfit}   & 0.027$\pm$0.007 & 1.63e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4064                & Sersic                   & Sersic         & mixed & 2.1 & 32.7  & 8.63 $\pm$0.04 & 0.997 & 2.82e+42 & NA    & NA    & 0.900 & ---   & 5.10e+09 & $C\mapsto$~B/T    & 0.122$\pm$0.032 & 8.50e+06 & H\,{\sevensize II} & 3.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
CGCG098-059            & Sersic + psfAgn          & Sersic         & disk  & 1.9 & 5.2   & 10.99$\pm$0.04 & 0.935 & 4.35e+43 & 2.04  & 0.818 & 0.841 & 7.16e+10 & 8.53e+10 & \textsc{Galfit}   & 0.137$\pm$0.035 & 1.02e+08 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{LightGray}
CGCG098-059            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.99$\pm$0.06 & 0.935 & 6.90e+42 & 2.22  & 0.849 & 0.841 & 1.18e+10 & 8.53e+10 & \textsc{Galfit}   & 0.137$\pm$0.035 & 1.02e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4116                & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 31.0  & 10.61$\pm$0.04 & 0.998 & 1.61e+42 & 2.65  & 0.929 & 0.806 & 3.01e+09 & 2.62e+09 & \textsc{Galfit}   & 1.000$\pm$0.265 & 1.60e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4136                & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 26.8  & 9.76 $\pm$0.04 & 0.991 & 3.64e+42 & 1.76  & 0.771 & 0.823 & 5.65e+09 & 6.31e+09 & \textsc{Galfit}   & 0.044$\pm$0.008 & 1.63e+07 & H\,{\sevensize II} & 1.7 \\ 
\rowcolor{LightGray}
NGC4136                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.10$\pm$0.04 & 0.991 & 1.68e+41 & 1.01  & 0.659 & 0.823 & 2.23e+08 & 6.31e+09 & \textsc{Galfit}   & 0.044$\pm$0.008 & 1.63e+07 & H\,{\sevensize II} & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4150                & Sersic + psfAgn          & Sersic         & disk  & 3.6 & 19.6  & 8.79 $\pm$0.04 & 0.994 & 6.30e+42 & 2.22  & 0.849 & 0.881 & 1.08e+10 & 1.22e+10 & \textsc{Galfit}   & 0.086$\pm$0.022 & 1.37e+07 & SN    & 1.0 \\ 
\rowcolor{White}
NGC4150                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.36$\pm$0.04 & 0.994 & 5.90e+41 & 3.01  & 1.002 & 0.881 & 1.19e+09 & 1.22e+10 & \textsc{Galfit}   & 0.086$\pm$0.022 & 1.37e+07 & SN    & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS12086+1441         & Sersic                   & Sersic         & disk  & 1.1 & 2.0   & 12.94$\pm$0.04 & 0.983 & 1.25e+41 & 2.01  & 0.813 & 0.783 & 2.04e+08 & 1.96e+08 & \textsc{Galfit}   & 0    $\pm$0     & 1.31e+07 & H\,{\sevensize II} & 5.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4162                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.2   & 12.00$\pm$0.05 & 0.983 & 3.12e+42 & 3.46  & 1.101 & 0.864 & 6.91e+09 & 6.45e+10 & \textsc{Galfit}   & 0.084$\pm$0.035 & 4.25e+07 & H\,{\sevensize II} & 22.2\\ 
\rowcolor{White}
NGC4162                & Sersic + exDisk          & exDisk         & disk  & --- & 11.0  & 9.41 $\pm$0.04 & 0.983 & 3.39e+43 & 1.83  & 0.783 & 0.864 & 5.34e+10 & 6.45e+10 & \textsc{Galfit}   & 0.084$\pm$0.035 & 4.25e+07 & H\,{\sevensize II} & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4178                & Sersic + psfAgn          & Sersic         & disk  & 2.2 & 103.5 & 8.83 $\pm$0.04 & 1.005 & 9.23e+42 & 1.65  & 0.754 & 0.797 & 1.40e+10 & 1.48e+10 & \textsc{Galfit}   & 0    $\pm$0     & 1.68e+07 & H\,{\sevensize II} & 14.5\\ 
\rowcolor{LightGray}
NGC4178                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 18.30$\pm$2.04 & 1.005 & 1.50e+39 & 2.74  & 0.947 & 0.797 & 2.86e+06 & 1.48e+10 & \textsc{Galfit}   & 0    $\pm$0     & 1.68e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS12112+0305         & Sersic                   & Sersic         & disk  & 0.2 & 2.3   & 12.86$\pm$0.03 & 0.821 & 6.02e+43 & 2.01  & 0.813 & 0.788 & 9.85e+10 & 9.54e+10 & \textsc{Galfit}   & 0    $\pm$0     & 3.04e+08 & SN    & 15.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4189                & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 38.4  & 8.95 $\pm$0.04 & 0.990 & 8.14e+42 & 2.00  & 0.811 & 0.848 & 1.33e+10 & 1.43e+10 & \textsc{Galfit}   & 0.028$\pm$0.003 & 1.68e+07 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{LightGray}
NGC4189                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.80$\pm$0.04 & 0.990 & 2.35e+41 & 2.21  & 0.847 & 0.848 & 4.00e+08 & 1.43e+10 & \textsc{Galfit}   & 0.028$\pm$0.003 & 1.68e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4194                & Sersic + psfAgn          & Sersic         & disk  & 5.0 & 5.9   & 9.60 $\pm$0.04 & 0.981 & 2.04e+43 & 0.85  & 0.637 & 0.687 & 2.61e+10 & 3.03e+10 & \textsc{Galfit}   & 0.074$\pm$0.014 & 3.60e+07 & H\,{\sevensize II} & 14.2\\ 
\rowcolor{White}
NGC4194                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.35$\pm$0.05 & 0.981 & 1.62e+42 & 3.47  & 1.103 & 0.687 & 3.60e+09 & 3.03e+10 & \textsc{Galfit}   & 0.074$\pm$0.014 & 3.60e+07 & H\,{\sevensize II} & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4204                & Sersic                   & Sersic         & disk  & 1.2 & 30.0  & 11.07$\pm$0.05 & 1.002 & 4.14e+41 & 2.01  & 0.813 & 0.738 & 6.77e+08 & 6.15e+08 & \textsc{Galfit}   & 0    $\pm$0     & 1.00e+07 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4207                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 16.7  & 10.10$\pm$0.04 & 0.990 & 2.82e+42 & 2.92  & 0.983 & 0.861 & 5.58e+09 & 1.04e+10 & \textsc{Galfit}   & 0.468$\pm$0.040 & 1.68e+07 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{White}
NGC4207                & Sersic + exDisk          & exDisk         & disk  & --- & 12.0  & 9.96 $\pm$0.03 & 0.990 & 3.21e+42 & 2.05  & 0.820 & 0.861 & 5.30e+09 & 1.04e+10 & \textsc{Galfit}   & 0.468$\pm$0.040 & 1.68e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC7286                & Sersic                   & Sersic         & mixed & 5.4 & 10.0  & 10.64$\pm$0.04 & 0.940 & 7.69e+43 & NA    & NA    & 0.941 & ---   & 1.46e+11 & $C\mapsto$~B/T    & 0.169$\pm$0.045 & 1.15e+08 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4234                & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 19.6  & 10.27$\pm$0.04 & 0.989 & 7.69e+42 & 1.39  & 0.714 & 0.746 & 1.10e+10 & 1.17e+10 & \textsc{Galfit}   & 0.013$\pm$0.006 & 3.00e+07 & H\,{\sevensize II} & 4.7 \\ 
\rowcolor{White}
NGC4234                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.98$\pm$0.08 & 0.989 & 1.00e+41 & 3.16  & 1.034 & 0.746 & 2.08e+08 & 1.17e+10 & \textsc{Galfit}   & 0.013$\pm$0.006 & 3.00e+07 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4237                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 30.6  & 9.24 $\pm$0.05 & 0.992 & 6.25e+42 & 2.51  & 0.902 & 0.849 & 1.13e+10 & 2.44e+10 & \textsc{Galfit}   & 0.438$\pm$0.004 & 1.68e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
NGC4237                & Sersic + exDisk          & exDisk         & disk  & --- & 22.0  & 8.97 $\pm$0.04 & 0.992 & 8.01e+42 & 1.94  & 0.801 & 0.849 & 1.29e+10 & 2.44e+10 & \textsc{Galfit}   & 0.438$\pm$0.004 & 1.68e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4244                & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 152.3 & 7.67 $\pm$0.04 & 0.999 & 1.75e+42 & 1.65  & 0.754 & 0.767 & 2.65e+09 & 2.70e+09 & \textsc{Galfit}   & 0.004$\pm$0.001 & 4.30e+06 & H\,{\sevensize II} & 1.8 \\ 
\rowcolor{White}
NGC4244                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.66$\pm$0.04 & 0.999 & 7.03e+39 & 1.65  & 0.754 & 0.767 & 1.07e+07 & 2.70e+09 & \textsc{Galfit}   & 0.004$\pm$0.001 & 4.30e+06 & H\,{\sevensize II} & 1.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4253                & Sersic + psfAgn          & Sersic         & disk  & 1.4 & 10.0  & 10.65$\pm$0.04 & 0.944 & 2.42e+43 & 1.84  & 0.784 & 0.805 & 3.82e+10 & 6.87e+10 & \textsc{Galfit}   & 0.432$\pm$0.004 & 6.49e+07 & SN    & 4.8 \\ 
\rowcolor{LightGray}
NGC4253                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 10.95$\pm$0.04 & 0.944 & 1.84e+43 & 1.85  & 0.786 & 0.805 & 2.91e+10 & 6.87e+10 & \textsc{Galfit}   & 0.432$\pm$0.004 & 6.49e+07 & SN    & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG3-32-005            & Sersic                   & Sersic         & disk  & 1.0 & 4.7   & 11.15$\pm$0.04 & 0.992 & 6.54e+41 & 2.01  & 0.813 & 0.816 & 1.07e+09 & 1.07e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.31e+07 & H\,{\sevensize II} & 2.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4290                & Sersic + psfAgn          & Sersic         & disk  & 1.6 & 25.1  & 9.36 $\pm$0.04 & 0.982 & 2.69e+43 & 2.16  & 0.839 & 0.857 & 4.54e+10 & 5.08e+10 & \textsc{Galfit}   & 0.085$\pm$0.008 & 3.70e+07 & H\,{\sevensize II} & 14.5\\ 
\rowcolor{LightGray}
NGC4290                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.94$\pm$0.04 & 0.982 & 2.50e+42 & 1.77  & 0.773 & 0.857 & 3.89e+09 & 5.08e+10 & \textsc{Galfit}   & 0.085$\pm$0.008 & 3.70e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4294                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 26.4  & 11.75$\pm$0.32 & 0.994 & 6.20e+41 & 2.86  & 0.971 & 0.699 & 1.21e+09 & 5.60e+09 & \textsc{Galfit}   & 0.155$\pm$0.119 & 1.68e+07 & H\,{\sevensize II} & 4.2 \\ 
\rowcolor{White}
NGC4294                & Sersic + exDisk          & exDisk         & disk  & --- & 23.3  & 9.91 $\pm$0.04 & 0.994 & 3.38e+42 & 1.26  & 0.694 & 0.699 & 4.72e+09 & 5.60e+09 & \textsc{Galfit}   & 0.155$\pm$0.119 & 1.68e+07 & H\,{\sevensize II} & 4.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4314                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 21.8  & 8.18 $\pm$0.04 & 0.992 & 1.56e+43 & 2.64  & 0.927 & 0.916 & 2.91e+10 & 5.48e+10 & \textsc{Galfit}   & 0.525$\pm$0.096 & 1.63e+07 & LINER & 3.2 \\ 
\rowcolor{LightGray}
NGC4314                & Sersic + exDisk          & exDisk         & disk  & --- & 36.9  & 8.29 $\pm$0.04 & 0.992 & 1.41e+43 & 2.15  & 0.837 & 0.916 & 2.37e+10 & 5.48e+10 & \textsc{Galfit}   & 0.525$\pm$0.096 & 1.63e+07 & LINER & 3.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4385                & Sersic + psfAgn          & Sersic         & disk  & 3.6 & 23.7  & 9.69 $\pm$0.04 & 0.990 & 1.23e+43 & 1.46  & 0.724 & 0.796 & 1.79e+10 & 2.06e+10 & \textsc{Galfit}   & 0.041$\pm$0.005 & 2.90e+07 & H\,{\sevensize II} & 6.9 \\ 
\rowcolor{White}
NGC4385                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.10$\pm$0.05 & 0.990 & 5.31e+41 & 1.14  & 0.677 & 0.796 & 7.23e+08 & 2.06e+10 & \textsc{Galfit}   & 0.041$\pm$0.005 & 2.90e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4395                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 12.8  & 12.25$\pm$0.18 & 0.999 & 3.08e+40 & 0.83  & 0.635 & 0.750 & 3.94e+07 & 4.35e+08 & \textsc{Galfit}   & 0.107$\pm$0.059 & 4.70e+06 & SN    & 1.8 \\ 
\rowcolor{LightGray}
NGC4395                & Sersic + exDisk          & exDisk         & disk  & --- & 33.4  & 9.94 $\pm$0.04 & 0.999 & 2.58e+41 & 1.75  & 0.770 & 0.750 & 4.00e+08 & 4.35e+08 & \textsc{Galfit}   & 0.107$\pm$0.059 & 4.70e+06 & SN    & 1.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4396                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 7.0   & 13.54$\pm$0.35 & 0.997 & 1.20e+41 & 2.65  & 0.929 & 0.816 & 2.24e+08 & 3.88e+09 & \textsc{Galfit}   & 0.051$\pm$0.086 & 1.68e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{White}
NGC4396                & Sersic + exDisk          & exDisk         & disk  & --- & 23.6  & 10.36$\pm$0.04 & 0.997 & 2.24e+42 & 2.01  & 0.813 & 0.816 & 3.66e+09 & 3.88e+09 & \textsc{Galfit}   & 0.051$\pm$0.086 & 1.68e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4412                & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 22.0  & 9.71 $\pm$0.03 & 0.979 & 1.33e+43 & 1.69  & 0.760 & 0.806 & 2.03e+10 & 2.25e+10 & \textsc{Galfit}   & 0.046$\pm$0.006 & 3.06e+07 & SN    & 9.5 \\ 
\rowcolor{LightGray}
NGC4412                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.99$\pm$0.03 & 0.979 & 6.47e+41 & 3.55  & 1.122 & 0.806 & 1.46e+09 & 2.25e+10 & \textsc{Galfit}   & 0.046$\pm$0.006 & 3.06e+07 & SN    & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4418                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 2.2   & 11.19$\pm$0.04 & 0.987 & 3.07e+42 & 2.99  & 0.998 & 0.890 & 6.16e+09 & 1.48e+10 & \textsc{Galfit}   & 0.371$\pm$0.066 & 2.90e+07 & SN    & 14.2\\ 
\rowcolor{White}
NGC4418                & Sersic + exDisk          & exDisk         & disk  & --- & 11.4  & 10.62$\pm$0.03 & 0.987 & 5.20e+42 & 2.21  & 0.847 & 0.890 & 8.86e+09 & 1.48e+10 & \textsc{Galfit}   & 0.371$\pm$0.066 & 2.90e+07 & SN    & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4420                & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 21.7  & 9.65 $\pm$0.03 & 0.994 & 4.71e+42 & 1.51  & 0.732 & 0.764 & 6.94e+09 & 7.30e+09 & \textsc{Galfit}   & 0.009$\pm$0.005 & 1.76e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{LightGray}
NGC4420                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.74$\pm$0.08 & 0.994 & 4.33e+40 & 3.61  & 1.136 & 0.764 & 9.90e+07 & 7.30e+09 & \textsc{Galfit}   & 0.009$\pm$0.005 & 1.76e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4424                & Sersic                   & Sersic         & mixed & 1.7 & 25.1  & 9.51 $\pm$0.03 & 0.999 & 6.25e+41 & NA    & NA    & 0.587 & ---   & 7.39e+08 & $C\mapsto$~B/T    & 0.078$\pm$0.021 & 6.00e+06 & H\,{\sevensize II} & 3.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4435                & Sersic                   & Sersic         & mixed & 4.2 & 21.4  & 7.56 $\pm$0.04 & 0.988 & 2.89e+43 & NA    & NA    & 1.293 & ---   & 1.50e+11 & $C\mapsto$~B/T    & 0.240$\pm$0.064 & 1.67e+07 & LINER & 2.0 \\ 
\rowcolor{LightGray}
NGC4435                & Sersic                   & Sersic         & mixed & 4.2 & 21.4  & 7.56 $\pm$0.04 & 0.988 & 2.89e+43 & NA    & NA    & 1.293 & ---   & 1.50e+11 & $C\mapsto$~B/T    & 0.240$\pm$0.064 & 1.67e+07 & LINER & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4448                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 18.6  & 8.58 $\pm$0.04 & 0.993 & 1.08e+43 & 2.64  & 0.927 & 0.945 & 2.01e+10 & 4.93e+10 & \textsc{Galfit}   & 0.415$\pm$0.006 & 1.63e+07 & H\,{\sevensize II} & 2.0 \\ 
\rowcolor{White}
NGC4448                & Sersic + exDisk          & exDisk         & disk  & --- & 32.6  & 8.21 $\pm$0.04 & 0.993 & 1.52e+43 & 2.40  & 0.882 & 0.945 & 2.70e+10 & 4.93e+10 & \textsc{Galfit}   & 0.415$\pm$0.006 & 1.63e+07 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4470                & Sersic + psfAgn          & Sersic         & disk  & 0.6 & 14.6  & 10.16$\pm$0.03 & 0.996 & 2.69e+42 & 1.36  & 0.709 & 0.719 & 3.84e+09 & 3.92e+09 & \textsc{Galfit}   & 0.011$\pm$0.006 & 1.68e+07 & H\,{\sevensize II} & 4.6 \\ 
\rowcolor{LightGray}
NGC4470                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.01$\pm$0.09 & 0.996 & 3.09e+40 & 1.05  & 0.665 & 0.719 & 4.13e+07 & 3.92e+09 & \textsc{Galfit}   & 0.011$\pm$0.006 & 1.68e+07 & H\,{\sevensize II} & 4.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS12274+0018         & Sersic + psfAgn          & Sersic         & disk  & 9.1 & 3.4   & 12.36$\pm$0.14 & 0.960 & 1.76e+42 & 2.51  & 0.902 & 0.894 & 3.19e+09 & 3.59e+09 & \textsc{Galfit}   & 0.119$\pm$0.032 & 3.81e+07 & H\,{\sevensize II} & 3.0 \\ 
\rowcolor{White}
IRAS12274+0018         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.53$\pm$0.13 & 0.960 & 2.38e+41 & 4.34  & 1.324 & 0.894 & 6.34e+08 & 3.59e+09 & \textsc{Galfit}   & 0.119$\pm$0.032 & 3.81e+07 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4491                & Sersic + psfAgn          & Sersic         & disk  & 1.4 & 23.9  & 9.84 $\pm$0.03 & 0.995 & 3.61e+42 & 2.05  & 0.820 & 0.833 & 5.96e+09 & 6.16e+09 & \textsc{Galfit}   & 0.017$\pm$0.007 & 1.68e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{LightGray}
NGC4491                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.26$\pm$0.05 & 0.995 & 6.15e+40 & 0.16  & 0.552 & 0.833 & 6.83e+07 & 6.16e+09 & \textsc{Galfit}   & 0.017$\pm$0.007 & 1.68e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4500                & Sersic + psfAgn          & Sersic         & disk  & 5.1 & 10.3  & 9.66 $\pm$0.04 & 0.978 & 4.01e+43 & 1.28  & 0.697 & 0.783 & 5.62e+10 & 6.62e+10 & \textsc{Galfit}   & 0.047$\pm$0.010 & 5.20e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{White}
NGC4500                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.93$\pm$0.05 & 0.978 & 1.97e+42 & 3.19  & 1.041 & 0.783 & 4.13e+09 & 6.62e+10 & \textsc{Galfit}   & 0.047$\pm$0.010 & 5.20e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4495                & Sersic + psfAgn          & Sersic         & disk  & 2.6 & 9.0   & 10.25$\pm$0.04 & 0.949 & 4.60e+43 & 2.46  & 0.893 & 0.852 & 8.27e+10 & 8.25e+10 & \textsc{Galfit}   & 0.047$\pm$0.014 & 7.42e+07 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{LightGray}
NGC4495                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.52$\pm$0.08 & 0.949 & 2.26e+42 & 2.46  & 0.893 & 0.852 & 4.06e+09 & 8.25e+10 & \textsc{Galfit}   & 0.047$\pm$0.014 & 7.42e+07 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC3476                 & Sersic                   & Sersic         & disk  & 1.2 & 23.6  & 10.60$\pm$0.04 & 0.995 & 1.79e+42 & 2.01  & 0.813 & 0.719 & 2.93e+09 & 2.59e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.68e+07 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4509                & Sersic                   & Sersic         & disk  & 0.7 & 9.5   & 12.24$\pm$0.04 & 0.997 & 1.73e+41 & 2.01  & 0.813 & 0.625 & 2.83e+08 & 2.17e+08 & \textsc{Galfit}   & 0    $\pm$0     & 1.11e+07 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4519                & Sersic + psfAgn          & Sersic         & disk  & 3.4 & 82.0  & 8.76 $\pm$0.05 & 0.992 & 9.72e+42 & 0.96  & 0.652 & 0.793 & 1.28e+10 & 1.55e+10 & \textsc{Galfit}   & 0    $\pm$0     & 1.68e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{White}
NGC4519                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 17.09$\pm$0.83 & 0.992 & 4.52e+39 & -0.39 & 0.491 & 0.793 & 4.47e+06 & 1.55e+10 & \textsc{Galfit}   & 0    $\pm$0     & 1.68e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4548                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 22.5  & 8.01 $\pm$0.04 & 0.994 & 1.81e+43 & 3.07  & 1.015 & 0.816 & 3.70e+10 & 9.73e+10 & \textsc{Galfit}   & 0.306$\pm$0.072 & 1.62e+07 & SN    & 13.2\\ 
\rowcolor{LightGray}
NGC4548                & Sersic + exDisk          & exDisk         & disk  & --- & 81.2  & 7.12 $\pm$0.04 & 0.994 & 4.10e+43 & 2.04  & 0.818 & 0.816 & 6.75e+10 & 9.73e+10 & \textsc{Galfit}   & 0.306$\pm$0.072 & 1.62e+07 & SN    & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS12337+5044         & Sersic + psfAgn          & Sersic         & disk  & 0.3 & 6.6   & 12.26$\pm$0.04 & 0.892 & 3.67e+43 & 1.90  & 0.794 & 0.734 & 5.86e+10 & 6.45e+10 & \textsc{Galfit}   & 0.157$\pm$0.042 & 1.72e+08 & H\,{\sevensize II} & 4.5 \\ 
\rowcolor{White}
IRAS12337+5044         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.08$\pm$0.06 & 0.892 & 6.86e+42 & 1.90  & 0.794 & 0.734 & 1.10e+10 & 6.45e+10 & \textsc{Galfit}   & 0.157$\pm$0.042 & 1.72e+08 & H\,{\sevensize II} & 4.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC3581                 & Sersic + exDisk          & Sersic         & bulge & 4.0 & 5.4   & 11.24$\pm$0.04 & 0.938 & 3.73e+43 & 2.99  & 0.998 & 0.842 & 7.49e+10 & 1.05e+11 & \textsc{Galfit}   & 0.600$\pm$0.035 & 1.06e+08 & H\,{\sevensize II} & 6.0 \\ 
\rowcolor{LightGray}
IC3581                 & Sersic + exDisk          & exDisk         & disk  & --- & 3.9   & 11.68$\pm$0.04 & 0.938 & 2.49e+43 & 1.86  & 0.788 & 0.842 & 3.95e+10 & 1.05e+11 & \textsc{Galfit}   & 0.600$\pm$0.035 & 1.06e+08 & H\,{\sevensize II} & 6.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4592                & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 53.4  & 9.49 $\pm$0.04 & 0.997 & 2.18e+42 & 2.65  & 0.929 & 0.727 & 4.07e+09 & 3.18e+09 & \textsc{Galfit}   & 1.000$\pm$0.265 & 1.11e+07 & H\,{\sevensize II} & 4.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4607                & Sersic + psfAgn          & Sersic         & disk  & 1.2 & 32.0  & 9.52 $\pm$0.03 & 0.987 & 4.80e+42 & 2.33  & 0.869 & 1.054 & 8.39e+09 & 1.03e+10 & \textsc{Galfit}   & 0.006$\pm$0.003 & 1.68e+07 & LINER & 13.2\\ 
\rowcolor{LightGray}
NGC4607                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.07$\pm$0.10 & 0.987 & 2.89e+40 & 2.18  & 0.842 & 1.054 & 4.90e+07 & 1.03e+10 & \textsc{Galfit}   & 0.006$\pm$0.003 & 1.68e+07 & LINER & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4625                & Sersic + psfAgn          & Sersic         & disk  & 1.4 & 23.2  & 9.70 $\pm$0.04 & 0.996 & 1.23e+42 & 1.61  & 0.747 & 0.760 & 1.85e+09 & 1.90e+09 & \textsc{Galfit}   & 0.013$\pm$0.003 & 9.20e+06 & H\,{\sevensize II} & 1.8 \\ 
\rowcolor{White}
NGC4625                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.39$\pm$0.05 & 0.996 & 1.64e+40 & 3.36  & 1.078 & 0.760 & 3.56e+07 & 1.90e+09 & \textsc{Galfit}   & 0.013$\pm$0.003 & 9.20e+06 & H\,{\sevensize II} & 1.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4630                & Sersic                   & Sersic         & mixed & 2.0 & 36.2  & 9.19 $\pm$0.04 & 0.994 & 5.65e+42 & NA    & NA    & 0.695 & ---   & 7.90e+09 & $C\mapsto$~B/T    & 0.103$\pm$0.027 & 1.56e+07 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC3690                 & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 6.9   & 11.46$\pm$0.04 & 0.988 & 4.90e+41 & 2.44  & 0.889 & 0.875 & 8.76e+08 & 9.99e+08 & \textsc{Galfit}   & 0.137$\pm$0.034 & 1.31e+07 & H\,{\sevensize II} & 3.0 \\ 
\rowcolor{White}
IC3690                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.46$\pm$0.05 & 0.988 & 7.76e+40 & 2.44  & 0.889 & 0.875 & 1.39e+08 & 9.99e+08 & \textsc{Galfit}   & 0.137$\pm$0.034 & 1.31e+07 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC7905\_NED01         & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.4   & 12.93$\pm$0.12 & 0.963 & 4.45e+42 & 0.18  & 0.554 & 0.679 & 4.96e+09 & 1.87e+10 & \textsc{Galfit}   & 0.326$\pm$0.138 & 7.87e+07 & H\,{\sevensize II} & 4.3 \\ 
\rowcolor{LightGray}
UGC7905\_NED01         & Sersic + exDisk          & exDisk         & disk  & --- & 2.5   & 12.14$\pm$0.05 & 0.963 & 9.21e+42 & 1.38  & 0.712 & 0.679 & 1.32e+10 & 1.87e+10 & \textsc{Galfit}   & 0.326$\pm$0.138 & 7.87e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG5-30-069            & Sersic + psfAgn          & Sersic         & disk  & 3.5 & 8.3   & 10.84$\pm$0.04 & 0.964 & 2.70e+43 & 2.70  & 0.939 & 0.899 & 5.10e+10 & 5.02e+10 & \textsc{Galfit}   & 0.023$\pm$0.011 & 7.40e+07 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{White}
MCG5-30-069            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.89$\pm$0.10 & 0.964 & 6.47e+41 & 5.17  & 1.576 & 0.899 & 2.05e+09 & 5.02e+10 & \textsc{Galfit}   & 0.023$\pm$0.011 & 7.40e+07 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC3721                 & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.4   & 10.88$\pm$0.04 & 0.945 & 4.52e+43 & 3.46  & 1.101 & 0.869 & 1.00e+11 & 1.40e+11 & \textsc{Galfit}   & 0.566$\pm$0.113 & 9.85e+07 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{LightGray}
IC3721                 & Sersic + exDisk          & exDisk         & disk  & --- & 7.9   & 11.17$\pm$0.04 & 0.945 & 3.46e+43 & 1.91  & 0.796 & 0.869 & 5.54e+10 & 1.40e+11 & \textsc{Galfit}   & 0.566$\pm$0.113 & 9.85e+07 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4670                & Sersic + psfAgn          & Sersic         & disk  & 2.5 & 15.6  & 10.27$\pm$0.04 & 0.994 & 1.76e+42 & 0.63  & 0.609 & 0.647 & 2.16e+09 & 2.37e+09 & \textsc{Galfit}   & 0.040$\pm$0.009 & 1.43e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{White}
NGC4670                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.72$\pm$0.06 & 0.994 & 7.32e+40 & -0.36 & 0.495 & 0.647 & 7.29e+07 & 2.37e+09 & \textsc{Galfit}   & 0.040$\pm$0.009 & 1.43e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4675                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.8   & 11.92$\pm$0.04 & 0.955 & 1.07e+43 & 3.79  & 1.180 & 0.952 & 2.54e+10 & 7.03e+10 & \textsc{Galfit}   & 0.291$\pm$0.040 & 7.69e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
NGC4675                & Sersic + exDisk          & exDisk         & disk  & --- & 9.3   & 10.95$\pm$0.04 & 0.955 & 2.61e+43 & 2.31  & 0.865 & 0.952 & 4.54e+10 & 7.03e+10 & \textsc{Galfit}   & 0.291$\pm$0.040 & 7.69e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG7-26-051            & Sersic + exDisk          & Sersic         & bulge & 4.0 & 4.3   & 11.96$\pm$0.05 & 0.842 & 3.31e+43 & 2.65  & 0.929 & 0.983 & 6.19e+10 & 1.71e+11 & \textsc{Galfit}   & 0.383$\pm$0.053 & 1.47e+08 & H\,{\sevensize II} & 4.7 \\ 
\rowcolor{White}
MCG7-26-051            & Sersic + exDisk          & exDisk         & disk  & --- & 3.1   & 11.44$\pm$0.04 & 0.842 & 5.34e+43 & 2.01  & 0.813 & 0.983 & 8.74e+10 & 1.71e+11 & \textsc{Galfit}   & 0.383$\pm$0.053 & 1.47e+08 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4689                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 83.0  & 8.25 $\pm$0.05 & 0.995 & 1.56e+43 & 1.98  & 0.808 & 0.864 & 2.54e+10 & 5.56e+10 & \textsc{Galfit}   & 0.489$\pm$0.007 & 1.68e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
NGC4689                & Sersic + exDisk          & exDisk         & disk  & --- & 79.4  & 8.20 $\pm$0.04 & 0.995 & 1.63e+43 & 1.95  & 0.803 & 0.864 & 2.63e+10 & 5.56e+10 & \textsc{Galfit}   & 0.489$\pm$0.007 & 1.68e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4688                & Sersic                   & Sersic         & disk  & 1.0 & 20.4  & 11.01$\pm$0.04 & 0.988 & 1.05e+42 & 2.01  & 0.813 & 0.787 & 1.72e+09 & 1.66e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.56e+07 & H\,{\sevensize II} & 2.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4704                & Sersic                   & Sersic         & mixed & 4.2 & 24.1  & 10.16$\pm$0.05 & 0.924 & 1.33e+44 & NA    & NA    & 0.917 & ---   & 2.46e+11 & $C\mapsto$~B/T    & 0.105$\pm$0.028 & 1.23e+08 & LINER & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4701                & Sersic + psfAgn          & Sersic         & disk  & 1.6 & 18.1  & 9.65 $\pm$0.03 & 0.993 & 3.69e+42 & 1.52  & 0.733 & 0.764 & 5.44e+09 & 5.78e+09 & \textsc{Galfit}   & 0.019$\pm$0.007 & 1.56e+07 & H\,{\sevensize II} & 2.0 \\ 
\rowcolor{White}
NGC4701                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.93$\pm$0.06 & 0.993 & 7.17e+40 & 1.71  & 0.763 & 0.764 & 1.10e+08 & 5.78e+09 & \textsc{Galfit}   & 0.019$\pm$0.007 & 1.56e+07 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS12468+3436         & Sersic$^{n=1}$           & Sersic$^{n=1}$ & disk  & 1.0 & 1.1   & 14.03$\pm$0.06 & 0.680 & 4.57e+43 & 2.01  & 0.813 & 0.926 & 7.48e+10 & 8.52e+10 & \textsc{Galfit}   & 0    $\pm$0     & 4.98e+08 & SN    & 3.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS12470+1404         & Sersic                   & Sersic         & mixed & 2.0 & 2.2   & 13.34$\pm$0.06 & 0.993 & 8.71e+40 & NA    & NA    & 0.685 & ---   & 1.20e+08 & $C\mapsto$~B/T    & 0.121$\pm$0.032 & 1.31e+07 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG8-23-097            & Sersic                   & Sersic         & mixed & 4.1 & 4.6   & 10.96$\pm$0.04 & 0.902 & 7.10e+43 & NA    & NA    & 1.093 & ---   & 1.56e+11 & $C\mapsto$~B/T    & 0.151$\pm$0.040 & 1.31e+08 & LINER & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4747                & Sersic                   & Sersic         & disk  & 0.5 & 23.9  & 10.71$\pm$0.04 & 0.999 & 1.18e+42 & 2.01  & 0.813 & 0.876 & 1.93e+09 & 2.07e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.43e+07 & H\,{\sevensize II} & 4.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8017                & Sersic + psfAgn + exDisk & Sersic         & bulge & 4.0 & 10.0  & 12.27$\pm$0.09 & 0.928 & 1.46e+43 & 2.50  & 0.901 & 0.881 & 2.65e+10 & 1.67e+11 & \textsc{Galfit}   & 0.155$\pm$0.040 & 1.07e+08 & TO    & 5.0 \\ 
\rowcolor{LightGray}
UGC8017                & Sersic + psfAgn + exDisk & psfAgn         & AGN   & --- & ---   & 14.19$\pm$0.07 & 0.928 & 2.49e+42 & NA    & NA    & 0.881 & ---   & 1.67e+11 & \textsc{Galfit}   & 0.155$\pm$0.040 & 1.07e+08 & TO    & 5.0 \\ 
\rowcolor{LightGray}
UGC8017                & Sersic + psfAgn + exDisk & exDisk         & disk  & --- & 7.2   & 10.43$\pm$0.04 & 0.928 & 7.94e+43 & 2.27  & 0.858 & 0.881 & 1.37e+11 & 1.67e+11 & \textsc{Galfit}   & 0.155$\pm$0.040 & 1.07e+08 & TO    & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4765                & Sersic                   & Sersic         & disk  & 1.3 & 10.1  & 10.72$\pm$0.03 & 0.995 & 1.38e+42 & 2.01  & 0.813 & 0.702 & 2.26e+09 & 1.95e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.56e+07 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8041                & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 18.4  & 11.08$\pm$0.05 & 1.004 & 2.18e+42 & 2.65  & 0.929 & 0.854 & 4.07e+09 & 3.74e+09 & \textsc{Galfit}   & 1.000$\pm$0.265 & 2.30e+07 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UM530                  & Sersic                   & Sersic         & mixed & 2.1 & 1.5   & 13.30$\pm$0.05 & 0.742 & 3.14e+43 & NA    & NA    & 0.634 & ---   & 4.01e+10 & $C\mapsto$~B/T    & 0.163$\pm$0.043 & 2.83e+08 & H\,{\sevensize II} & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC4861                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.3   & 13.58$\pm$0.36 & 0.994 & 1.39e+41 & 0.20  & 0.556 & 0.567 & 1.56e+08 & 3.57e+08 & \textsc{Galfit}   & 0.444$\pm$0.304 & 1.85e+07 & H\,{\sevensize II} & 5.3 \\ 
\rowcolor{LightGray}
NGC4861                & Sersic + exDisk          & exDisk         & disk  & --- & 2.7   & 13.34$\pm$0.24 & 0.994 & 1.74e+41 & 0.28  & 0.566 & 0.567 & 1.98e+08 & 3.57e+08 & \textsc{Galfit}   & 0.444$\pm$0.304 & 1.85e+07 & H\,{\sevensize II} & 5.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC4868                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.8   & 12.50$\pm$0.05 & 0.969 & 5.88e+42 & 2.04  & 0.818 & 0.885 & 9.68e+09 & 1.71e+11 & \textsc{Galfit}   & 0.061$\pm$0.050 & 7.40e+07 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
NGC4868                & Sersic + exDisk          & exDisk         & disk  & --- & 9.4   & 9.54 $\pm$0.04 & 0.969 & 8.98e+43 & 1.71  & 0.763 & 0.885 & 1.38e+11 & 1.71e+11 & \textsc{Galfit}   & 0.061$\pm$0.050 & 7.40e+07 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8179                & Sersic                   & Sersic         & mixed & 3.6 & 8.9   & 10.73$\pm$0.04 & 0.877 & 2.45e+44 & NA    & NA    & 0.937 & ---   & 4.61e+11 & $C\mapsto$~B/T    & 0.193$\pm$0.051 & 2.22e+08 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5001                & Sersic + psfAgn          & Sersic         & disk  & 5.0 & 32.1  & 9.59 $\pm$0.06 & 0.927 & 2.72e+44 & 2.52  & 0.904 & 0.857 & 4.95e+11 & 4.82e+11 & \textsc{Galfit}   & 0.026$\pm$0.008 & 1.35e+08 & H\,{\sevensize II} & 2.7 \\ 
\rowcolor{White}
NGC5001                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.53$\pm$0.06 & 0.927 & 7.22e+42 & 6.01  & 1.879 & 0.857 & 2.73e+10 & 4.82e+11 & \textsc{Galfit}   & 0.026$\pm$0.008 & 1.35e+08 & H\,{\sevensize II} & 2.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC856                  & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 10.3  & 11.10$\pm$0.04 & 0.957 & 1.59e+43 & 1.80  & 0.778 & 0.753 & 2.49e+10 & 2.46e+10 & \textsc{Galfit}   & 0.019$\pm$0.010 & 6.43e+07 & H\,{\sevensize II} & 4.7 \\ 
\rowcolor{LightGray}
IC856                  & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.38$\pm$0.13 & 0.957 & 3.09e+41 & -0.40 & 0.490 & 0.753 & 3.05e+08 & 2.46e+10 & \textsc{Galfit}   & 0.019$\pm$0.010 & 6.43e+07 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC8269                & Sersic + psfAgn          & Sersic         & mixed & 7.6 & 20.7  & 10.75$\pm$0.06 & 0.936 & 8.00e+43 & NA    & NA    & 0.888 & ---   & 1.44e+11 & $C\mapsto$~B/T    & 0.166$\pm$0.044 & 1.24e+08 & TO    & 8.4 \\ 
\rowcolor{White}
UGC8269                & Sersic + psfAgn          & psfAgn         & AGN   & --- & ---   & 15.22$\pm$0.17 & 0.936 & 1.30e+42 & NA    & NA    & 0.888 & ---   & 1.44e+11 & $C\mapsto$~B/T    & 0.166$\pm$0.044 & 1.24e+08 & TO    & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5014                & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 12.9  & 10.10$\pm$0.04 & 0.993 & 3.44e+42 & 1.61  & 0.747 & 0.911 & 5.17e+09 & 6.36e+09 & \textsc{Galfit}   & 0.011$\pm$0.007 & 1.85e+07 & H\,{\sevensize II} & 4.2 \\ 
\rowcolor{LightGray}
NGC5014                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.01$\pm$0.11 & 0.993 & 3.73e+40 & -2.05 & 0.347 & 0.911 & 2.60e+07 & 6.36e+09 & \textsc{Galfit}   & 0.011$\pm$0.007 & 1.85e+07 & H\,{\sevensize II} & 4.2 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5012                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.9   & 11.13$\pm$0.04 & 0.980 & 6.19e+42 & 3.60  & 1.134 & 0.879 & 1.41e+10 & 9.28e+10 & \textsc{Galfit}   & 0.118$\pm$0.020 & 4.02e+07 & LINER & 22.2\\ 
\rowcolor{White}
NGC5012                & Sersic + exDisk          & exDisk         & disk  & --- & 17.1  & 8.95 $\pm$0.04 & 0.980 & 4.61e+43 & 1.98  & 0.808 & 0.879 & 7.49e+10 & 9.28e+10 & \textsc{Galfit}   & 0.118$\pm$0.020 & 4.02e+07 & LINER & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS13116+4508         & Sersic + psfAgn          & Sersic         & disk  & 2.6 & 2.5   & 12.77$\pm$0.04 & 0.797 & 4.60e+43 & 2.33  & 0.869 & 0.876 & 8.04e+10 & 9.39e+10 & \textsc{Galfit}   & 0.139$\pm$0.037 & 2.58e+08 & H\,{\sevensize II} & 4.5 \\ 
\rowcolor{LightGray}
IRAS13116+4508         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.75$\pm$0.16 & 0.797 & 7.42e+42 & 3.39  & 1.085 & 0.876 & 1.62e+10 & 9.39e+10 & \textsc{Galfit}   & 0.139$\pm$0.037 & 2.58e+08 & H\,{\sevensize II} & 4.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC860                  & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 8.8   & 10.61$\pm$0.04 & 0.974 & 1.83e+43 & 2.23  & 0.851 & 0.863 & 3.13e+10 & 3.42e+10 & \textsc{Galfit}   & 0.069$\pm$0.016 & 5.45e+07 & LINER & 14.2\\ 
\rowcolor{White}
IC860                  & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.44$\pm$0.06 & 0.974 & 1.35e+42 & 2.23  & 0.851 & 0.863 & 2.31e+09 & 3.42e+10 & \textsc{Galfit}   & 0.069$\pm$0.016 & 5.45e+07 & LINER & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5060                & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 16.5  & 10.25$\pm$0.04 & 0.936 & 7.81e+43 & 2.13  & 0.833 & 0.894 & 1.31e+11 & 1.54e+11 & \textsc{Galfit}   & 0.084$\pm$0.014 & 9.74e+07 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{LightGray}
NGC5060                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.84$\pm$0.04 & 0.936 & 7.19e+42 & 2.05  & 0.820 & 0.894 & 1.19e+10 & 1.54e+11 & \textsc{Galfit}   & 0.084$\pm$0.014 & 9.74e+07 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC8357\_NED01         & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 7.9   & 11.23$\pm$0.03 & 0.935 & 7.20e+43 & 2.01  & 0.813 & 0.789 & 1.18e+11 & 1.14e+11 & \textsc{Galfit}   & 0    $\pm$0     & 1.47e+08 & TO    & 7.4 \\ 
\rowcolor{White}
UGC8357\_NED01         & Sersic + psfAgn          & psfAgn         & AGN   & --- & ---   & 13.15$\pm$0.04 & 0.935 & 1.23e+43 & NA    & NA    & 0.789 & ---   & 1.14e+11 & \textsc{Galfit}   & 0    $\pm$0     & 1.47e+08 & TO    & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8361                & Sersic + psfAgn          & Sersic         & disk  & 3.6 & 5.9   & 10.79$\pm$0.04 & 0.924 & 5.59e+43 & 2.48  & 0.897 & 0.876 & 1.01e+11 & 1.06e+11 & \textsc{Galfit}   & 0.067$\pm$0.041 & 1.06e+08 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{LightGray}
UGC8361                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.65$\pm$0.10 & 0.924 & 4.01e+42 & 2.48  & 0.897 & 0.876 & 7.24e+09 & 1.06e+11 & \textsc{Galfit}   & 0.067$\pm$0.041 & 1.06e+08 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC883                  & Sersic                   & Sersic         & mixed & 5.2 & 6.2   & 10.68$\pm$0.04 & 0.942 & 6.12e+43 & NA    & NA    & 0.802 & ---   & 9.87e+10 & $C\mapsto$~B/T    & 0.136$\pm$0.036 & 1.05e+08 & SN    & 15.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5100\_NED02         & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 5.8   & 10.50$\pm$0.03 & 0.913 & 1.29e+44 & 2.32  & 0.867 & 0.858 & 2.25e+11 & 2.31e+11 & \textsc{Galfit}   & 0.035$\pm$0.022 & 1.42e+08 & SN    & 2.7 \\ 
\rowcolor{LightGray}
NGC5100\_NED02         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.11$\pm$0.14 & 0.913 & 4.64e+42 & 4.53  & 1.378 & 0.858 & 1.29e+10 & 2.31e+11 & \textsc{Galfit}   & 0.035$\pm$0.022 & 1.42e+08 & SN    & 2.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5104                & Sersic                   & Sersic         & mixed & 3.6 & 7.8   & 9.83 $\pm$0.03 & 0.943 & 9.42e+43 & NA    & NA    & 0.930 & ---   & 1.76e+11 & $C\mapsto$~B/T    & 0.190$\pm$0.050 & 8.78e+07 & SN    & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5107                & Sersic                   & Sersic         & disk  & 1.1 & 26.0  & 11.18$\pm$0.04 & 0.997 & 1.28e+42 & 2.01  & 0.813 & 0.691 & 2.09e+09 & 1.77e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.85e+07 & H\,{\sevensize II} & 2.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5112                & Sersic                   & Sersic         & disk  & 1.5 & 41.5  & 9.71 $\pm$0.04 & 0.994 & 4.92e+42 & 2.01  & 0.813 & 0.771 & 8.05e+09 & 7.63e+09 & \textsc{Galfit}   & 0    $\pm$0     & 1.85e+07 & TO    & 4.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5123                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 12.8  & 10.43$\pm$0.09 & 0.938 & 1.07e+44 & 2.62  & 0.923 & 0.856 & 1.99e+11 & 3.37e+11 & \textsc{Galfit}   & 0.545$\pm$0.013 & 1.23e+08 & H\,{\sevensize II} & 4.8 \\ 
\rowcolor{LightGray}
NGC5123                & Sersic + exDisk          & exDisk         & disk  & --- & 11.5  & 10.62$\pm$0.07 & 0.938 & 8.94e+43 & 1.56  & 0.740 & 0.856 & 1.33e+11 & 3.37e+11 & \textsc{Galfit}   & 0.545$\pm$0.013 & 1.23e+08 & H\,{\sevensize II} & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS13232+1731         & Sersic + exDisk          & Sersic         & bulge & 4.0 & 5.2   & 12.05$\pm$0.08 & 0.858 & 1.58e+44 & 2.01  & 0.813 & 0.743 & 2.58e+11 & 3.33e+11 & \textsc{Galfit}   & 0.713$\pm$0.189 & 3.32e+08 & H\,{\sevensize II} & 1.0 \\ 
\rowcolor{White}
IRAS13232+1731         & Sersic + exDisk          & exDisk         & disk  & --- & 3.7   & 13.04$\pm$0.11 & 0.858 & 6.37e+43 & 1.21  & 0.687 & 0.743 & 8.81e+10 & 3.33e+11 & \textsc{Galfit}   & 0.713$\pm$0.189 & 3.32e+08 & H\,{\sevensize II} & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5147                & Sersic + psfAgn          & Sersic         & disk  & 0.4 & 42.9  & 9.58 $\pm$0.03 & 0.994 & 5.25e+42 & 2.01  & 0.813 & 0.827 & 8.59e+09 & 9.76e+09 & \textsc{Galfit}   & 0.104$\pm$0.025 & 1.80e+07 & H\,{\sevensize II} & 4.6 \\ 
\rowcolor{LightGray}
NGC5147                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.92$\pm$0.03 & 0.994 & 6.09e+41 & 2.65  & 0.929 & 0.827 & 1.14e+09 & 9.76e+09 & \textsc{Galfit}   & 0.104$\pm$0.025 & 1.80e+07 & H\,{\sevensize II} & 4.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5204                & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 33.7  & 9.76 $\pm$0.04 & 0.999 & 1.41e+41 & 1.50  & 0.730 & 0.706 & 2.07e+08 & 2.01e+08 & \textsc{Galfit}   & 0.001$\pm$0.007 & 3.20e+06 & H\,{\sevensize II} & 1.7 \\ 
\rowcolor{White}
NGC5204                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 16.87$\pm$0.27 & 0.999 & 2.03e+38 & 1.50  & 0.730 & 0.706 & 2.98e+05 & 2.01e+08 & \textsc{Galfit}   & 0.001$\pm$0.007 & 3.20e+06 & H\,{\sevensize II} & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8561                & Sersic + psfAgn          & Sersic         & disk  & 1.9 & 11.4  & 10.50$\pm$0.04 & 0.970 & 7.83e+43 & 2.00  & 0.811 & 0.828 & 1.28e+11 & 1.37e+11 & \textsc{Galfit}   & 0.041$\pm$0.012 & 1.08e+08 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{LightGray}
UGC8561                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.91$\pm$0.06 & 0.970 & 3.39e+42 & 1.88  & 0.791 & 0.828 & 5.40e+09 & 1.37e+11 & \textsc{Galfit}   & 0.041$\pm$0.012 & 1.08e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5230                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.0   & 12.53$\pm$0.06 & 0.982 & 1.18e+43 & 2.12  & 0.832 & 0.834 & 1.98e+10 & 1.37e+11 & \textsc{Galfit}   & 0.145$\pm$0.049 & 1.06e+08 & H\,{\sevensize II} & 4.8 \\ 
\rowcolor{White}
NGC5230                & Sersic + exDisk          & exDisk         & disk  & --- & 9.5   & 10.60$\pm$0.04 & 0.982 & 6.98e+43 & 2.05  & 0.820 & 0.834 & 1.15e+11 & 1.37e+11 & \textsc{Galfit}   & 0.145$\pm$0.049 & 1.06e+08 & H\,{\sevensize II} & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS13349+2438         & Sersic$^{n=1}$           & Sersic$^{n=1}$ & disk  & 1.0 & 0.5   & 10.47$\pm$0.10 & 0.352 & 5.20e+44 & 2.01  & 0.813 & 0.716 & 8.51e+11 & 7.49e+11 & \textsc{Galfit}   & 0    $\pm$0     & 4.54e+08 & SN    & 1.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC8626                & Sersic                   & Sersic         & mixed & 9.1 & 14.2  & 10.68$\pm$0.07 & 0.935 & 6.55e+43 & NA    & NA    & 0.881 & ---   & 1.16e+11 & $C\mapsto$~B/T    & 0.186$\pm$0.049 & 1.09e+08 & H\,{\sevensize II} & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5263                & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 17.2  & 10.21$\pm$0.04 & 0.956 & 5.24e+43 & 2.15  & 0.837 & 0.841 & 8.82e+10 & 9.55e+10 & \textsc{Galfit}   & 0.069$\pm$0.007 & 7.75e+07 & H\,{\sevensize II} & 13.2\\ 
\rowcolor{LightGray}
NGC5263                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.03$\pm$0.04 & 0.956 & 3.90e+42 & 2.65  & 0.929 & 0.841 & 7.29e+09 & 9.55e+10 & \textsc{Galfit}   & 0.069$\pm$0.007 & 7.75e+07 & H\,{\sevensize II} & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG1-35-028            & Sersic + psfAgn          & Sersic         & disk  & 1.3 & 8.2   & 11.05$\pm$0.04 & 0.936 & 4.36e+43 & 2.30  & 0.864 & 0.864 & 7.58e+10 & 9.71e+10 & \textsc{Galfit}   & 0.221$\pm$0.024 & 1.05e+08 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{White}
MCG1-35-028            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.41$\pm$0.04 & 0.936 & 1.24e+43 & 2.02  & 0.814 & 0.864 & 2.03e+10 & 9.71e+10 & \textsc{Galfit}   & 0.221$\pm$0.024 & 1.05e+08 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC910                  & Sersic                   & Sersic         & mixed & 6.0 & 6.3   & 10.91$\pm$0.05 & 0.944 & 6.55e+43 & NA    & NA    & 0.820 & ---   & 1.08e+11 & $C\mapsto$~B/T    & 0.149$\pm$0.039 & 1.20e+08 & SN    & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MK268                  & Sersic                   & Sersic         & mixed & 7.9 & 9.2   & 10.50$\pm$0.05 & 0.950 & 2.00e+44 & NA    & NA    & 0.868 & ---   & 3.50e+11 & $C\mapsto$~B/T    & 0.215$\pm$0.057 & 1.74e+08 & SN    & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5278                & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 10.5  & 10.35$\pm$0.04 & 0.951 & 9.99e+43 & 1.95  & 0.803 & 0.898 & 1.61e+11 & 2.00e+11 & \textsc{Galfit}   & 0.097$\pm$0.015 & 1.14e+08 & LINER & 4.8 \\ 
\rowcolor{LightGray}
NGC5278                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.78$\pm$0.04 & 0.951 & 1.07e+43 & 3.36  & 1.078 & 0.898 & 2.32e+10 & 2.00e+11 & \textsc{Galfit}   & 0.097$\pm$0.015 & 1.14e+08 & LINER & 4.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5273                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.0   & 10.52$\pm$0.04 & 0.995 & 1.86e+42 & 1.96  & 0.804 & 0.887 & 3.01e+09 & 1.77e+10 & \textsc{Galfit}   & 0.188$\pm$0.014 & 1.65e+07 & SN    & 2.0 \\ 
\rowcolor{White}
NGC5273                & Sersic + exDisk          & exDisk         & disk  & --- & 19.7  & 8.93 $\pm$0.04 & 0.995 & 8.04e+42 & 2.47  & 0.895 & 0.887 & 1.45e+10 & 1.77e+10 & \textsc{Galfit}   & 0.188$\pm$0.014 & 1.65e+07 & SN    & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8685                & Sersic + psfAgn          & Sersic         & disk  & 2.4 & 15.4  & 10.68$\pm$0.04 & 0.926 & 1.28e+44 & 2.15  & 0.837 & 0.866 & 2.16e+11 & 2.46e+11 & \textsc{Galfit}   & 0.096$\pm$0.015 & 1.53e+08 & H\,{\sevensize II} & 4.7 \\ 
\rowcolor{LightGray}
UGC8685                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.11$\pm$0.05 & 0.926 & 1.36e+43 & 2.25  & 0.855 & 0.866 & 2.34e+10 & 2.46e+11 & \textsc{Galfit}   & 0.096$\pm$0.015 & 1.53e+08 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC8686                & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 13.3  & 10.93$\pm$0.03 & 0.946 & 4.94e+43 & 2.19  & 0.844 & 0.826 & 8.39e+10 & 8.92e+10 & \textsc{Galfit}   & 0.083$\pm$0.012 & 1.05e+08 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
UGC8686                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.54$\pm$0.04 & 0.946 & 4.47e+42 & 2.37  & 0.876 & 0.826 & 7.88e+09 & 8.92e+10 & \textsc{Galfit}   & 0.083$\pm$0.012 & 1.05e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8696                & Sersic + psfAgn          & Sersic         & disk  & 4.7 & 5.2   & 10.79$\pm$0.06 & 0.872 & 1.24e+44 & 0.81  & 0.632 & 0.860 & 1.58e+11 & 2.35e+11 & \textsc{Galfit}   & 0.089$\pm$0.049 & 1.63e+08 & SN    & 15.5\\ 
\rowcolor{LightGray}
UGC8696                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.32$\pm$0.16 & 0.872 & 1.21e+43 & 0.46  & 0.587 & 0.860 & 1.43e+10 & 2.35e+11 & \textsc{Galfit}   & 0.089$\pm$0.049 & 1.63e+08 & SN    & 15.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5297                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 2.0   & 11.92$\pm$0.05 & 0.986 & 1.78e+42 & 3.69  & 1.156 & 1.024 & 4.14e+09 & 6.08e+10 & \textsc{Galfit}   & 0.060$\pm$0.022 & 3.09e+07 & LINER & 22.2\\ 
\rowcolor{White}
NGC5297                & Sersic + exDisk          & exDisk         & disk  & --- & 23.0  & 8.94 $\pm$0.04 & 0.986 & 2.77e+43 & 2.15  & 0.837 & 1.024 & 4.66e+10 & 6.08e+10 & \textsc{Galfit}   & 0.060$\pm$0.022 & 3.09e+07 & LINER & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MK796                  & Sersic                   & Sersic         & mixed & 4.0 & 2.4   & 11.05$\pm$0.04 & 0.924 & 3.78e+43 & NA    & NA    & 0.740 & ---   & 5.62e+10 & $C\mapsto$~B/T    & 0.144$\pm$0.038 & 9.85e+07 & SN    & 7.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS13446+1121         & Sersic + psfAgn          & Sersic         & disk  & 7.2 & 0.5   & 11.56$\pm$0.05 & 0.902 & 2.60e+43 & 2.71  & 0.941 & 0.880 & 4.92e+10 & 5.13e+10 & \textsc{Galfit}   & 0.106$\pm$0.028 & 1.04e+08 & SN    & 8.1 \\ 
\rowcolor{White}
IRAS13446+1121         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.87$\pm$0.32 & 0.902 & 3.09e+42 & 1.84  & 0.784 & 0.880 & 4.87e+09 & 5.13e+10 & \textsc{Galfit}   & 0.106$\pm$0.028 & 1.04e+08 & SN    & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5303                & Sersic + psfAgn          & Sersic         & disk  & 0.5 & 10.3  & 10.40$\pm$0.04 & 0.992 & 4.02e+42 & 1.27  & 0.696 & 0.754 & 5.63e+09 & 6.45e+09 & \textsc{Galfit}   & 0.053$\pm$0.012 & 2.30e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{LightGray}
NGC5303                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.54$\pm$0.04 & 0.992 & 2.23e+41 & 3.61  & 1.136 & 0.754 & 5.10e+08 & 6.45e+09 & \textsc{Galfit}   & 0.053$\pm$0.012 & 2.30e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5313                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.1   & 10.99$\pm$0.04 & 0.984 & 4.18e+42 & 2.67  & 0.933 & 0.947 & 7.85e+09 & 6.16e+10 & \textsc{Galfit}   & 0.129$\pm$0.021 & 3.09e+07 & LINER & 22.2\\ 
\rowcolor{White}
NGC5313                & Sersic + exDisk          & exDisk         & disk  & --- & 14.3  & 8.92 $\pm$0.04 & 0.984 & 2.82e+43 & 2.11  & 0.830 & 0.947 & 4.71e+10 & 6.16e+10 & \textsc{Galfit}   & 0.129$\pm$0.021 & 3.09e+07 & LINER & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG3-35-034\_NED01     & Sersic                   & Sersic         & mixed & 5.2 & 9.2   & 10.50$\pm$0.04 & 0.900 & 2.01e+44 & NA    & NA    & 0.867 & ---   & 3.50e+11 & $C\mapsto$~B/T    & 0.178$\pm$0.047 & 1.79e+08 & TO    & 4.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5347                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.7   & 11.50$\pm$0.04 & 0.981 & 4.15e+42 & 2.28  & 0.860 & 0.886 & 7.18e+09 & 3.20e+10 & \textsc{Galfit}   & 0.230$\pm$0.024 & 3.90e+07 & SN    & 4.3 \\ 
\rowcolor{White}
NGC5347                & Sersic + exDisk          & exDisk         & disk  & --- & 11.8  & 10.19$\pm$0.04 & 0.981 & 1.39e+43 & 2.32  & 0.867 & 0.886 & 2.42e+10 & 3.20e+10 & \textsc{Galfit}   & 0.230$\pm$0.024 & 3.90e+07 & SN    & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5350                & Sersic + psfAgn          & Sersic         & disk  & 2.2 & 44.2  & 8.19 $\pm$0.04 & 0.999 & 5.60e+43 & 2.27  & 0.858 & 0.816 & 9.67e+10 & 9.28e+10 & \textsc{Galfit}   & 0.013$\pm$0.003 & 3.09e+07 & H\,{\sevensize II} & 22.2\\ 
\rowcolor{LightGray}
NGC5350                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.90$\pm$0.04 & 0.999 & 7.31e+41 & 0.91  & 0.645 & 0.816 & 9.49e+08 & 9.28e+10 & \textsc{Galfit}   & 0.013$\pm$0.003 & 3.09e+07 & H\,{\sevensize II} & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5368                & Sersic + psfAgn          & Sersic         & disk  & 2.2 & 6.5   & 10.39$\pm$0.04 & 0.968 & 4.17e+43 & 2.24  & 0.853 & 0.900 & 7.16e+10 & 8.43e+10 & \textsc{Galfit}   & 0.108$\pm$0.022 & 7.46e+07 & H\,{\sevensize II} & 4.3 \\ 
\rowcolor{White}
NGC5368                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.68$\pm$0.06 & 0.968 & 5.06e+42 & 3.51  & 1.113 & 0.900 & 1.13e+10 & 8.43e+10 & \textsc{Galfit}   & 0.108$\pm$0.022 & 7.46e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC8827                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.9   & 11.12$\pm$0.05 & 0.958 & 2.76e+43 & 1.94  & 0.801 & 0.822 & 4.45e+10 & 8.53e+10 & \textsc{Galfit}   & 0.535$\pm$0.080 & 8.54e+07 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{LightGray}
UGC8827                & Sersic + exDisk          & exDisk         & disk  & --- & 5.1   & 11.27$\pm$0.04 & 0.958 & 2.40e+43 & 2.00  & 0.811 & 0.822 & 3.92e+10 & 8.53e+10 & \textsc{Galfit}   & 0.535$\pm$0.080 & 8.54e+07 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC8856\_NED01         & Sersic                   & Sersic         & mixed & 3.6 & 5.5   & 11.53$\pm$0.04 & 0.900 & 4.63e+43 & NA    & NA    & 0.841 & ---   & 7.84e+10 & $C\mapsto$~B/T    & 0.177$\pm$0.047 & 1.38e+08 & H\,{\sevensize II} & 4.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5374                & Sersic                   & Sersic         & mixed & 5.7 & 31.2  & 9.29 $\pm$0.04 & 0.981 & 9.92e+43 & NA    & NA    & 0.797 & ---   & 1.59e+11 & $C\mapsto$~B/T    & 0.105$\pm$0.028 & 6.89e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC8902                & Sersic + psfAgn + exDisk & Sersic         & bulge & 4.0 & 3.3   & 10.74$\pm$0.04 & 0.951 & 6.98e+43 & 3.26  & 1.056 & 0.958 & 1.48e+11 & 2.90e+11 & \textsc{Galfit}   & 0.461$\pm$0.079 & 1.14e+08 & TO    & 3.8 \\ 
\rowcolor{White}
UGC8902                & Sersic + psfAgn + exDisk & psfAgn         & AGN   & --- & ---   & 13.99$\pm$0.06 & 0.951 & 3.50e+42 & NA    & NA    & 0.958 & ---   & 2.90e+11 & \textsc{Galfit}   & 0.461$\pm$0.079 & 1.14e+08 & TO    & 3.8 \\ 
\rowcolor{White}
UGC8902                & Sersic + psfAgn + exDisk & exDisk         & disk  & --- & 13.3  & 10.57$\pm$0.04 & 0.951 & 8.16e+43 & 1.97  & 0.806 & 0.958 & 1.32e+11 & 2.90e+11 & \textsc{Galfit}   & 0.461$\pm$0.079 & 1.14e+08 & TO    & 3.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG7-29-036            & Sersic + psfAgn          & Sersic         & disk  & 0.5 & 8.1   & 12.12$\pm$0.04 & 0.913 & 3.00e+43 & 2.75  & 0.949 & 0.954 & 5.73e+10 & 7.39e+10 & \textsc{Galfit}   & 0.222$\pm$0.038 & 1.45e+08 & H\,{\sevensize II} & 8.4 \\ 
\rowcolor{LightGray}
MCG7-29-036            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.48$\pm$0.04 & 0.913 & 8.58e+42 & 4.05  & 1.246 & 0.954 & 2.15e+10 & 7.39e+10 & \textsc{Galfit}   & 0.222$\pm$0.038 & 1.45e+08 & H\,{\sevensize II} & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5414                & Sersic                   & Sersic         & mixed & 1.7 & 7.7   & 10.98$\pm$0.04 & 0.986 & 2.07e+43 & NA    & NA    & 0.708 & ---   & 2.94e+10 & $C\mapsto$~B/T    & 0.164$\pm$0.043 & 6.83e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG5-33-046            & Sersic + psfAgn          & Sersic         & disk  & 3.0 & 5.9   & 11.06$\pm$0.04 & 0.955 & 5.40e+43 & 2.60  & 0.920 & 1.008 & 1.00e+11 & 1.22e+11 & \textsc{Galfit}   & 0.101$\pm$0.032 & 1.16e+08 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{LightGray}
MCG5-33-046            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.43$\pm$0.08 & 0.955 & 6.08e+42 & 2.60  & 0.920 & 1.008 & 1.13e+10 & 1.22e+11 & \textsc{Galfit}   & 0.101$\pm$0.032 & 1.16e+08 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5474                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 37.4  & 9.35 $\pm$0.04 & 0.999 & 6.31e+41 & 1.71  & 0.763 & 0.816 & 9.69e+08 & 1.04e+09 & \textsc{Galfit}   & 0.001$\pm$0.002 & 5.60e+06 & H\,{\sevensize II} & 1.7 \\ 
\rowcolor{White}
NGC5474                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 16.62$\pm$0.31 & 0.999 & 7.80e+38 & 1.71  & 0.763 & 0.816 & 1.20e+06 & 1.04e+09 & \textsc{Galfit}   & 0.001$\pm$0.002 & 5.60e+06 & H\,{\sevensize II} & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5480                & Sersic                   & Sersic         & mixed & 3.0 & 41.7  & 8.70 $\pm$0.04 & 0.988 & 3.37e+43 & NA    & NA    & 0.760 & ---   & 5.15e+10 & $C\mapsto$~B/T    & 0.097$\pm$0.026 & 3.05e+07 & H\,{\sevensize II} & 5.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG6-31-070            & Sersic + psfAgn          & Sersic         & disk  & 1.8 & 4.3   & 11.56$\pm$0.05 & 0.881 & 5.63e+43 & 2.52  & 0.904 & 0.958 & 1.02e+11 & 1.41e+11 & \textsc{Galfit}   & 0.231$\pm$0.052 & 1.56e+08 & H\,{\sevensize II} & 8.4 \\ 
\rowcolor{White}
MCG6-31-070            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.87$\pm$0.06 & 0.881 & 1.69e+43 & 2.52  & 0.904 & 0.958 & 3.07e+10 & 1.41e+11 & \textsc{Galfit}   & 0.231$\pm$0.052 & 1.56e+08 & H\,{\sevensize II} & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
CGCG74-129             & Sersic + psfAgn          & Sersic         & disk  & 6.9 & 13.1  & 11.15$\pm$0.10 & 0.956 & 2.15e+43 & 2.84  & 0.967 & 0.938 & 4.18e+10 & 4.79e+10 & \textsc{Galfit}   & 0.154$\pm$0.043 & 7.65e+07 & SN    & 8.1 \\ 
\rowcolor{LightGray}
CGCG74-129             & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.00$\pm$0.08 & 0.956 & 3.91e+42 & 2.84  & 0.967 & 0.938 & 7.61e+09 & 4.79e+10 & \textsc{Galfit}   & 0.154$\pm$0.043 & 7.65e+07 & SN    & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5520                & Sersic                   & Sersic         & mixed & 3.9 & 10.3  & 9.88 $\pm$0.04 & 0.987 & 1.14e+43 & NA    & NA    & 0.792 & ---   & 1.81e+10 & $C\mapsto$~B/T    & 0.200$\pm$0.053 & 3.05e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5515                & Sersic + psfAgn          & Sersic         & disk  & 1.8 & 8.2   & 10.10$\pm$0.04 & 0.929 & 1.22e+44 & 2.21  & 0.847 & 0.913 & 2.08e+11 & 2.48e+11 & \textsc{Galfit}   & 0.098$\pm$0.013 & 1.14e+08 & SN    & 3.8 \\ 
\rowcolor{LightGray}
NGC5515                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.51$\pm$0.05 & 0.929 & 1.33e+43 & 3.00  & 1.000 & 0.913 & 2.68e+10 & 2.48e+11 & \textsc{Galfit}   & 0.098$\pm$0.013 & 1.14e+08 & SN    & 3.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5526\_NED02         & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 19.4  & 10.42$\pm$0.04 & 0.982 & 5.75e+42 & 2.24  & 0.853 & 0.807 & 9.87e+09 & 9.51e+09 & \textsc{Galfit}   & 0.022$\pm$0.009 & 2.79e+07 & H\,{\sevensize II} & 2.3 \\ 
\rowcolor{White}
NGC5526\_NED02         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.53$\pm$0.06 & 0.982 & 1.31e+41 & 2.35  & 0.873 & 0.807 & 2.30e+08 & 9.51e+09 & \textsc{Galfit}   & 0.022$\pm$0.009 & 2.79e+07 & H\,{\sevensize II} & 2.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5522                & Sersic + psfAgn          & Sersic         & disk  & 1.5 & 13.3  & 10.10$\pm$0.04 & 0.957 & 5.02e+43 & 2.54  & 0.908 & 0.876 & 9.17e+10 & 1.01e+11 & \textsc{Galfit}   & 0.122$\pm$0.012 & 7.21e+07 & H\,{\sevensize II} & 4.3 \\ 
\rowcolor{LightGray}
NGC5522                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.24$\pm$0.04 & 0.957 & 7.00e+42 & 4.19  & 1.283 & 0.876 & 1.81e+10 & 1.01e+11 & \textsc{Galfit}   & 0.122$\pm$0.012 & 7.21e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5541                & Sersic + psfAgn          & Sersic         & disk  & 0.4 & 11.5  & 10.21$\pm$0.04 & 0.931 & 1.13e+44 & 1.69  & 0.760 & 0.816 & 1.73e+11 & 1.98e+11 & \textsc{Galfit}   & 0.058$\pm$0.012 & 1.15e+08 & LINER & 8.7 \\ 
\rowcolor{White}
NGC5541                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.23$\pm$0.04 & 0.931 & 7.01e+42 & 3.35  & 1.076 & 0.816 & 1.52e+10 & 1.98e+11 & \textsc{Galfit}   & 0.058$\pm$0.012 & 1.15e+08 & LINER & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC4395                 & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 4.5   & 10.92$\pm$0.04 & 0.913 & 1.11e+44 & 1.82  & 0.781 & 0.842 & 1.74e+11 & 2.38e+11 & \textsc{Galfit}   & 0.204$\pm$0.015 & 1.60e+08 & H\,{\sevensize II} & 8.4 \\ 
\rowcolor{LightGray}
IC4395                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.40$\pm$0.04 & 0.913 & 2.85e+43 & 3.40  & 1.087 & 0.842 & 6.23e+10 & 2.38e+11 & \textsc{Galfit}   & 0.204$\pm$0.015 & 1.60e+08 & H\,{\sevensize II} & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC9165                & Sersic + psfAgn          & Sersic         & disk  & 0.6 & 13.2  & 10.42$\pm$0.04 & 0.932 & 4.64e+43 & 2.62  & 0.923 & 0.849 & 8.62e+10 & 8.52e+10 & \textsc{Galfit}   & 0.072$\pm$0.007 & 8.13e+07 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
UGC9165                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.20$\pm$0.04 & 0.932 & 3.58e+42 & 3.42  & 1.092 & 0.849 & 7.87e+09 & 8.52e+10 & \textsc{Galfit}   & 0.072$\pm$0.007 & 8.13e+07 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MK1490                 & Sersic + psfAgn          & Sersic         & disk  & 6.7 & 4.5   & 11.36$\pm$0.10 & 0.908 & 3.88e+43 & 2.30  & 0.864 & 0.885 & 6.75e+10 & 9.11e+10 & \textsc{Galfit}   & 0.241$\pm$0.105 & 1.16e+08 & H\,{\sevensize II} & 14.2\\ 
\rowcolor{LightGray}
MK1490                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.61$\pm$0.12 & 0.908 & 1.23e+43 & 2.30  & 0.864 & 0.885 & 2.14e+10 & 9.11e+10 & \textsc{Galfit}   & 0.241$\pm$0.105 & 1.16e+08 & H\,{\sevensize II} & 14.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5585                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 34.3  & 11.22$\pm$0.25 & 0.999 & 1.13e+41 & 1.23  & 0.690 & 0.769 & 1.57e+08 & 9.95e+08 & \textsc{Galfit}   & 0.176$\pm$0.081 & 5.60e+06 & H\,{\sevensize II} & 1.7 \\ 
\rowcolor{White}
NGC5585                & Sersic + exDisk          & exDisk         & disk  & --- & 30.8  & 9.54 $\pm$0.05 & 0.999 & 5.30e+41 & 1.52  & 0.733 & 0.769 & 7.82e+08 & 9.95e+08 & \textsc{Galfit}   & 0.176$\pm$0.081 & 5.60e+06 & H\,{\sevensize II} & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC4408                 & Sersic + psfAgn          & Sersic         & disk  & 1.3 & 6.8   & 10.67$\pm$0.04 & 0.931 & 1.01e+44 & 2.35  & 0.873 & 0.858 & 1.77e+11 & 1.86e+11 & \textsc{Galfit}   & 0.064$\pm$0.020 & 1.35e+08 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{LightGray}
IC4408                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.58$\pm$0.08 & 0.931 & 6.94e+42 & 4.02  & 1.238 & 0.858 & 1.73e+10 & 1.86e+11 & \textsc{Galfit}   & 0.064$\pm$0.020 & 1.35e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5584                & Sersic                   & Sersic         & disk  & 1.2 & 30.1  & 9.56 $\pm$0.03 & 0.991 & 8.79e+42 & 2.01  & 0.813 & 0.796 & 1.44e+10 & 1.41e+10 & \textsc{Galfit}   & 0    $\pm$0     & 2.31e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5633                & Sersic + psfAgn          & Sersic         & disk  & 0.6 & 12.6  & 9.71 $\pm$0.04 & 0.985 & 1.90e+43 & 1.76  & 0.771 & 0.787 & 2.95e+10 & 3.09e+10 & \textsc{Galfit}   & 0.030$\pm$0.005 & 3.65e+07 & H\,{\sevensize II} & 22.2\\ 
\rowcolor{LightGray}
NGC5633                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.48$\pm$0.04 & 0.985 & 5.89e+41 & 3.17  & 1.036 & 0.787 & 1.23e+09 & 3.09e+10 & \textsc{Galfit}   & 0.030$\pm$0.005 & 3.65e+07 & H\,{\sevensize II} & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5660                & Sersic                   & Sersic         & mixed & 3.0 & 43.4  & 9.06 $\pm$0.04 & 0.986 & 3.93e+43 & NA    & NA    & 0.813 & ---   & 6.43e+10 & $C\mapsto$~B/T    & 0.088$\pm$0.023 & 3.89e+07 & H\,{\sevensize II} & 14.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5656                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.4   & 11.96$\pm$0.06 & 0.974 & 5.12e+42 & 2.87  & 0.973 & 0.883 & 1.00e+10 & 9.88e+10 & \textsc{Galfit}   & 0.093$\pm$0.029 & 5.37e+07 & LINER & 22.2\\ 
\rowcolor{LightGray}
NGC5656                & Sersic + exDisk          & exDisk         & disk  & --- & 8.2   & 9.48 $\pm$0.04 & 0.974 & 5.02e+43 & 1.97  & 0.806 & 0.883 & 8.14e+10 & 9.88e+10 & \textsc{Galfit}   & 0.093$\pm$0.029 & 5.37e+07 & LINER & 22.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5657                & Sersic + psfAgn          & Sersic         & disk  & 2.8 & 7.0   & 10.39$\pm$0.04 & 0.970 & 3.11e+43 & 2.71  & 0.941 & 0.860 & 5.89e+10 & 5.49e+10 & \textsc{Galfit}   & 0.018$\pm$0.010 & 6.44e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{White}
NGC5657                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.75$\pm$0.16 & 0.970 & 5.61e+41 & 6.21  & 1.959 & 0.860 & 2.21e+09 & 5.49e+10 & \textsc{Galfit}   & 0.018$\pm$0.010 & 6.44e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
CGCG133-083            & Sersic + psfAgn          & Sersic         & disk  & 5.2 & 15.9  & 11.71$\pm$0.13 & 0.865 & 7.21e+43 & 2.06  & 0.821 & 0.816 & 1.19e+11 & 1.55e+11 & \textsc{Galfit}   & 0.235$\pm$0.050 & 1.91e+08 & H\,{\sevensize II} & 8.4 \\ 
\rowcolor{LightGray}
CGCG133-083            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.99$\pm$0.05 & 0.865 & 2.22e+43 & 3.07  & 1.015 & 0.816 & 4.53e+10 & 1.55e+11 & \textsc{Galfit}   & 0.235$\pm$0.050 & 1.91e+08 & H\,{\sevensize II} & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG7-30-028            & Sersic + psfAgn          & Sersic         & disk  & 5.0 & 3.7   & 11.07$\pm$0.04 & 0.912 & 5.09e+43 & 2.01  & 0.813 & 0.811 & 8.33e+10 & 8.53e+10 & \textsc{Galfit}   & 0.030$\pm$0.020 & 1.16e+08 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
MCG7-30-028            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.84$\pm$0.20 & 0.912 & 1.58e+42 & 2.65  & 0.929 & 0.811 & 2.95e+09 & 8.53e+10 & \textsc{Galfit}   & 0.030$\pm$0.020 & 1.16e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG6-32-070            & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 5.8   & 10.76$\pm$0.04 & 0.944 & 8.38e+43 & 1.53  & 0.735 & 0.768 & 1.24e+11 & 1.35e+11 & \textsc{Galfit}   & 0.042$\pm$0.014 & 1.27e+08 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{LightGray}
MCG6-32-070            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.16$\pm$0.06 & 0.944 & 3.66e+42 & 3.80  & 1.182 & 0.768 & 8.70e+09 & 1.35e+11 & \textsc{Galfit}   & 0.042$\pm$0.014 & 1.27e+08 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC9412                & Sersic + psfAgn          & Sersic         & disk  & 1.6 & 7.5   & 11.02$\pm$0.04 & 0.859 & 7.15e+43 & 0.75  & 0.624 & 0.675 & 8.98e+10 & 1.92e+11 & \textsc{Galfit}   & 0.493$\pm$0.017 & 1.39e+08 & SN    & 1.7 \\ 
\rowcolor{White}
UGC9412                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 11.05$\pm$0.04 & 0.859 & 6.96e+43 & 0.03  & 0.537 & 0.675 & 7.52e+10 & 1.92e+11 & \textsc{Galfit}   & 0.493$\pm$0.017 & 1.39e+08 & SN    & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5698                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.4   & 12.16$\pm$0.05 & 0.973 & 5.47e+42 & 1.95  & 0.803 & 0.854 & 8.84e+09 & 5.71e+10 & \textsc{Galfit}   & 0.165$\pm$0.044 & 6.09e+07 & H\,{\sevensize II} & 4.3 \\ 
\rowcolor{LightGray}
NGC5698                & Sersic + exDisk          & exDisk         & disk  & --- & 12.8  & 10.40$\pm$0.04 & 0.973 & 2.77e+43 & 2.09  & 0.826 & 0.854 & 4.60e+10 & 5.71e+10 & \textsc{Galfit}   & 0.165$\pm$0.044 & 6.09e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5691                & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 18.2  & 10.01$\pm$0.03 & 0.993 & 4.27e+42 & 1.32  & 0.703 & 0.695 & 6.04e+09 & 6.09e+09 & \textsc{Galfit}   & 0.017$\pm$0.009 & 1.98e+07 & H\,{\sevensize II} & 9.5 \\ 
\rowcolor{White}
NGC5691                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.43$\pm$0.06 & 0.993 & 7.29e+40 & 0.95  & 0.651 & 0.695 & 9.55e+07 & 6.09e+09 & \textsc{Galfit}   & 0.017$\pm$0.009 & 1.98e+07 & H\,{\sevensize II} & 9.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG9-24-035            & Sersic + psfAgn          & Sersic         & disk  & 3.4 & 8.6   & 10.50$\pm$0.05 & 0.912 & 1.20e+44 & 2.31  & 0.865 & 0.868 & 2.09e+11 & 2.44e+11 & \textsc{Galfit}   & 0.139$\pm$0.034 & 1.37e+08 & H\,{\sevensize II} & 6.0 \\ 
\rowcolor{LightGray}
MCG9-24-035            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.49$\pm$0.05 & 0.912 & 1.93e+43 & 2.38  & 0.878 & 0.868 & 3.41e+10 & 2.44e+11 & \textsc{Galfit}   & 0.139$\pm$0.034 & 1.37e+08 & H\,{\sevensize II} & 6.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG9-24-038            & Sersic + psfAgn          & Sersic         & disk  & 3.4 & 7.2   & 11.29$\pm$0.05 & 0.881 & 8.26e+43 & 3.20  & 1.043 & 0.990 & 1.73e+11 & 1.79e+11 & \textsc{Galfit}   & 0.081$\pm$0.030 & 1.67e+08 & H\,{\sevensize II} & 4.7 \\ 
\rowcolor{White}
MCG9-24-038            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.93$\pm$0.11 & 0.881 & 7.26e+42 & 2.06  & 0.821 & 0.990 & 1.20e+10 & 1.79e+11 & \textsc{Galfit}   & 0.081$\pm$0.030 & 1.67e+08 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC9560                & Sersic                   & Sersic         & mixed & 3.6 & 7.8   & 12.42$\pm$0.09 & 0.994 & 6.27e+41 & NA    & NA    & 0.594 & ---   & 7.50e+08 & $C\mapsto$~B/T    & 0.169$\pm$0.045 & 2.30e+07 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC1076                 & Sersic + psfAgn          & Sersic         & disk  & 0.8 & 7.3   & 11.13$\pm$0.04 & 0.966 & 3.23e+43 & 1.59  & 0.744 & 0.762 & 4.84e+10 & 5.05e+10 & \textsc{Galfit}   & 0.021$\pm$0.021 & 9.25e+07 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
IC1076                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.31$\pm$0.16 & 0.966 & 6.88e+41 & 2.66  & 0.931 & 0.762 & 1.29e+09 & 5.05e+10 & \textsc{Galfit}   & 0.021$\pm$0.021 & 9.25e+07 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS14538+1730         & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 0.9   & 12.51$\pm$0.04 & 0.564 & 1.16e+44 & 2.65  & 0.929 & 1.021 & 2.17e+11 & 2.38e+11 & \textsc{Galfit}   & 1.000$\pm$0.265 & 4.33e+08 & H\,{\sevensize II} & 6.6 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC9618\_NED02         & Sersic                   & Sersic         & mixed & 2.0 & 8.0   & 10.25$\pm$0.04 & 0.863 & 1.61e+44 & NA    & NA    & 1.183 & ---   & 3.84e+11 & $C\mapsto$~B/T    & 0.162$\pm$0.043 & 1.46e+08 & TO    & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC9639                & Sersic + psfAgn          & Sersic         & disk  & 1.6 & 6.3   & 10.60$\pm$0.04 & 0.920 & 1.46e+44 & 1.97  & 0.806 & 0.865 & 2.37e+11 & 2.79e+11 & \textsc{Galfit}   & 0.088$\pm$0.016 & 1.58e+08 & SN    & 1.5 \\ 
\rowcolor{LightGray}
UGC9639                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.14$\pm$0.06 & 0.920 & 1.41e+43 & 4.00  & 1.233 & 0.865 & 3.50e+10 & 2.79e+11 & \textsc{Galfit}   & 0.088$\pm$0.016 & 1.58e+08 & SN    & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5879                & Sersic + psfAgn          & Sersic         & disk  & 1.7 & 19.4  & 8.84 $\pm$0.04 & 0.994 & 7.70e+42 & 2.20  & 0.846 & 0.864 & 1.31e+10 & 1.36e+10 & \textsc{Galfit}   & 0.020$\pm$0.004 & 1.55e+07 & LINER & 13.2\\ 
\rowcolor{White}
NGC5879                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.06$\pm$0.05 & 0.994 & 1.58e+41 & 4.12  & 1.265 & 0.864 & 4.02e+08 & 1.36e+10 & \textsc{Galfit}   & 0.020$\pm$0.004 & 1.55e+07 & LINER & 13.2\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG9-25-036            & Sersic + psfAgn          & Sersic         & disk  & 0.6 & 6.5   & 12.01$\pm$0.04 & 0.958 & 4.27e+43 & 1.67  & 0.757 & 0.770 & 6.50e+10 & 7.19e+10 & \textsc{Galfit}   & 0.080$\pm$0.042 & 1.60e+08 & H\,{\sevensize II} & 2.0 \\ 
\rowcolor{LightGray}
MCG9-25-036            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.66$\pm$0.06 & 0.958 & 3.72e+42 & 2.66  & 0.931 & 0.770 & 6.97e+09 & 7.19e+10 & \textsc{Galfit}   & 0.080$\pm$0.042 & 1.60e+08 & H\,{\sevensize II} & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5905                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 2.1   & 10.84$\pm$0.04 & 0.974 & 1.72e+43 & 2.14  & 0.835 & 0.892 & 2.89e+10 & 1.09e+11 & \textsc{Galfit}   & 0.283$\pm$0.041 & 5.87e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{White}
NGC5905                & Sersic + exDisk          & exDisk         & disk  & --- & 16.0  & 9.83 $\pm$0.04 & 0.974 & 4.35e+43 & 2.25  & 0.855 & 0.892 & 7.48e+10 & 1.09e+11 & \textsc{Galfit}   & 0.283$\pm$0.041 & 5.87e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IC4553                 & Sersic + psfAgn          & Sersic         & disk  & 3.7 & 13.3  & 9.61 $\pm$0.04 & 0.939 & 1.04e+44 & 2.88  & 0.975 & 0.910 & 2.04e+11 & 2.07e+11 & \textsc{Galfit}   & 0.083$\pm$0.010 & 8.35e+07 & LINER & 15.5\\ 
\rowcolor{LightGray}
IC4553                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.21$\pm$0.04 & 0.939 & 9.47e+42 & 2.88  & 0.975 & 0.910 & 1.86e+10 & 2.07e+11 & \textsc{Galfit}   & 0.083$\pm$0.010 & 8.35e+07 & LINER & 15.5\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC4567                 & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.1   & 12.33$\pm$0.08 & 0.957 & 9.73e+42 & 2.89  & 0.977 & 0.839 & 1.91e+10 & 1.48e+11 & \textsc{Galfit}   & 0.111$\pm$0.191 & 8.86e+07 & H\,{\sevensize II} & 5.0 \\ 
\rowcolor{White}
IC4567                 & Sersic + exDisk          & exDisk         & disk  & --- & 7.9   & 10.07$\pm$0.04 & 0.957 & 7.80e+43 & 1.83  & 0.783 & 0.839 & 1.23e+11 & 1.48e+11 & \textsc{Galfit}   & 0.111$\pm$0.191 & 8.86e+07 & H\,{\sevensize II} & 5.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG4-37-016            & Sersic + psfAgn          & Sersic         & disk  & 3.2 & 15.5  & 10.91$\pm$0.06 & 0.947 & 4.80e+43 & 1.99  & 0.809 & 0.792 & 7.81e+10 & 8.55e+10 & \textsc{Galfit}   & 0.105$\pm$0.024 & 1.03e+08 & H\,{\sevensize II} & 8.1 \\ 
\rowcolor{LightGray}
MCG4-37-016            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.24$\pm$0.06 & 0.947 & 5.62e+42 & 1.01  & 0.659 & 0.792 & 7.45e+09 & 8.55e+10 & \textsc{Galfit}   & 0.105$\pm$0.024 & 1.03e+08 & H\,{\sevensize II} & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5975                & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 10.2  & 10.13$\pm$0.04 & 0.958 & 4.52e+43 & 2.99  & 0.998 & 0.952 & 9.08e+10 & 9.32e+10 & \textsc{Galfit}   & 0.072$\pm$0.011 & 6.93e+07 & LINER & 7.4 \\ 
\rowcolor{White}
NGC5975                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.91$\pm$0.04 & 0.958 & 3.49e+42 & 4.16  & 1.275 & 0.952 & 8.95e+09 & 9.32e+10 & \textsc{Galfit}   & 0.072$\pm$0.011 & 6.93e+07 & LINER & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5980                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 0.9   & 11.99$\pm$0.06 & 0.960 & 7.24e+42 & 4.32  & 1.319 & 0.884 & 1.92e+10 & 1.31e+11 & \textsc{Galfit}   & 0.098$\pm$0.076 & 6.52e+07 & H\,{\sevensize II} & 12.1\\ 
\rowcolor{LightGray}
NGC5980                & Sersic + exDisk          & exDisk         & disk  & --- & 9.6   & 9.58 $\pm$0.04 & 0.960 & 6.66e+43 & 2.18  & 0.842 & 0.884 & 1.13e+11 & 1.31e+11 & \textsc{Galfit}   & 0.098$\pm$0.076 & 6.52e+07 & H\,{\sevensize II} & 12.1\\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC5992                & Sersic + psfAgn          & Sersic         & disk  & 2.4 & 8.1   & 11.32$\pm$0.04 & 0.955 & 6.16e+43 & 1.29  & 0.699 & 0.713 & 8.66e+10 & 9.18e+10 & \textsc{Galfit}   & 0.034$\pm$0.022 & 1.40e+08 & H\,{\sevensize II} & 3.0 \\ 
\rowcolor{White}
NGC5992                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.96$\pm$0.11 & 0.955 & 2.16e+42 & 1.67  & 0.757 & 0.713 & 3.29e+09 & 9.18e+10 & \textsc{Galfit}   & 0.034$\pm$0.022 & 1.40e+08 & H\,{\sevensize II} & 3.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC5996                & Sersic + psfAgn          & Sersic         & disk  & 1.9 & 18.9  & 10.32$\pm$0.04 & 0.966 & 2.32e+43 & 1.31  & 0.702 & 0.696 & 3.28e+10 & 3.47e+10 & \textsc{Galfit}   & 0.066$\pm$0.023 & 5.40e+07 & H\,{\sevensize II} & 8.3 \\ 
\rowcolor{LightGray}
NGC5996                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.19$\pm$0.04 & 0.966 & 1.65e+42 & 0.47  & 0.589 & 0.696 & 1.96e+09 & 3.47e+10 & \textsc{Galfit}   & 0.066$\pm$0.023 & 5.40e+07 & H\,{\sevensize II} & 8.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS15519+3537         & Sersic                   & Sersic         & mixed & 2.8 & 1.8   & 12.59$\pm$0.04 & 0.713 & 9.11e+43 & NA    & NA    & 0.872 & ---   & 1.60e+11 & $C\mapsto$~B/T    & 0.158$\pm$0.042 & 3.54e+08 & H\,{\sevensize II} & 3.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC10099               & Sersic                   & Sersic         & mixed & 7.5 & 8.0   & 10.88$\pm$0.07 & 0.945 & 1.08e+44 & NA    & NA    & 0.671 & ---   & 1.46e+11 & $C\mapsto$~B/T    & 0.159$\pm$0.042 & 1.52e+08 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
MCG5-38-006            & Sersic + psfAgn          & Sersic         & disk  & 2.0 & 7.4   & 11.04$\pm$0.04 & 0.996 & 2.05e+43 & 2.08  & 0.825 & 0.852 & 3.40e+10 & 4.90e+10 & \textsc{Galfit}   & 0.279$\pm$0.098 & 6.96e+07 & H\,{\sevensize II} & 9.8 \\ 
\rowcolor{White}
MCG5-38-006            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.07$\pm$0.04 & 0.996 & 7.95e+42 & 2.02  & 0.814 & 0.852 & 1.30e+10 & 4.90e+10 & \textsc{Galfit}   & 0.279$\pm$0.098 & 6.96e+07 & H\,{\sevensize II} & 9.8 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC10120               & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 12.3  & 11.82$\pm$0.04 & 0.910 & 3.64e+43 & 1.34  & 0.706 & 0.747 & 5.17e+10 & 9.69e+10 & \textsc{Galfit}   & 0.434$\pm$0.010 & 1.39e+08 & SN    & 1.7 \\ 
\rowcolor{LightGray}
UGC10120               & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 12.11$\pm$0.04 & 0.910 & 2.79e+43 & 0.78  & 0.628 & 0.747 & 3.53e+10 & 9.69e+10 & \textsc{Galfit}   & 0.434$\pm$0.010 & 1.39e+08 & SN    & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC6027A               & Sersic$^{n=4}$           & Sersic$^{n=4}$ & bulge & 4.0 & 6.8   & 10.52$\pm$0.04 & 0.967 & 3.31e+43 & 2.65  & 0.929 & 1.003 & 6.19e+10 & 6.68e+10 & \textsc{Galfit}   & 1.000$\pm$0.265 & 7.06e+07 & H\,{\sevensize II} & 4.3 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
NGC6040B               & Sersic                   & Sersic         & mixed & 4.3 & 5.2   & 10.92$\pm$0.04 & 0.915 & 1.36e+44 & NA    & NA    & 0.980 & ---   & 2.68e+11 & $C\mapsto$~B/T    & 0.228$\pm$0.060 & 1.77e+08 & LINER & 1.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC10200               & Sersic + psfAgn          & Sersic         & disk  & 2.1 & 5.9   & 11.53$\pm$0.04 & 0.996 & 2.62e+42 & 1.12  & 0.674 & 0.663 & 3.55e+09 & 3.67e+09 & \textsc{Galfit}   & 0.048$\pm$0.029 & 3.12e+07 & H\,{\sevensize II} & 6.9 \\ 
\rowcolor{White}
UGC10200               & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.77$\pm$0.11 & 0.996 & 1.33e+41 & 2.68  & 0.935 & 0.663 & 2.50e+08 & 3.67e+09 & \textsc{Galfit}   & 0.048$\pm$0.029 & 3.12e+07 & H\,{\sevensize II} & 6.9 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS16052+5334         & Sersic                   & Sersic         & mixed & 3.2 & 1.8   & 12.53$\pm$0.04 & 0.725 & 1.05e+44 & NA    & NA    & 0.921 & ---   & 1.94e+11 & $C\mapsto$~B/T    & 0.124$\pm$0.033 & 3.66e+08 & H\,{\sevensize II} & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS16053+1836         & Sersic                   & Sersic         & mixed & 5.4 & 1.5   & 11.29$\pm$0.04 & 0.902 & 7.93e+43 & NA    & NA    & 0.958 & ---   & 1.53e+11 & $C\mapsto$~B/T    & 0.251$\pm$0.067 & 1.61e+08 & H\,{\sevensize II} & 6.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC10273\_NED01        & Sersic + psfAgn          & Sersic         & disk  & 1.1 & 11.6  & 12.01$\pm$0.04 & 0.933 & 2.01e+43 & 1.33  & 0.705 & 0.725 & 2.85e+10 & 3.13e+10 & \textsc{Galfit}   & 0.064$\pm$0.037 & 1.11e+08 & H\,{\sevensize II} & 4.0 \\ 
\rowcolor{LightGray}
UGC10273\_NED01        & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.92$\pm$0.07 & 0.933 & 1.38e+42 & 0.88  & 0.641 & 0.725 & 1.78e+09 & 3.13e+10 & \textsc{Galfit}   & 0.064$\pm$0.037 & 1.11e+08 & H\,{\sevensize II} & 4.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IRAS16150+2233         & Sersic + psfAgn          & Sersic         & disk  & 0.6 & 4.1   & 13.08$\pm$0.04 & 0.855 & 4.29e+43 & 2.81  & 0.961 & 0.962 & 8.30e+10 & 9.03e+10 & \textsc{Galfit}   & 0.077$\pm$0.020 & 2.78e+08 & SN    & 1.5 \\ 
\rowcolor{White}
IRAS16150+2233         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 15.78$\pm$0.16 & 0.855 & 3.57e+42 & 3.75  & 1.170 & 0.962 & 8.40e+09 & 9.03e+10 & \textsc{Galfit}   & 0.077$\pm$0.020 & 2.78e+08 & SN    & 1.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
UGC10322               & Sersic + exDisk          & Sersic         & bulge & 4.0 & 1.1   & 13.61$\pm$0.14 & 0.956 & 1.82e+42 & 1.85  & 0.786 & 0.830 & 2.88e+09 & 5.00e+10 & \textsc{Galfit}   & 0.061$\pm$0.061 & 6.91e+07 & H\,{\sevensize II} & 5.5 \\ 
\rowcolor{LightGray}
UGC10322               & Sersic + exDisk          & exDisk         & disk  & --- & 8.0   & 10.64$\pm$0.04 & 0.956 & 2.81e+43 & 2.06  & 0.821 & 0.830 & 4.64e+10 & 5.00e+10 & \textsc{Galfit}   & 0.061$\pm$0.061 & 6.91e+07 & H\,{\sevensize II} & 5.5 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC6120                & Sersic + psfAgn          & Sersic         & disk  & 0.9 & 5.8   & 10.60$\pm$0.04 & 0.940 & 1.09e+44 & 1.78  & 0.774 & 0.842 & 1.70e+11 & 2.02e+11 & \textsc{Galfit}   & 0.084$\pm$0.017 & 1.35e+08 & H\,{\sevensize II} & 7.4 \\ 
\rowcolor{White}
NGC6120                & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.19$\pm$0.04 & 0.940 & 1.00e+43 & 3.96  & 1.223 & 0.842 & 2.46e+10 & 2.02e+11 & \textsc{Galfit}   & 0.084$\pm$0.017 & 1.35e+08 & H\,{\sevensize II} & 7.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG3-42-004            & Sersic + exDisk          & Sersic         & bulge & 4.0 & 3.5   & 11.63$\pm$0.04 & 0.905 & 6.60e+43 & 2.82  & 0.963 & 0.893 & 1.28e+11 & 1.93e+11 & \textsc{Galfit}   & 0.611$\pm$0.027 & 1.72e+08 & H\,{\sevensize II} & 4.7 \\ 
\rowcolor{LightGray}
MCG3-42-004            & Sersic + exDisk          & exDisk         & disk  & --- & 6.9   & 12.12$\pm$0.04 & 0.905 & 4.20e+43 & 2.19  & 0.844 & 0.893 & 7.13e+10 & 1.93e+11 & \textsc{Galfit}   & 0.611$\pm$0.027 & 1.72e+08 & H\,{\sevensize II} & 4.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC10407               & Sersic + exDisk          & Sersic         & bulge & 4.0 & 7.1   & 13.50$\pm$0.59 & 0.914 & 6.27e+42 & -0.36 & 0.495 & 0.678 & 6.24e+09 & 3.73e+10 & \textsc{Galfit}   & 0.229$\pm$0.189 & 1.25e+08 & H\,{\sevensize II} & 7.0 \\ 
\rowcolor{White}
UGC10407               & Sersic + exDisk          & exDisk         & disk  & --- & 5.1   & 12.18$\pm$0.10 & 0.914 & 2.11e+43 & 0.84  & 0.636 & 0.678 & 2.70e+10 & 3.73e+10 & \textsc{Galfit}   & 0.229$\pm$0.189 & 1.25e+08 & H\,{\sevensize II} & 7.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS16320+3922         & Sersic                   & Sersic         & mixed & 3.0 & 8.7   & 10.67$\pm$0.04 & 0.934 & 1.08e+44 & NA    & NA    & 0.844 & ---   & 1.84e+11 & $C\mapsto$~B/T    & 0.153$\pm$0.041 & 1.39e+08 & LINER & 2.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
NGC6186                & Sersic + exDisk          & Sersic         & bulge & 4.0 & 6.8   & 10.35$\pm$0.04 & 0.927 & 1.97e+44 & 2.18  & 0.842 & 0.847 & 3.34e+11 & 7.02e+11 & \textsc{Galfit}   & 0.477$\pm$0.123 & 1.63e+08 & H\,{\sevensize II} & 2.7 \\ 
\rowcolor{White}
NGC6186                & Sersic + exDisk          & exDisk         & disk  & --- & 15.2  & 10.25$\pm$0.04 & 0.927 & 2.16e+44 & 2.10  & 0.828 & 0.847 & 3.60e+11 & 7.02e+11 & \textsc{Galfit}   & 0.477$\pm$0.123 & 1.63e+08 & H\,{\sevensize II} & 2.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
MCG9-27-053            & Sersic + psfAgn          & Sersic         & disk  & 2.9 & 6.4   & 11.50$\pm$0.05 & 0.930 & 4.32e+43 & 3.42  & 1.092 & 1.048 & 9.49e+10 & 1.03e+11 & \textsc{Galfit}   & 0.110$\pm$0.028 & 1.29e+08 & H\,{\sevensize II} & 4.0 \\ 
\rowcolor{LightGray}
MCG9-27-053            & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 13.77$\pm$0.14 & 0.930 & 5.34e+42 & 4.77  & 1.449 & 1.048 & 1.56e+10 & 1.03e+11 & \textsc{Galfit}   & 0.110$\pm$0.028 & 1.29e+08 & H\,{\sevensize II} & 4.0 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
UGC10514               & Sersic                   & Sersic         & mixed & 3.2 & 8.5   & 11.36$\pm$0.04 & 0.945 & 3.02e+43 & NA    & NA    & 0.798 & ---   & 4.85e+10 & $C\mapsto$~B/T    & 0.221$\pm$0.059 & 1.00e+08 & H\,{\sevensize II} & 8.1 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS16435+2154         & Sersic + psfAgn          & Sersic         & disk  & 0.7 & 4.6   & 12.35$\pm$0.04 & 0.933 & 2.40e+43 & 2.33  & 0.869 & 0.879 & 4.20e+10 & 5.15e+10 & \textsc{Galfit}   & 0.180$\pm$0.048 & 1.42e+08 & H\,{\sevensize II} & 8.4 \\ 
\rowcolor{LightGray}
IRAS16435+2154         & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.00$\pm$0.11 & 0.933 & 5.26e+42 & 1.97  & 0.806 & 0.879 & 8.53e+09 & 5.15e+10 & \textsc{Galfit}   & 0.180$\pm$0.048 & 1.42e+08 & H\,{\sevensize II} & 8.4 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{White}
IC4623                 & Sersic + psfAgn          & Sersic         & disk  & 1.0 & 7.0   & 11.21$\pm$0.04 & 0.911 & 6.35e+43 & 2.32  & 0.867 & 0.848 & 1.11e+11 & 1.15e+11 & \textsc{Galfit}   & 0.057$\pm$0.026 & 1.38e+08 & H\,{\sevensize II} & 8.7 \\ 
\rowcolor{White}
IC4623                 & Sersic + psfAgn          & psfAgn         & bulge & --- & ---   & 14.25$\pm$0.10 & 0.911 & 3.86e+42 & 2.62  & 0.923 & 0.848 & 7.17e+09 & 1.15e+11 & \textsc{Galfit}   & 0.057$\pm$0.026 & 1.38e+08 & H\,{\sevensize II} & 8.7 \\ 
\addlinespace % requires packages booktabs and longtable
\rowcolor{LightGray}
IRAS16516+3030         & Sersic                   & Sersic         & mixed & 2.6 & 1.5   & 11.84$\pm$0.04 & 0.784 & 1.49e+44 & NA    & NA    & 0.893 & ---   & 2.68e+11 & $C\mapsto$~B/T    & 0.129$\pm$0.034 & 3.06e+08 & LINER & 1.5 \\ 

   \hline
   \addlinespace % requires packages booktabs and longtable

   \label{table:GALFIT_selected_models}
  \end{longtable}

  \vspace{-0.8cm}   

  \noindent 
  $^{(1)}$  Galaxy name;
  $^{(2)}$  Selected model (see definition in Section 4.2;
  $^{(3)}$  Selected model component (see definition in Section 4.2);
  $^{(4)}$  Physical interpretation of component;
  $^{(5)}$  S\'{e}rsic index;
  $^{(6)}$  Effective radius (for S\'{e}rsic), or scale height (for exDisk);
  $^{(7)}$  Component $K$-band magnitude (Vega system);
  $^{(8)}$  K correction factor;
  $^{(9)}$  Component $K$-band luminosity;
  $^{(10)}$ Component color form our decomposition (the global galaxy color is reported in Table D1;
  $^{(11)}$ Component mass-to-light;
  $^{(12)}$ Galaxy mass-to-light ratio;
  $^{(13)}$ Component mass;
  $^{(14)}$ Total mass$^{\dagger}$ (omitting AGN light, if any);
  $^{(15)}$ Decomposition method: labelled as ``\GALFIT{}'' in case it was
              obtained through 2D fitting, or ``$C\mapsto$~B/T''
              in case it was derived using the concentration index
	      (see Section 6.2);
  $^{(16)}$ Bulge-to-total ratio;
  $^{(17)}$ Distance from Ashby et al.\ (2001);
  $^{(18)}$ Nuclear classification by Maragkoudakis et al.\ (2018);
  $^{(19)}$ Galaxy representativeness weight from Ashby et al.\ (2001).
              If multiplied by a constant factor of 6.7, a weight provides the
	      number of galaxies that the SFRS target represents in
	      the \PSCz{} catalogue (see Ashby et al.\ 2001 for details).
	      
  \smallskip
  \noindent$^{\dagger}${\textsc NOTE}:
   Because a different $M/L$ is used for bulge, disk, and whole galaxy, the
   masses of the sub-components do \emph{not} necessarily sum up to the total
   mass.\\
 }

\end{landscape}
%----------------------------------------------------------------------------------

